The orthogonal unit group of the trivial source ring

Let $G$ be a finite group, $p$ a prime, and $(K,\mathcal{O},F)$ a $p$-modular system. We prove that the trivial source ring of $\mathcal{O} G$ is isomorphic to the ring of {\em coherent} $G$-stable tuples $(\chi_P)$, where $\chi_P$ is a virtual character of $K[N_G(P)/P]$, $P$ runs through all $p$-subgroups of $G$, and the coherence condition is the equality of certain character values. We use this result to describe the group of orthogonal units of the trivial source ring as the product of the unit group of the Burnside ring of the fusion system of $G$ with the group of coherent $G$-stable tuples $(\varphi_P)$ of homomorphisms $N_G(P)/P\to F^\times$. The orthogonal unit group of the trivial source ring of $\mathcal{O} G$ is of interest, since it embeds into the group of $p$-permutation autoequivalences of $\mathcal{O} G$.

==> diagram.tex <==
% DIAGRAM MACROS (version 3.1)

\catcode`\@=11

%%%%% FIXING SOME PARAMETERS

%%% Fixing the printerresolution
%%% unit = 1 dpi
\newcount\printerresolution
\global\printerresolution=300

%%% Fixing the length of a segment in an arrowhead
%%% unit = 0.01pt
\newcount\headsize
\global\headsize=450

%%% Fixing the thickness of an arrowhead
%%% value = 1/5 of the font size
\font\dotfont = lcircle10 at 3pt

%%% Fixing the distance between the two heads of an epimorphism
%%% unit = 0.01pt
\newcount\epihead
\global\epihead=200

%%% Fixing the default scaling factor for diagrams
\newcount\defaultscale
\def\setdefaultscale#1{\global\defaultscale=#1}
\setdefaultscale{100}

\newcount\actualtextarrowspace
\newcount\actualtextarrowlength

% \computetextparameters computes the parameters
% required to design a text arrow
\newcommand{\computetextparameters}%
{\global\actualtextarrowspace=\textarrowlength%
\global\advance\actualtextarrowspace by 3%
\global\actualtextarrowlength=\textarrowlength%
\global\multiply\actualtextarrowlength by 100}

%%% Fixing the default length of text arrows
\newcount\textarrowlength
\def\settextarrowlength#1{\global\textarrowlength=#1%
\computetextparameters}
\settextarrowlength{20}

\newcount\actualdisplayarrowspace
\newcount\actualdisplayarrowlength

% \computedisplayparameters computes the parameters
% required to design a displayed arrow
\newcommand{\computedisplayparameters}%
{\global\actualdisplayarrowspace=\displayarrowlength%
\global\advance\actualdisplayarrowspace by 3%
\global\actualdisplayarrowlength=\displayarrowlength%
\global\multiply\actualdisplayarrowlength by 100}

%%% Fixing the default length of displayed arrows
\newcount\displayarrowlength
\def\setdisplayarrowlength#1{\global\displayarrowlength=#1%
\computedisplayparameters}
\setdisplayarrowlength{30}


% ERROR MESSAGES

% Checking the next token without gobbling blanks
\def\@ifnexttok#1#2#3{\let\@tempe #1\def\@tempa{#2}\def\@tempb{#3}%
\futurelet\@tempc\@ifntok}
\def\@ifntok{\ifx \@tempc \@tempe\let\@tempd\@tempa\else\let\@tempd\@tempb\fi%
\@tempd}

%  \@diagramerror{MSG}{HLP}: Types a Diagram error message MSG and gives an error
%                            halt with error help message HLP.
\def\@diagramerror#1#2{%
\edef\@@tempc{#2}\expandafter\errhelp\expandafter{\@@tempc}%
\typeout{Diagram error. \space See User's guide for explanation.^^J
 \space\@spaces\@spaces\@spaces Type \space H <return> \space for
 immediate help.}\errmessage{#1}}

\newif\ifdiagram

% error test and message for text arrows
\def\testtextmode{%
\ifdiagram\@diagramerror{Text arrows are not allowed in diagrams}{Here you
should use east or west diagram arrows, not forward or backward text arrows.
Try proceeding now, typeset could succeed but with unpredictable output.}
\else\ifmmode\relax\else%
\@diagramerror{Missing \string$}{Text arrows should be introduced in math mode.
Try proceeding now, typeset could succeed but output could not be what you expected.}\fi\fi}

% error test and message for diagram arrows
\def\testdiagrammode{\ifdiagram\relax\else
\@diagramerror{Diagram arrows are not allowed in formulas}{Here you
should use forward or backward text arrows, not diagram arrows. Proceeding
could work with unpredictable output, but overflow arithmetic
could also occur.}\fi}

% error test and message for diagrams in math mode
\def\checkmode{\ifmmode\@diagramerror{Wrong mode: no diagrams
allowed in math mode.}{You should leave math mode before
introducing your diagram. All items in the diagram will automatically be
processed in math mode.}\else\relax\fi\global\diagramtrue}

\global\diagramfalse

%%%%% DESIGING THE ARROW HEADS

%%% Customizing the unitlength for the sake of precision
\setlength{\unitlength}{0.01pt}

%%% Printing one dot at the required scale
\def\DOT{{\dotfont q}}

%%% Computing the distance between two dots in an arrowhead
\newcount\basicstep
\basicstep=7227
\global\divide\basicstep by \printerresolution

%%% Computing the number of dots in an arrowhead
\newcount\numberofsteps
\numberofsteps=\headsize
\global\divide\numberofsteps by \basicstep

%%% Producing an arrow head
\newcommand{\makehead}[3]{%
\begin{picture}(0,0)%
\multiput(0,0)(#1,#2){#3}{\DOT}%
\multiput(0,0)(-#2,#1){#3}{\DOT}%
\end{picture}}

%%% Creating bitmap images of the arrowheads
\newcount\xstep
\newcount\ystep

\newsavebox{\northhead}
\savebox{\northhead}{%
\xstep=-\basicstep%
\multiply\xstep by 7071%
\divide\xstep by 10000%
\ystep=\xstep%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nhead}{\usebox{\northhead}}

\newsavebox{\easthead}
\savebox{\easthead}{%
\xstep=-\basicstep%
\multiply\xstep by 7071%
\divide\xstep by 10000%
\ystep=-\xstep%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\ehead}{\usebox{\easthead}}

\newsavebox{\southhead}
\savebox{\southhead}{%
\xstep=\basicstep%
\multiply\xstep by 7071%
\divide\xstep by 10000%
\ystep=\xstep%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\shead}{\usebox{\southhead}}

\newsavebox{\westhead}
\savebox{\westhead}{%
\xstep=\basicstep%
\multiply\xstep by 7071%
\divide\xstep by 10000%
\ystep=-\xstep%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\whead}{\usebox{\westhead}}

\newsavebox{\northwesthead}
\savebox{\northwesthead}{%
\makehead{0}{-\basicstep}{\numberofsteps}}
\newcommand{\nwhead}{\usebox{\northwesthead}}

\newsavebox{\northeasthead}
\savebox{\northeasthead}{%
\makehead{-\basicstep}{0}{\numberofsteps}}
\newcommand{\nehead}{\usebox{\northeasthead}}

\newsavebox{\southwesthead}
\savebox{\southwesthead}{%
\makehead{\basicstep}{0}{\numberofsteps}}
\newcommand{\swhead}{\usebox{\southwesthead}}

\newsavebox{\southeasthead}
\savebox{\southeasthead}{%
\makehead{0}{\basicstep}{\numberofsteps}}
\newcommand{\sehead}{\usebox{\southeasthead}}

\newsavebox{\eastnortheasthead}
\savebox{\eastnortheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 9486%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by -3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\enehead}{\usebox{\eastnortheasthead}}

\newsavebox{\northnortheasthead}
\savebox{\northnortheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 9486%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by 3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nnehead}{\usebox{\northnortheasthead}}

\newsavebox{\southsouthwesthead}
\savebox{\southsouthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 9486%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by 3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\sswhead}{\usebox{\southsouthwesthead}}

\newsavebox{\westsouthwesthead}
\savebox{\westsouthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 9486%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by -3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\wswhead}{\usebox{\westsouthwesthead}}

\newsavebox{\westnorthwesthead}
\savebox{\westnorthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 3162%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by -3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\wnwhead}{\usebox{\westnorthwesthead}}

\newsavebox{\eastsoutheasthead}
\savebox{\eastsoutheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 3162%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by -3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\esehead}{\usebox{\eastsoutheasthead}}

\newsavebox{\northnorthwesthead}
\savebox{\northnorthwesthead}{%
\xstep=-\basicstep%
\multiply\xstep by 3162%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by 3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nnwhead}{\usebox{\northnorthwesthead}}

\newsavebox{\southsoutheasthead}
\savebox{\southsoutheasthead}{%
\xstep=\basicstep%
\multiply\xstep by 3162%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by 3%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\ssehead}{\usebox{\southsoutheasthead}}

\newsavebox{\easteastnortheasthead}
\savebox{\easteastnortheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 8944%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by -2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\eenehead}{\usebox{\easteastnortheasthead}}

\newsavebox{\northnorthnortheasthead}
\savebox{\northnorthnortheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 8944%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by 2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nnnehead}{\usebox{\northnorthnortheasthead}}

\newsavebox{\southsouthsouthwesthead}
\savebox{\southsouthsouthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 8944%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by 2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\ssswhead}{\usebox{\southsouthsouthwesthead}}

\newsavebox{\westwestsouthwesthead}
\savebox{\westwestsouthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 8944%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by -2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\wwswhead}{\usebox{\westwestsouthwesthead}}

\newsavebox{\westwestnorthwesthead}
\savebox{\westwestnorthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 4472%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by -2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\wwnwhead}{\usebox{\westwestnorthwesthead}}

\newsavebox{\easteastsoutheasthead}
\savebox{\easteastsoutheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 4472%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by -2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\eesehead}{\usebox{\easteastsoutheasthead}}

\newsavebox{\northnorthnorthwesthead}
\savebox{\northnorthnorthwesthead}{%
\xstep=-\basicstep%
\multiply\xstep by 4472%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by 2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nnnwhead}{\usebox{\northnorthnorthwesthead}}

\newsavebox{\southsouthsoutheasthead}
\savebox{\southsouthsoutheasthead}{%
\xstep=\basicstep%
\multiply\xstep by 4472%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by 2%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\sssehead}{\usebox{\southsouthsoutheasthead}}

\newsavebox{\northeasteastnortheasthead}
\savebox{\northeasteastnortheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 9806%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by -5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\neenehead}{\usebox{\northeasteastnortheasthead}}

\newsavebox{\northeastnorthnortheasthead}
\savebox{\northeastnorthnortheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 9806%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by 5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nennehead}{\usebox{\northeastnorthnortheasthead}}

\newsavebox{\southwestsouthsouthwesthead}
\savebox{\southwestsouthsouthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 9806%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by 5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\swsswhead}{\usebox{\southwestsouthsouthwesthead}}

\newsavebox{\southwestwestsouthwesthead}
\savebox{\southwestwestsouthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 9806%
\divide\xstep by 10000%
\ystep=\xstep%
\divide\ystep by -5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\swwswhead}{\usebox{\southwestwestsouthwesthead}}

\newsavebox{\northwestwestnorthwesthead}
\savebox{\northwestwestnorthwesthead}{%
\xstep=\basicstep%
\multiply\xstep by 1961%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by -5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nwwnwhead}{\usebox{\northwestwestnorthwesthead}}

\newsavebox{\southeasteastsoutheasthead}
\savebox{\southeasteastsoutheasthead}{%
\xstep=-\basicstep%
\multiply\xstep by 1961%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by -5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\seesehead}{\usebox{\southeasteastsoutheasthead}}

\newsavebox{\northwestnorthnorthwesthead}
\savebox{\northwestnorthnorthwesthead}{%
\xstep=-\basicstep%
\multiply\xstep by 1961%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by 5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\nwnnwhead}{\usebox{\northwestnorthnorthwesthead}}

\newsavebox{\southeastsouthsoutheasthead}
\savebox{\southeastsouthsoutheasthead}{%
\xstep=\basicstep%
\multiply\xstep by 1961%
\divide\xstep by 10000%
\ystep=\xstep%
\multiply\ystep by 5%
\makehead{\xstep}{\ystep}{\numberofsteps}}
\newcommand{\sessehead}{\usebox{\southeastsouthsoutheasthead}}

%%% Restoring the standard unitlength
\setlength{\unitlength}{1pt}


% MACROS FOR MARKED ARROWS

\newsavebox{\isomorphismmark}
\newcommand{\isomark}[1]{\savebox{\isomorphismmark}{#1}}
\isomark{$\cong$}
\newcommand{\isosign}{\usebox{\isomorphismmark}}

\newif\ifuserdist
\newsavebox{\distributormark}
\newcommand{\distmark}[1]{\ifx#1\distcircle\userdistfalse\else%
\userdisttrue\savebox{\distributormark}{#1}\fi}
\newsavebox{\distributorcircle}
\savebox{\distributorcircle}{\begin{picture}(0,0)%
\put(0,0){\circle{4}}\end{picture}}
\newcommand{\distsign}{\ifuserdist\usebox{\distributormark}\else%
\usebox{\distributorcircle}\fi}
\userdistfalse



% MACROS FOR ADJUSTING THE LENGTH OF MONOMORPHISMS AND EPIMORPHISMS

\newcount\monolength
\newcount\epilength
\newcount\bimolength
\newcount\secondmonolength
\newcount\secondepilength

\newcount\monotail%
\global\monotail=\headsize%
\global\multiply\monotail by 7070%
\global\divide\monotail by 10000%

\newcount\truemonotail%
\newcount\trueepihead%

\def\truetail{\truemonotail=\monotail%
\multiply\truemonotail by 100%
\divide\truemonotail by \SCALE}

\def\truehead{\trueepihead=\epihead%
\multiply\trueepihead by 100%
\divide\trueepihead by \SCALE}

\newcount\Monotail%
\global\Monotail=\headsize%
\global\divide\Monotail by 2%

\newcount\Epihead%
\global\Epihead=\epihead%
\global\multiply\Epihead by 7070%
\global\divide\Epihead by 10000%

\newcount\Truemonotail%
\newcount\Trueepihead%

\def\Truetail{\Truemonotail=\Monotail%
\multiply\Truemonotail by 100%
\divide\Truemonotail by \SCALE}%

\def\Truehead{\Trueepihead=\Epihead%
\multiply\Trueepihead by 100%
\divide\Trueepihead by \SCALE}

\newcount\MonoTail%
\global\MonoTail=\headsize%
\global\multiply\MonoTail by 6324%
\global\divide\MonoTail by 10000%

\newcount\EpiHead%
\global\EpiHead=\epihead%
\global\multiply\EpiHead by 8944%
\global\divide\EpiHead by 10000%

\newcount\TrueMonoTail%
\newcount\TrueEpiHead%

\def\TrueTail{\TrueMonoTail=\MonoTail%
\multiply\TrueMonoTail by 100%
\divide\TrueMonoTail by \SCALE}%

\def\TrueHead{\TrueEpiHead=\EpiHead%
\multiply\TrueEpiHead by 100%
\divide\TrueEpiHead by \SCALE}

\newcount\monotaiL%
\global\monotaiL=\headsize%
\global\multiply\monotaiL by 3162%
\global\divide\monotaiL by 10000%

\newcount\epiheaD%
\global\epiheaD=\epihead%
\global\multiply\epiheaD by 4472%
\global\divide\epiheaD by 10000%

\newcount\truemonotaiL%
\newcount\trueepiheaD%

\def\truetaiL{\truemonotaiL=\monotaiL%
\multiply\truemonotaiL by 100%
\divide\truemonotaiL by \SCALE}%

\def\trueheaD{\trueepiheaD=\epiheaD%
\multiply\trueepiheaD by 100%
\divide\trueepiheaD by \SCALE}


% INITIALIZATION

\newcount\SCALE%

\newcount\NUMBER%

\newcount\LINE%

\newcount\COLUMN%

\newcount\WIDTH%

\newcount\SOURCE%

\newcount\ARROW%

\newcount\TARGET%

\newcount\ARROWLENGTH%

\newcount\NUMBEROFDOTS%

\newcounter{x}%

\newcounter{y}%

\newcounter{z}%

\newcounter{horizontal}%

\newcounter{vertical}%

\newskip\itemlength%

\newskip\firstitem%

\newskip\seconditem%

\newcommand{\printarrow}{}%

\newcount\X%

\newcount\Y%

\newcount\Z%


% MACROS FOR DESIGNING DIAGRAMS


% \truex{n} divides n x 100 by the scaling factor and puts the result
% in counter x
\newcommand{\truex}[1]{%
\NUMBER=#1%
\multiply\NUMBER by 100%
\divide\NUMBER by \SCALE%
\setcounter{x}{\NUMBER}}%

% \truey{n} divides n x 100 by the scaling factor and puts the result
% in counter y
\newcommand{\truey}[1]{%
\NUMBER=#1%
\multiply\NUMBER by 100%
\divide\NUMBER by \SCALE%
\setcounter{y}{\NUMBER}}%

% \truez{n} divides n x 100 by the scaling factor and puts the result
% in counter z
\newcommand{\truez}[1]{%
\NUMBER=#1%
\multiply\NUMBER by 100%
\divide\NUMBER by \SCALE%
\setcounter{z}{\NUMBER}}%


% \changecounters computes the values of the various parameters required
% to design an arrow with adjusted length.
\newcommand{\changecounters}[1]{%
\SOURCE=\ARROW%
\ARROW=\TARGET%
\settowidth{\itemlength}{#1}%
\ifdim \itemlength > 2800\unitlength%
\addtolength{\itemlength}{-2800\unitlength}%
\TARGET=\itemlength%
\divide\TARGET by 1310%
\multiply\TARGET by 100%
\divide\TARGET by \SCALE%
\else%
\TARGET=0%
\fi%
\ARROWLENGTH=5000%
\advance\ARROWLENGTH by -\SOURCE%
\advance\ARROWLENGTH by -\TARGET%
\divide\ARROWLENGTH by 100%
\advance\SOURCE by -\TARGET}%

% \initialize initializes the counters required to produce the diagram
% and defines the formal dimensions of the diagram to be (0,0).
\newcommand{\initialize}[1]{%
\LINE=0%
\COLUMN=0%
\WIDTH=0%
\ARROW=0%
\TARGET=0%
\changecounters{#1}%
\renewcommand{\printarrow}{#1}%
\begin{center}%
\vspace{2pt}%
\begin{picture}(0,0)}%

% \DIAGV{n} starts the construction of a diagram scaled by a factor
% n percent, computes the scaled unit length and the unscaling factor.
\newcommand{\DIAGV}[2]{%
\checkmode%
\SCALE=#1%
\setlength{\unitlength}{655sp}%
\multiply\unitlength by \SCALE%
\divide\unitlength by 100%
\initialize{\mbox{$#2$}}}%

% \n introduces the next item of the diagram, computes its parameters
% and prints the previous item.
\newcommand{\n}[1]{%
\changecounters{\mbox{$#1$}}%
\put(\COLUMN,\LINE){\makebox(0,0){\printarrow}}%
\thinlines%
\renewcommand{\printarrow}{\mbox{$#1$}}%
\advance\COLUMN by 4000}%

% \nn prints the  last item of a line and starts a new line.
\newcommand{\nn}[1]{%
\put(\COLUMN,\LINE){\makebox(0,0){\printarrow}}%
\thinlines%
\ifnum \WIDTH < \COLUMN%
\WIDTH=\COLUMN%
\else%
\fi%
\advance\LINE by -4000%
\COLUMN=0%
\ARROW=0%
\TARGET=0%
\changecounters{\mbox{$#1$}}%
\renewcommand{\printarrow}{\mbox{$#1$}}}%

% \conclude prints the last item of the diagram and sets the
% dimensions of the diagram;
\newcommand{\conclude}{%
\put(\COLUMN,\LINE){\makebox(0,0){\printarrow}}%
\thinlines%
\ifnum \WIDTH < \COLUMN%
\WIDTH=\COLUMN%
\else%
\fi%
\setcounter{horizontal}{\WIDTH}%
\setcounter{vertical}{-\LINE}%
\end{picture}}%

% \diag prints the last item of the diagram and takes care of the spacing
\newcommand{\diag}{%
\conclude%
\raisebox{0pt}[0pt][\value{vertical}\unitlength]{}%
\hspace*{\value{horizontal}\unitlength}%
\vspace{12pt}%
\end{center}%
\setlength{\unitlength}{1pt}%
\global\diagramfalse}%

% \diagv{t}{l}{b} prints the last item of the diagram and
% adds a t points extra space at the top of the diagram
% adds a l points extra space at the left of the diagram
% adds a b points extra space at the bottom of the diagram
\newcommand{\diagv}[3]{%
\conclude%
\NUMBER=#1%
\rule{0pt}{\NUMBER pt}%
\hspace*{-#2pt}%
\raisebox{0pt}[0pt][\value{vertical}\unitlength]{}%
\hspace*{\value{horizontal}\unitlength}%6
\NUMBER=#3%
\advance\NUMBER by 12%
\vspace*{\NUMBER pt}%
\end{center}%
\setlength{\unitlength}{1pt}%
\global\diagramfalse}%

% \movename(n,m){f} moves the name f of the arrow n points right
% and m points up.
\def\movename(#1,#2)#3{%
\hspace{#1pt}%
\raisebox{#2pt}[5pt][2pt]{\raisebox{#2pt}{$#3$}}%
\hspace{-#1pt}}%

% \movearrow(n,m){\...} moves arrow \... n points right
% and m points up.
\def\movearrow(#1,#2)#3{%
\makebox[0pt]{%
\hspace{#1pt}\hspace{#1pt}%
\raisebox{#2pt}[0pt][0pt]{\raisebox{#2pt}{$#3$}}}}%

% \movevertex(n,m){A} moves vertex A n points right and m points up
\def\movevertex(#1,#2)#3{%
\mbox{\hspace{#1pt}%
\raisebox{#2pt}{\raisebox{#2pt}{$#3$}}%
\hspace{-#1pt}}}%

% \movevertexleft{XXX} moves vertex XXX left
\newcommand{\movevertexleft}[1]{\makebox[2800\unitlength][r]{$#1$}}

% \movevertexright{XXX} moves vertex XXX right
\newcommand{\movevertexright}[1]{\makebox[2800\unitlength][l]{$#1$}}

% \crosslength{P}{Q} computes the formal dimensions of the
% superposition of pictures P and Q
\newcommand{\crosslength}[2]{%
\settowidth{\firstitem}{#1}%
\settowidth{\seconditem}{#2}%
\ifdim\firstitem < \seconditem%
\itemlength=\seconditem%
\else%
\itemlength=\firstitem%
\fi%
\divide\itemlength by 2%
\hspace{\itemlength}}%

% \cross{P}{Q} superposes pictures P and Q
\newcommand{\cross}[2]{%
\crosslength{\mbox{$#1$}}{\mbox{$#2$}}%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0){$#1$}}%
\thinlines%
\put(0,0){\makebox(0,0){$#2$}}%
\thinlines%
\end{picture}%
\crosslength{\mbox{$#1$}}{\mbox{$#2$}}}%

% \bold prints the next arrow in bold-face type
\newcommand{\bold}{\ifdiagram\thicklines\else\typeout{Sorry: command
\string\bold does not apply to text arrows; I am ignoring it.}\fi}

% \unbold switches back to normal arrows
\newcommand{\unbold}{\thinlines}

% SHORTENING THE TYPING OF DIAGRAMS

\def\basicDIAG#1&{\DIAGV{\defaultscale}{#1}\@ifnexttok&{\finishline}{\basicn}}
\def\basicDIAGV[#1]#2&{\DIAGV{#1}{#2}\@ifnexttok&{\finishline}{\basicn}}
\def\basicn#1&{\n{#1}\@ifnexttok&{\finishline}{\basicn}}
\def\basicnn#1&{\nn{#1}\@ifnexttok&{\finishline}{\basicn}}
\def\finishline#1{\@ifnextchar\end{\diag}%
{\@ifnextchar\spacing{\relax}{\basicnn}}}
\def\spacing(#1,#2,#3){\diagv{#1}{#2}{#3}}

\newif\ifcaption%

\newenvironment{diagram}{%
\iffloatdiag\relax\else
\global\def\diagramcaption##1{%
\global\captiontrue%
\global\def\@diagcaption{##1}}%
\global\def\@diagcaption{}\fi%
\@ifnextchar[{\basicDIAGV}{\basicDIAG}}%
{\iffloatdiag\relax\else%
\ifcaption
\begin{center}\mbox{}\@diagcaption\end{center}%
\else\relax\fi\fi\global\captionfalse}

\global\captionfalse


% MACROS FOR FLOATING DIAGRAMS

\gdef\@diaglabel{Diagram}
\gdef\diagramlabel#1{\gdef\@diaglabel{#1}}

\newcounter{Diagram}
\setcounter{Diagram}{0}
\def\theDiagram{\@arabic\c@Diagram}
\def\fps@Diagram{tbp}
\def\ftype@Diagram{1}
\def\ext@Diagram{lof}
\def\fnum@Diagram{\@diaglabel\ \theDiagram}
\def\Diagram{\@float{Diagram}}
\let\endDiagram\end@float
\@namedef{Diagram*}{\@dblfloat{Diagram}}
\@namedef{endDiagram*}{\end@dblfloat}

\def\setdiagramcounter#1{\@addtoreset{Diagram}{#1}%
\def\theDiagram{\arabic{#1}.\@arabic\c@Diagram}}

\newif\iffloatdiag

\newenvironment{floatingdiagram}{%
\global\floatdiagtrue%
\long\def\@makecaption##1##2{
 \vskip 0pt
 \setbox\@tempboxa\hbox{##1##2}
 \ifdim \wd\@tempboxa >\hsize \unhbox\@tempboxa\par \else \hbox
to\hsize{\hfil\box\@tempboxa\hfil}
 \fi}%
\global\def\diagramcaption##1{\global\def\@diagcaption{: ##1}}%
\global\def\@diagcaption{}%
\begin{Diagram}[tbp]\begin{diagram}}%
{\end{diagram}\caption{\@diagcaption}\end{Diagram}%
\global\floatdiagfalse}

\global\floatdiagfalse


% MACROS FOR DRAWING TEXT PICTURES

% moving a name up
\newcommand{\TUP}[1]{\raisebox{0pt}[0pt][3pt]{}#1}

% moving a name down
\newcommand{\TDOWN}[1]{\raisebox{0pt}[6pt][0pt]{}#1}

% \tlowername{P}{f} puts the name f under the picture P
\newcommand{\tlowername}[2]%
{$\stackrel{\makebox[1pt]{#1}}%
{\begin{picture}(0,0)%
\put(0,0){\makebox(0,6)[t]{\makebox[1pt]{$\scriptstyle#2$}}}%
\end{picture}}$}%

% \tcase{P} draws the picture P with length \textarrowlength pt.
\newcommand{\tcase}[1]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualtextarrowspace pt]%
{\raisebox{2.5pt}{#1{\actualtextarrowlength}}}%
\setlength{\unitlength}{1pt}}%

% \Tcase{P}{f} draws the picture P with upper name f
% and length \textarrowlength pt.
\newcommand{\Tcase}[2]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualtextarrowspace pt]%
{\raisebox{2.5pt}{$\stackrel{\scriptstyle #2}{#1{\actualtextarrowlength}}$}}%
\setlength{\unitlength}{1pt}}%

% \tbicase{P} draws the bi-picture P
% with length \textarrowlength pt.
\newcommand{\tbicase}[1]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualtextarrowspace pt]%
{\raisebox{1pt}{#1{\actualtextarrowlength}}}%
\setlength{\unitlength}{1pt}}%

% \Tbicase{P}{f}{g} draws the bi-picture P with names f, g
% and length \textarrowlength pt.
\newcommand{\Tbicase}[3]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualtextarrowspace pt]%
{\raisebox{-1pt}%
{$\stackrel{\scriptstyle #2}%
{\mbox{\tlowername{#1{\actualtextarrowlength}}%
{\scriptstyle #3}}}$}}%
\setlength{\unitlength}{1pt}}%

% MACROS FOR DRAWING DISPLAYED PICTURES

% moving a name up
\newcommand{\DUP}[1]{\raisebox{0pt}[0pt][4pt]{}#1}

% moving a name down
\newcommand{\DDOWN}[1]{\raisebox{0pt}[9pt][0pt]{}#1}

% \dlowername{P}{f} puts the name f under the picture P
\newcommand{\dlowername}[2]%
{$\stackrel{\makebox[1pt]{#1}}%
{\begin{picture}(0,0)%
\put(0,0){\makebox(0,6)[t]{\makebox[1pt]{$\textstyle#2$}}}%
\end{picture}}$}%

% \dcase{P} draws the picture P with length \displayarrowlength pt.
\newcommand{\dcase}[1]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualdisplayarrowspace pt]%
{\raisebox{2.5pt}{#1{\actualdisplayarrowlength}}}%
\setlength{\unitlength}{1pt}}%

% \Dcase{P}{f} draws the picture P with upper name f
% and length \displayarrowlength pt.
\newcommand{\Dcase}[2]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualdisplayarrowspace pt]%
{\raisebox{2.5pt}{$\stackrel{\textstyle #2}{#1{\actualdisplayarrowlength}}$}}%
\setlength{\unitlength}{1pt}}%

% \dbicase{P} draws the bi-picture P
% with length \displayarrowlength pt.
\newcommand{\dbicase}[1]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualdisplayarrowspace pt]%
{\raisebox{1pt}{#1{\actualdisplayarrowlength}}}%
\setlength{\unitlength}{1pt}}%

% \Dbicase{P}{f}{g} draws the bi-picture P with names f, g
% and length \displayarrowlength pt.
\newcommand{\Dbicase}[3]{%
\testtextmode%
\setlength{\unitlength}{0.01pt}%
\makebox[\actualdisplayarrowspace pt]%
{\raisebox{-1pt}%
{$\stackrel{\textstyle #2}%
{\mbox{\tlowername{#1{\actualdisplayarrowlength}}%
{\textstyle #3}}}$}}%
\setlength{\unitlength}{1pt}}%


% IN-TEXT ARROWS

% \AR{n} draws an arrow of length n units
\newcommand{\AR}[1]%
{\begin{picture}(#1,0)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\end{picture}}%

% \DIST{n} draws a distributor of length n units
\newcommand{\DIST}[1]%
{\begin{picture}(#1,0)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{400}}%
\end{picture}}%

% \DOTAR{n} draws a dotted  arrow of length n units
\newcommand{\DOTAR}[1]%
{\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by 300%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(#1,0)%
\multiput(0,0)(300,0){\NUMBEROFDOTS}{\circle*{100}}%
\put(#1,0){\ehead}%
\end{picture}}%

% \MONO{n} draws a monomorphism of length n units
\newcommand{\MONO}[1]%
{\monolength=#1%
\advance\monolength by -\monotail%
\begin{picture}(#1,0)%
\put(\monotail,0){\line(1,0){\monolength}}%
\put(#1,0){\ehead}%
\put(\monotail,0){\ehead}%
\end{picture}}%

% \EPI{n} draws an epimorphism of length n units
\newcommand{\EPI}[1]%
{\epilength=#1%
\advance\epilength by -\epihead%
\begin{picture}(#1,0)(-#1,0)%
\put(-#1,0){\line(1,0){\epilength}}%
\put(-\epihead,0){\ehead}%
\put(0,0){\ehead}%
\end{picture}}%

% \BIMO{n} draws a bimorphism of length n units
\newcommand{\BIMO}[1]%
{\monolength=#1%
\advance\monolength by -\monotail%
\epilength=\monolength%
\advance\epilength by -\epihead%
\begin{picture}(#1,0)(-#1,0)%
\put(-\monolength,0){\line(1,0){\epilength}}%
\put(-\monolength,0){\ehead}%
\put(-\epihead,0){\ehead}%
\put(0,0){\ehead}%
\end{picture}}%

% \BIAR{n} draws a pair of arrows of length n units
\newcommand{\BIAR}[1]%
{\begin{picture}(#1,700)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(0,700){\line(1,0){#1}}%
\put(#1,700){\ehead}%
\end{picture}}%

% \BIDIST{n} draws a pair of distributors of length n units
\newcommand{\BIDIST}[1]%
{\begin{picture}(#1,700)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(0,700){\line(1,0){#1}}%
\put(#1,700){\ehead}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{400}}%
\put(\NUMBER,700){\circle{400}}%
\end{picture}}%

% \EQL{n} draws an equality of length n units
\newcommand{\EQL}[1]%
{\begin{picture}(#1,0)%
\put(0,100){\line(1,0){#1}}%
\put(0,-100){\line(1,0){#1}}%
\end{picture}}%

% \ADJAR{n} draws a pair of adjoint arrows of length n units
\newcommand{\ADJAR}[1]%
{\begin{picture}(#1,700)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(#1,700){\line(-1,0){#1}}%
\put(0,700){\whead}
\end{picture}}%

% \ADJDIST{n} draws a pair of adjoint distibutors of length n units
\newcommand{\ADJDIST}[1]%
{\begin{picture}(#1,700)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(#1,700){\line(-1,0){#1}}%
\put(0,700){\whead}
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{400}}%
\put(\NUMBER,700){\circle{400}}%
\end{picture}}%


% All the following commands produce arrows with length 20pt
% and scriptstyle names in math mode but arrows with length
% \displayarrowlength pt and textstyle names in display math mode.

% arrow
\newcommand{\ar}{\ifinner\tcase{\AR}\else\dcase{\AR}\fi}%

% arrow with upper name [1]
\newcommand{\Ar}[1]{\ifinner\Tcase{\AR}{#1}\else\Dcase{\AR}{#1}\fi}%

% distributor
\newcommand{\dist}{\ifinner\tcase{\DIST}\else\dcase{\DIST}\fi}%

% distributor with upper name [1]
\newcommand{\Dist}[1]{\ifinner\Tcase{\DIST}{\TUP{#1}}%
\else\Dcase{\DIST}{\TUP{#1}}\fi}%

% dotted arrow
\newcommand{\dotar}{\ifinner\tcase{\DOTAR}\else\dcase{\DOTAR}\fi}%

% dotted arrow with upper name [1]
\newcommand{\Dotar}[1]{\ifinner\Tcase{\DOTAR}{#1}%
\else\Dcase{\DOTAR}{#1}\fi}%

% monomorphism
\newcommand{\mono}{\ifinner\tcase{\MONO}\else\dcase{\MONO}\fi}%

% monomorphism with upper name [1]
\newcommand{\Mono}[1]{\ifinner\Tcase{\MONO}{#1}\else\Dcase{\MONO}{#1}\fi}%

% epimorphism
\newcommand{\epi}{\ifinner\tcase{\EPI}\else\dcase{\EPI}\fi}%

% epimorphism with upper name [1]
\newcommand{\Epi}[1]{\ifinner\Tcase{\EPI}{#1}\else\Dcase{\EPI}{#1}\fi}%

% bimorphism
\newcommand{\bimo}{\ifinner\tcase{\BIMO}\else\dcase{\BIMO}\fi}%

% bimorphism with upper name [1]
\newcommand{\Bimo}[1]{\ifinner\Tcase{\BIMO}{#1}%
\else\Dcase{\BIMO}{#1}\fi}%

% isomorphism
\newcommand{\iso}{\ifinner\Tcase{\AR}{\cong}\else\Dcase{\AR}{\cong}\fi}%

% isomorphism with upper name [1]
\newcommand{\Iso}[1]{\ifinner\Tcase{\AR}{\cong{#1}}%
\else\Dcase{\AR}{\cong{#1}}\fi}%

% pair of arrows
\newcommand{\biar}{\ifinner\tbicase{\BIAR}\else\dbicase{\BIAR}\fi}%

% pair of arrows with names [1],[2]
\newcommand{\Biar}[2]{\ifinner\Tbicase{\BIAR}{#1}{#2}%
\else\Dbicase{\BIAR}{#1}{#2}\fi}%

% pair of distributors
\newcommand{\bidist}{\ifinner\tbicase{\BIDIST}\else\dbicase{\BIDIST}\fi}%

% pair of distributors with names [1],[2]
\newcommand{\Bidist}[2]{\ifinner\Tbicase{\BIDIST}{\TUP{#1}}{\TDOWN{#2}}%
\else\Dbicase{\BIDIST}{\DUP{#1}}{\DDOWN{#2}}\fi}%

% equality
\newcommand{\eql}{\ifinner\tcase{\EQL}\else\dcase{\EQL}\fi}%

% equality with name [1]
\newcommand{\Eql}[1]{\ifinner\Tcase{\EQL}{\TUP{#1}}%
\else\Dcase{\EQL}{\DUP{#1}}\fi}%

% pair of adjoint arrows
\newcommand{\adjar}{\ifinner\tbicase{\ADJAR}\else\dbicase{\ADJAR}\fi}%

% pair of adjoint arrows with names [1],[2]
\newcommand{\Adjar}[2]{\ifinner\Tbicase{\ADJAR}{#1}{#2}%
\else\Dbicase{\ADJAR}{#1}{#2}\fi}%

% pair of adjoint distributors
\newcommand{\adjdist}{\ifinner\tbicase{\ADJDIST}\else\dbicase{\ADJDIST}\fi}%

% pair of adjoint distributors with names [1],[2]
\newcommand{\Adjdist}[2]{\ifinner\Tbicase{\ADJDIST}{\TUP{#1}}{\TDOWN{#2}}%
\else\Dbicase{\ADJDIST}{\DUP{#1}}{\DDOWN{#2}}\fi}%


% IN-TEXT BACK ARROWS

% \BKAR{n} draws a pointing back arrow of length n units
\newcommand{\BKAR}[1]%
{\begin{picture}(#1,0)%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\end{picture}}%

% \BKDIST{n} draws a pointing back distributor of length n units
\newcommand{\BKDIST}[1]%
{\begin{picture}(#1,0)%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{400}}%
\end{picture}}%

% \BKDOTAR{n} draws a backward dotted  arrow
% of length n units
\newcommand{\BKDOTAR}[1]%
{\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by 300%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(#1,0)%
\multiput(#1,0)(-300,0){\NUMBEROFDOTS}{\circle*{100}}%
\put(0,0){\whead}%
\end{picture}}%

% \BKMONO{n} draws a pointing back monomorphism of length n units
\newcommand{\BKMONO}[1]%
{\monolength=#1%
\advance\monolength by -\monotail%
\begin{picture}(#1,0)(-#1,0)%
\put(-\monotail,0){\line(-1,0){\monolength}}%
\put(-\monotail,0){\whead}%
\put(-#1,0){\whead}%
\end{picture}}%

% \BKEPI{n} draws a pointing back epimorphism of length n units
\newcommand{\BKEPI}[1]%
{\epilength=#1%
\advance\epilength by -\epihead%
\begin{picture}(#1,0)%
\put(#1,0){\line(-1,0){\epilength}}%
\put(\epihead,0){\whead}%
\put(0,0){\whead}%
\end{picture}}%

% \BKBIMO{n} draws a pointing back bimorphism of length n units
\newcommand{\BKBIMO}[1]%
{\monolength=#1%
\advance\monolength by -\monotail%
\epilength=\monolength%
\advance\epilength by -\epihead%
\begin{picture}(#1,0)%
\put(\monolength,0){\line(-1,0){\epilength}}%
\put(\monolength,0){\whead}%
\put(\epihead,0){\whead}%
\put(0,0){\whead}%
\end{picture}}%

% \BKBIAR{n} draws a pair of pointing back arrows of length n units
\newcommand{\BKBIAR}[1]%
{\begin{picture}(#1,700)%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\put(#1,700){\line(-1,0){#1}}%
\put(0,700){\whead}%
\end{picture}}%

% \BKBIDIST{n} draws a pair of pointing back distributors of length n units
\newcommand{\BKBIDIST}[1]%
{\begin{picture}(#1,700)%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\put(#1,700){\line(-1,0){#1}}%
\put(0,700){\whead}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{400}}%
\put(\NUMBER,700){\circle{400}}%
\end{picture}}%

% \BKADJAR{n} draws a pair of adjoint arrows of length n units
\newcommand{\BKADJAR}[1]%
{\begin{picture}(#1,700)%
\put(0,700){\line(1,0){#1}}%
\put(#1,700){\ehead}%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\end{picture}}%

% \BKADJDIST{n} draws a pair of adjoint distributors of length n units
\newcommand{\BKADJDIST}[1]%
{\begin{picture}(#1,700)%
\put(0,700){\line(1,0){#1}}%
\put(#1,700){\ehead}%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{400}}%
\put(\NUMBER,700){\circle{400}}%
\end{picture}}%

% All the following commands produce back arrows with length 20pt
% and scriptstyle names in math mode but arrows with length
% \displayarrowlength and textstyle names in display math mode.

% back arrow
\newcommand{\bkar}{\ifinner\tcase{\BKAR}\else\dcase{\BKAR}\fi}%

% back arrow with upper name [1]
\newcommand{\Bkar}[1]{\ifinner\Tcase{\BKAR}{#1}\else\Dcase{\BKAR}{#1}\fi}%

% back distributor
\newcommand{\bkdist}{\ifinner\tcase{\BKDIST}\else\dcase{\BKDIST}\fi}%

% back distributor with upper name [1]
\newcommand{\Bkdist}[1]{\ifinner\Tcase{\BKDIST}{\TUP{#1}}%
\else\Dcase{\BKDIST}{\TUP{#1}}\fi}%

% backward dotted arrow
\newcommand{\bkdotar}{\ifinner\tcase{\BKDOTAR}\else\dcase{\BKDOTAR}\fi}%

% backward dotted arrow with upper name [1]
\newcommand{\Bkdotar}[1]{\ifinner\Tcase{\BKDOTAR}{#1}%
\else\Dcase{\BKDOTAR}{#1}\fi}%

% back monomorphism
\newcommand{\bkmono}{\ifinner\tcase{\BKMONO}\else\dcase{\BKMONO}\fi}%

% back monomorphism with upper name [1]
\newcommand{\Bkmono}[1]{\ifinner\Tcase{\BKMONO}{#1}%
\else\Dcase{\BKMONO}{#1}\fi}%

% back epimorphism
\newcommand{\bkepi}{\ifinner\tcase{\BKEPI}\else\dcase{\BKEPI}\fi}%

% back epimorphism with upper name [1]
\newcommand{\Bkepi}[1]{\ifinner\Tcase{\BKEPI}{#1}%
\else\Dcase{\BKEPI}{#1}\fi}%

% back bimorphism
\newcommand{\bkbimo}{\ifinner\tcase{\BKBIMO}\else\dcase{\BKBIMO}\fi}%

% back bimorphism with upper name [1]
\newcommand{\Bkbimo}[1]{\ifinner\Tcase{\BKBIMO}{\hspace{9pt}#1}%
\else\Dcase{\BKBIMO}{\hspace{9pt}#1}\fi}%

% back isomorphism
\newcommand{\bkiso}{\ifinner\Tcase{\BKAR}{\cong}%
\else\Dcase{\BKAR}{\cong}\fi}%

% back isomorphism with upper name [1]
\newcommand{\Bkiso}[1]{\ifinner\Tcase{\BKAR}{\cong{#1}}%
\else\Dcase{\BKAR}{\cong{#1}}\fi}%

% pair of back arrows
\newcommand{\bkbiar}{\ifinner\tbicase{\BKBIAR}\else\dbicase{\BKBIAR}\fi}%

% pair of back arrows with names [1],[2]
\newcommand{\Bkbiar}[2]{\ifinner\Tbicase{\BKBIAR}{#1}{#2}%
\else\Dbicase{\BKBIAR}{#1}{#2}\fi}%

% pair of back distributors
\newcommand{\bkbidist}{\ifinner\tbicase{\BKBIDIST}%
\else\dbicase{\BKBIDIST}\fi}%

% pair of back distributors with names [1],[2]
\newcommand{\Bkbidist}[2]{\ifinner\Tbicase{\BKBIDIST}{\TUP{#1}}{\TDOWN{#2}}%
\else\Tbicase{\BKBIDIST}{\DUP{#1}}{\DDOWN{#2}}\fi}%

% back equality
\let\bkeql=\eql%

% back equality with name [1]
\let\Bkeql=\Eql%

% back pair of adjoint arrows
\newcommand{\bkadjar}{\ifinner\tbicase{\BKADJAR}%
\else\dbicase{\BKADJAR}\fi}%

% back pair of adjoint arrows with names [1],[2]
\newcommand{\Bkadjar}[2]{\ifinner\Tbicase{\BKADJAR}{#1}{#2}%
\else\Dbicase{\BKADJAR}{#1}{#2}\fi}%

% back pair of adjoint distributors
\newcommand{\bkadjdist}{\ifinner\tbicase{\BKADJDIST}%
\else\dbicase{\BKADJDIST}\fi}%

% back pair of adjoint distributors with names [1],[2]
\newcommand{\Bkadjdist}[2]{\ifinner\Tbicase{\BKADJDIST}{\TUP{#1}}{\TDOWN{#2}}%
\else\Dbicase{\BKADJDIST}{\TUP{#1}}{\TDOWN{#2}}\fi}%


% MACROS FOR DRAWING HORIZONTAL PICTURES

% \lowername{P}{f} puts the name f under the picture P
%\newcommand{\lowername}[2]%
%{$\stackrel{\makebox[1pt]{#1}}%
%{\begin{picture}(0,0)%
%\truex{600}%
%\put(0,0){\makebox(0,\value{x})[t]{\makebox[1pt]{$#2$}}}%
%\end{picture}}$}%

% My correction of the previous command
\newcommand{\lowername}[2]%
{$\stackrel{\makebox[1pt]{#1}}%
{\begin{picture}(0,0)%
\truex{600}%
\put(0,-600){\makebox(0,\value{x})[t]{\makebox[1pt]{$#2$}}}%
%\put(0,0){\makebox(0,\value{x})[t]{\makebox[1pt]{$#2$}}}%
\end{picture}}$}%

% \hcase{P}{n} draws the picture P with length n units
\newcommand{\hcase}[2]%
{\testdiagrammode\makebox[0pt]%
{\raisebox{0pt}[0pt][0pt]{#1{#2}}}}%

% \Hcase{P}{f}{n} draws the picture P with upper name f
% and length n units.
\newcommand{\Hcase}[3]%
{\testdiagrammode\makebox[0pt]
{\raisebox{0pt}[0pt][0pt]%
{$\stackrel{\makebox[0pt]{$\textstyle{#2}$}}{#1{#3}}$}}}%

% \hcasE{P}{f}{n} draws the picture P with lower name f
% and length n units.
%\newcommand{\hcasE}[3]%
%{\testdiagrammode\makebox[0pt]%
%{\raisebox{-8pt}[0pt][0pt]%
%{\lowername{#1{#3}}{#2}}}}%

% My correction of the previous command
\newcommand{\hcasE}[3]%
{\testdiagrammode\makebox[0pt]%
{\raisebox{-3pt}[0pt][0pt]%
{\lowername{#1{#3}}{#2}}}}%

% \Hisocase{P}{f}{g}{n} draws an arrow P with names f, g
% and length n units.
\newcommand{\Hisocase}[4]%
{\testdiagrammode\makebox[0pt]
{\raisebox{-8pt}[0pt][0pt]%
{$\stackrel{\makebox[0pt]{$\textstyle{#2}$}}%
{\mbox{\lowername{#1{#4}}{#3}}}$}}}%

% \hbicase{P}{n} draws the bi-picture P with length n units.
\newcommand{\hbicase}[2]%
{\testdiagrammode\makebox[0pt]%
{\raisebox{-2.4pt}[0pt][0pt]{#1{#2}}}}%

% \Hbicase{P}{f}{g}{n} draws the bi-picture P with names f, g
% and length n units.
\newcommand{\Hbicase}[4]%
{\testdiagrammode\makebox[0pt]
{\raisebox{-10.4pt}[0pt][0pt]%
{$\stackrel{\makebox[0pt]{$\textstyle{#2}$}}%
{\mbox{\lowername{#1{#4}}{#3}}}$}}}%

% EAST ARROWS

% \EAR{n} draws an east arrow of length n units
\newcommand{\EAR}[1]%
{\begin{picture}(#1,0)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\end{picture}}%

% \EDIST{n} draws an east distributor of length n units
\newcommand{\EDIST}[1]%
{\begin{picture}(#1,0)%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\truex{400}
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{\value{x}}}
\end{picture}}%

% \EDOTAR draws a dotted arrow of length n units
\newcommand{\EDOTAR}[1]%
{\truex{100}\truey{300}%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(#1,0)%
\multiput(0,0)(\value{y},0){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(#1,0){\ehead}%
\end{picture}}%


% \EMONO{n} draws an east monomorphism of length n units
\newcommand{\EMONO}[1]%
{\truetail
\monolength=#1%
\advance\monolength by -\truemonotail%
\begin{picture}(#1,0)%
\put(\truemonotail,0){\line(1,0){\monolength}}%
\put(#1,0){\ehead}%
\put(\truemonotail,0){\ehead}%
\end{picture}}%


% \EEPI{n} draws an east epimorphism of length n units
\newcommand{\EEPI}[1]%
{\truehead%
\epilength=#1%
\advance\epilength by -\trueepihead%
\begin{picture}(#1,0)(-#1,0)%
\put(-#1,0){\line(1,0){\epilength}}%
\put(-\trueepihead,0){\ehead}%
\put(0,0){\ehead}%
\end{picture}}%


% \EBIMO{n} draws an east bimorphism of length n units
\newcommand{\EBIMO}[1]%
{\truehead\truetail%
\monolength=#1%
\advance\monolength by -\truemonotail%
\epilength=\monolength%
\advance\epilength by -\trueepihead%
\begin{picture}(#1,0)(-#1,0)%
\put(-\monolength,0){\line(1,0){\epilength}}%
\put(-\monolength,0){\ehead}%
\put(-\trueepihead,0){\ehead}%
\put(0,0){\ehead}%
\end{picture}}%


% \EBIAR{n} draws an east pair of arrows of length n units
\newcommand{\EBIAR}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(0,\value{x}){\line(1,0){#1}}%
\put(#1,\value{x}){\ehead}%
\end{picture}}%

% \EBIDIST{n} draws an east pair of distributors of length n units
\newcommand{\EBIDIST}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(0,\value{x}){\line(1,0){#1}}%
\put(#1,\value{x}){\ehead}%
\truey{400}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{\value{y}}}
\put(\NUMBER,\value{x}){\circle{\value{y}}}%
\end{picture}}%

% \EEQL{n} draws an east equality of length n units
\newcommand{\EEQL}[1]%
{\begin{picture}(#1,0)%
\truex{200}%
\put(0,\value{x}){\line(1,0){#1}}%
\put(0,0){\line(1,0){#1}}%
\end{picture}}%

% \EADJAR{n} draws an east pair of adjoint arrows of length n
% units
\newcommand{\EADJAR}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(#1,\value{x}){\line(-1,0){#1}}%
\put(0,\value{x}){\whead}%
\end{picture}}%

% \EADJDIST{n} draws an east pair of adjoint distributors of length n
% units
\newcommand{\EADJDIST}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(0,0){\line(1,0){#1}}%
\put(#1,0){\ehead}%
\put(#1,\value{x}){\line(-1,0){#1}}%
\put(0,\value{x}){\whead}%
\truey{400}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{\value{y}}}
\put(\NUMBER,\value{x}){\circle{\value{y}}}%
\end{picture}}%


% All the following commands produce east arrows

% basic east arrow
\def\basicear[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EAR}{\Z}}%

% east arrow
\newcommand{\ear}{\@ifnextchar[{\basicear}%
{\hspace{\SOURCE\unitlength}\basicear[\ARROWLENGTH]}}%

% basic east arrow with upper name
\def\basicEar[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EAR}{#2}{\Z}}%

% east arrow with upper name
\newcommand{\Ear}{\@ifnextchar[{\basicEar}%
{\hspace{\SOURCE\unitlength}\basicEar[\ARROWLENGTH]}}%

% basic east arrow with lower name
\def\basiceaR[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EAR}{#2}{\Z}}%

% east arrow with lower name
\newcommand{\eaR}{\@ifnextchar[{\basiceaR}%
{\hspace{\SOURCE\unitlength}\basiceaR[\ARROWLENGTH]}}%

% basic east distributor
\def\basicedist[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EDIST}{\Z}}%

% east distributor
\newcommand{\edist}{\@ifnextchar[{\basicedist}%
{\hspace{\SOURCE\unitlength}\basicedist[\ARROWLENGTH]}}%

% basic east distributor with upper name
\def\basicEdist[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EDIST}{\DUP{#2}}{\Z}}%

% east distributor with upper name
\newcommand{\Edist}{\@ifnextchar[{\basicEdist}%
{\hspace{\SOURCE\unitlength}\basicEdist[\ARROWLENGTH]}}%

% basic east distributor with lower name
\def\basicedisT[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EDIST}{\DDOWN{#2}}{\Z}}%

% east distributor with lower name
\newcommand{\edisT}{\@ifnextchar[{\basicedisT}%
{\hspace{\SOURCE\unitlength}\basicedisT[\ARROWLENGTH]}}%

% basic east dotted arrow
\def\basicedotar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EDOTAR}{\Z}}%

% east dotted arrow
\newcommand{\edotar}{\@ifnextchar[{\basicedotar}%
{\hspace{\SOURCE\unitlength}\basicedotar[\ARROWLENGTH]}}%

% basic east dotted arrow with upper name
\def\basicEdotar[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EDOTAR}{#2}{\Z}}%

% east dotted arrow with upper name
\newcommand{\Edotar}{\@ifnextchar[{\basicEdotar}%
{\hspace{\SOURCE\unitlength}\basicEdotar[\ARROWLENGTH]}}%

% basic east dotted arrow with lower name
\def\basicedotaR[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EDOTAR}{#2}{\Z}}%

% east dotted arrow with lower name
\newcommand{\edotaR}{\@ifnextchar[{\basicedotaR}%
{\hspace{\SOURCE\unitlength}\basicedotaR[\ARROWLENGTH]}}%

% basic east monomorphism
\def\basicemono[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EMONO}{\Z}}%

% east arrow
\newcommand{\emono}{\@ifnextchar[{\basicemono}%
{\hspace{\SOURCE\unitlength}\basicemono[\ARROWLENGTH]}}%

% basic east monomorphism with upper name
\def\basicEmono[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EMONO}{#2}{\Z}}%

% east monomorphism with upper name
\newcommand{\Emono}{\@ifnextchar[{\basicEmono}%
{\hspace{\SOURCE\unitlength}\basicEmono[\ARROWLENGTH]}}%

% basic east monomorphism with lower name
\def\basicemonO[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EMONO}{#2}{\Z}}%

% east monomorphism with lower name
\newcommand{\emonO}{\@ifnextchar[{\basicemonO}%
{\hspace{\SOURCE\unitlength}\basicemonO[\ARROWLENGTH]}}%

% basic east epimorphism
\def\basiceepi[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EEPI}{\Z}}%

% east epimorphism
\newcommand{\eepi}{\@ifnextchar[{\basiceepi}%
{\hspace{\SOURCE\unitlength}\basiceepi[\ARROWLENGTH]}}%

% basic east epimorphism with upper name
\def\basicEepi[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EEPI}{#2}{\Z}}%

% east epimorphism with upper name
\newcommand{\Eepi}{\@ifnextchar[{\basicEepi}%
{\hspace{\SOURCE\unitlength}\basicEepi[\ARROWLENGTH]}}%

% basic east epimorphism with lower name
\def\basiceepI[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EEPI}{#2}{\Z}}%

% east epimorphism with lower name
\newcommand{\eepI}{\@ifnextchar[{\basiceepI}%
{\hspace{\SOURCE\unitlength}\basiceepI[\ARROWLENGTH]}}%

% basic east bimorphism
\def\basicebimo[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EBIMO}{\Z}}%

% east bimorphism
\newcommand{\ebimo}{\@ifnextchar[{\basicebimo}%
{\hspace{\SOURCE\unitlength}\basicebimo[\ARROWLENGTH]}}%

% basic east bimorphism with upper name
\def\basicEbimo[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EBIMO}{#2}{\Z}}%

% east bimorphism with upper name
\newcommand{\Ebimo}{\@ifnextchar[{\basicEbimo}%
{\hspace{\SOURCE\unitlength}\basicEbimo[\ARROWLENGTH]}}%

% basic east bimorphism with lower name
\def\basicebimO[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EBIMO}{#2}{\Z}}%

% east bimorphism with lower name
\newcommand{\ebimO}{\@ifnextchar[{\basicebimO}%
{\hspace{\SOURCE\unitlength}\basicebimO[\ARROWLENGTH]}}%

% basic east isomorphism
\def\basiceiso[#1]{%
\Z=#1%
\multiply \Z by 100%
\Hisocase{\EAR}{\cong}{}{\Z}}%

% east isomorphism
\newcommand{\eiso}{\@ifnextchar[{\basiceiso}%
{\hspace{\SOURCE\unitlength}\basiceiso[\ARROWLENGTH]}}%

% basic east isomorphism with upper name
\def\basicEiso[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hisocase{\EAR}{#2}{\cong}{\Z}}%

% east isomorphism with upper name
\newcommand{\Eiso}{\@ifnextchar[{\basicEiso}%
{\hspace{\SOURCE\unitlength}\basicEiso[\ARROWLENGTH]}}%

% basic east isomorphism with lower name
\def\basiceisO[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hisocase{\EAR}{\cong}{#2}{\Z}}%

% east isomorphism with lower name
\newcommand{\eisO}{\@ifnextchar[{\basiceisO}%
{\hspace{\SOURCE\unitlength}\basiceisO[\ARROWLENGTH]}}%

% basic east equality
\def\basiceeql[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\EEQL}{\Z}}%

% east equality
\newcommand{\eeql}{\@ifnextchar[{\basiceeql}%
{\hspace{\SOURCE\unitlength}\basiceeql[\ARROWLENGTH]}}%

% basic east equality with upper name
\def\basicEeql[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\EEQL}{\DUP{#2}}{\Z}}%

% east equality with upper name
\newcommand{\Eeql}{\@ifnextchar[{\basicEeql}%
{\hspace{\SOURCE\unitlength}\basicEeql[\ARROWLENGTH]}}%

% basic east equality with lower name
\def\basiceeqL[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\EEQL}{#2}{\Z}}%

% east equality with lower name
\newcommand{\eeqL}{\@ifnextchar[{\basiceeqL}%
{\hspace{\SOURCE\unitlength}\basiceeqL[\ARROWLENGTH]}}%

% basic pair of east arrows
\def\basicebiar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\EBIAR}{\Z}}%

% pair of east arrows
\newcommand{\ebiar}{\@ifnextchar[{\basicebiar}%
{\hspace{\SOURCE\unitlength}\basicebiar[\ARROWLENGTH]}}%

% basic pair of east arrows with names
\def\basicEbiar[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\EBIAR}{#2}{#3}{\Z}}%

% pair of east arrows with names
\newcommand{\Ebiar}{\@ifnextchar[{\basicEbiar}%
{\hspace{\SOURCE\unitlength}\basicEbiar[\ARROWLENGTH]}}%
\let\ebiaR=\Ebiar

% basic pair of east distributors
\def\basicebidist[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\EBIDIST}{\Z}}%

% pair of east distributors
\newcommand{\ebidist}{\@ifnextchar[{\basicebidist}%
{\hspace{\SOURCE\unitlength}\basicebidist[\ARROWLENGTH]}}%

% basic pair of east distributors with names
\def\basicEbidist[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\EBIDIST}{\DUP{#2}}{\DDOWN{#3}}{\Z}}%

% pair of east distributors with names
\newcommand{\Ebidist}{\@ifnextchar[{\basicEbidist}%
{\hspace{\SOURCE\unitlength}\basicEbidist[\ARROWLENGTH]}}%
\let\ebidisT=\Ebidist

% basic pair of east adjoint arrows
\def\basiceadjar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\EADJAR}{\Z}}%

% pair of east adjoint arrows
\newcommand{\eadjar}{\@ifnextchar[{\basiceadjar}%
{\hspace{\SOURCE\unitlength}\basiceadjar[\ARROWLENGTH]}}%

% basic pair of east adjoint arrows with names
\def\basicEadjar[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\EADJAR}{#2}{#3}{\Z}}%

% pair of east adjoint arrows with names
\newcommand{\Eadjar}{\@ifnextchar[{\basicEadjar}%
{\hspace{\SOURCE\unitlength}\basicEadjar[\ARROWLENGTH]}}%
\let\eadjaR=\Eadjar

% basic pair of east adjoint distributors
\def\basiceadjdist[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\EADJDIST}{\Z}}%

% pair of east adjoint distributors
\newcommand{\eadjdist}{\@ifnextchar[{\basiceadjdist}%
{\hspace{\SOURCE\unitlength}\basiceadjdist[\ARROWLENGTH]}}%

% basic pair of east adjoint distributors with names
\def\basicEadjdist[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\EADJDIST}{\DUP{#2}}{\DDOWN{#3}}{\Z}}%

% pair of east adjoint distributors with names
\newcommand{\Eadjdist}{\@ifnextchar[{\basicEadjdist}%
{\hspace{\SOURCE\unitlength}\basicEadjdist[\ARROWLENGTH]}}%
\let\eadjdisT=\Eadjdist

% WEST ARROWS

% \WAR{n} draws a pointing back arrow of length n units
\newcommand{\WAR}[1]%
{\begin{picture}(#1,0)%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\end{picture}}%

% \WDIST{n} draws a pointing back distributor of length n units
\newcommand{\WDIST}[1]%
{\begin{picture}(#1,0)%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\truex{400}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{\value{x}}}%
\end{picture}}%

% \WDOTAR draws a dotted arrow of length n units
\newcommand{\WDOTAR}[1]%
{\truex{100}\truey{300}%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(#1,0)%
\multiput(#1,0)(-\value{y},0){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(0,0){\whead}%
\end{picture}}%

% \WMONO{n} draws a pointing back monomorphism of length n units
\newcommand{\WMONO}[1]%
{\truetail%
\monolength=#1%
\advance\monolength by -\truemonotail%
\begin{picture}(#1,0)(-#1,0)%
\put(-\truemonotail,0){\line(-1,0){\monolength}}%
\put(-\truemonotail,0){\whead}%
\put(-#1,0){\whead}%
\end{picture}}%


% \WEPI{n} draws a pointing back epimorphism of length n units
\newcommand{\WEPI}[1]%
{\truehead%
\epilength=#1%
\advance\epilength by -\trueepihead%
\begin{picture}(#1,0)%
\put(#1,0){\line(-1,0){\epilength}}%
\put(\trueepihead,0){\whead}%
\put(0,0){\whead}%
\end{picture}}%

% \WBIMO{n} draws a pointing back bimorphism of length n units
\newcommand{\WBIMO}[1]%
{\truehead\truetail%
\monolength=#1
\advance\monolength by -\truemonotail%
\epilength=\monolength%
\advance\epilength by -\trueepihead%
\begin{picture}(#1,0)%
\put(\monolength,0){\line(-1,0){\epilength}}%
\put(\monolength,0){\whead}%
\put(\trueepihead,0){\whead}%
\put(0,0){\whead}%
\end{picture}}%

% \WBIAR{n} draws a pair of pointing back arrows of length n units
\newcommand{\WBIAR}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\put(#1,\value{x}){\line(-1,0){#1}}%
\put(0,\value{x}){\whead}%
\end{picture}}%

% \WBIDIST{n} draws a pair of pointing back distributors of length n units
\newcommand{\WBIDIST}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\put(#1,\value{x}){\line(-1,0){#1}}%
\put(0,\value{x}){\whead}%
\truey{400}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{\value{y}}}%
\put(\NUMBER,\value{x}){\circle{\value{y}}}%
\end{picture}}%

% \WADJAR{n} draws a pair of adjoint arrows of length n units
\newcommand{\WADJAR}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(0,\value{x}){\line(1,0){#1}}%
\put(#1,\value{x}){\ehead}%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\end{picture}}%

% \WADJDIST{n} draws a pair of adjoint distributors of length n units
\newcommand{\WADJDIST}[1]%
{\truex{700}%
\begin{picture}(#1,\value{x})%
\put(0,\value{x}){\line(1,0){#1}}%
\put(#1,\value{x}){\ehead}%
\put(#1,0){\line(-1,0){#1}}%
\put(0,0){\whead}%
\truey{400}%
\NUMBER=#1%
\divide\NUMBER by 2%
\put(\NUMBER,0){\circle{\value{y}}}%
\put(\NUMBER,\value{x}){\circle{\value{y}}}%
\end{picture}}%


% All the following commands produce west arrows

% basic west arrow
\def\basicwar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\WAR}{\Z}}%

% west arrow
\newcommand{\war}{\@ifnextchar[{\basicwar}%
{\hspace{\SOURCE\unitlength}\basicwar[\ARROWLENGTH]}}%

% basic west arrow with upper name
\def\basicWar[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\WAR}{#2}{\Z}}%

% west arrow with upper name
\newcommand{\War}{\@ifnextchar[{\basicWar}%
{\hspace{\SOURCE\unitlength}\basicWar[\ARROWLENGTH]}}%

% basic west arrow with lower name
\def\basicwaR[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\WAR}{#2}{\Z}}%

% west arrow with lower name
\newcommand{\waR}{\@ifnextchar[{\basicwaR}%
{\hspace{\SOURCE\unitlength}\basicwaR[\ARROWLENGTH]}}%

% basic west distributor
\def\basicwdist[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\WDIST}{\Z}}%

% west distributor
\newcommand{\wdist}{\@ifnextchar[{\basicwdist}%
{\hspace{\SOURCE\unitlength}\basicwdist[\ARROWLENGTH]}}%

% basic west distributor with upper name
\def\basicWdist[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\WDIST}{\DUP{#2}}{\Z}}%

% west distributor with upper name
\newcommand{\Wdist}{\@ifnextchar[{\basicWdist}%
{\hspace{\SOURCE\unitlength}\basicWdist[\ARROWLENGTH]}}%

% basic west distributor with lower name
\def\basicwdisT[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\WDIST}{\DDOWN{#2}}{\Z}}%

% west distributor with lower name
\newcommand{\wdisT}{\@ifnextchar[{\basicwdisT}%
{\hspace{\SOURCE\unitlength}\basicwdisT[\ARROWLENGTH]}}%

% basic west dotted arrow
\def\basicwdotar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\WDOTAR}{\Z}}%

% west dotted arrow
\newcommand{\wdotar}{\@ifnextchar[{\basicwdotar}%
{\hspace{\SOURCE\unitlength}\basicwdotar[\ARROWLENGTH]}}%

% basic west dotted arrow with upper name
\def\basicWdotar[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\WDOTAR}{#2}{\Z}}%

% west dotted arrow with upper name
\newcommand{\Wdotar}{\@ifnextchar[{\basicWdotar}%
{\hspace{\SOURCE\unitlength}\basicWdotar[\ARROWLENGTH]}}%

% basic west dotted arrow with lower name
\def\basicwdotaR[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\WDOTAR}{#2}{\Z}}%

% west dotted arrow with lower name
\newcommand{\wdotaR}{\@ifnextchar[{\basicwdotaR}%
{\hspace{\SOURCE\unitlength}\basicwdotaR[\ARROWLENGTH]}}%

% basic west monomorphism
\def\basicwmono[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\WMONO}{\Z}}%

% west arrow
\newcommand{\wmono}{\@ifnextchar[{\basicwmono}%
{\hspace{\SOURCE\unitlength}\basicwmono[\ARROWLENGTH]}}%

% basic west monomorphism with upper name
\def\basicWmono[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\WMONO}{#2}{\Z}}%

% west monomorphism with upper name
\newcommand{\Wmono}{\@ifnextchar[{\basicWmono}%
{\hspace{\SOURCE\unitlength}\basicWmono[\ARROWLENGTH]}}%

% basic west monomorphism with lower name
\def\basicwmonO[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\WMONO}{#2}{\Z}}%

% west monomorphism with lower name
\newcommand{\wmonO}{\@ifnextchar[{\basicwmonO}%
{\hspace{\SOURCE\unitlength}\basicwmonO[\ARROWLENGTH]}}%

% basic west epimorphism
\def\basicwepi[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\WEPI}{\Z}}%

% west epimorphism
\newcommand{\wepi}{\@ifnextchar[{\basicwepi}%
{\hspace{\SOURCE\unitlength}\basicwepi[\ARROWLENGTH]}}%

% basic west epimorphism with upper name
\def\basicWepi[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\WEPI}{#2}{\Z}}%

% west epimorphism with upper name
\newcommand{\Wepi}{\@ifnextchar[{\basicWepi}%
{\hspace{\SOURCE\unitlength}\basicWepi[\ARROWLENGTH]}}%

% basic west epimorphism with lower name
\def\basicwepI[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\WEPI}{#2}{\Z}}%

% west epimorphism with lower name
\newcommand{\wepI}{\@ifnextchar[{\basicwepI}%
{\hspace{\SOURCE\unitlength}\basicwepI[\ARROWLENGTH]}}%

% basic west bimorphism
\def\basicwbimo[#1]{%
\Z=#1%
\multiply \Z by 100%
\hcase{\WBIMO}{\Z}}%

% west bimorphism
\newcommand{\wbimo}{\@ifnextchar[{\basicwbimo}%
{\hspace{\SOURCE\unitlength}\basicwbimo[\ARROWLENGTH]}}%

% basic west bimorphism with upper name
\def\basicWbimo[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hcase{\WBIMO}{#2}{\Z}}%

% west bimorphism with upper name
\newcommand{\Wbimo}{\@ifnextchar[{\basicWbimo}%
{\hspace{\SOURCE\unitlength}\basicWbimo[\ARROWLENGTH]}}%

% basic west bimorphism with lower name
\def\basicwbimO[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\hcasE{\WBIMO}{#2}{\Z}}%

% west bimorphism with lower name
\newcommand{\wbimO}{\@ifnextchar[{\basicwbimO}%
{\hspace{\SOURCE\unitlength}\basicwbimO[\ARROWLENGTH]}}%

% basic west isomorphism
\def\basicwiso[#1]{%
\Z=#1%
\multiply \Z by 100%
\Hisocase{\WAR}{\cong}{}{\Z}}%

% west isomorphism
\newcommand{\wiso}{\@ifnextchar[{\basicwiso}%
{\hspace{\SOURCE\unitlength}\basicwiso[\ARROWLENGTH]}}%

% basic west isomorphism with upper name
\def\basicWiso[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hisocase{\WAR}{#2}{\cong}{\Z}}%

% west isomorphism with upper name
\newcommand{\Wiso}{\@ifnextchar[{\basicWiso}%
{\hspace{\SOURCE\unitlength}\basicWiso[\ARROWLENGTH]}}%

% basic west isomorphism with lower name
\def\basicwisO[#1]#2{%
\Z=#1%
\multiply \Z by 100%
\Hisocase{\WAR}{\cong}{#2}{\Z}}%

% west isomorphism with lower name
\newcommand{\wisO}{\@ifnextchar[{\basicwisO}%
{\hspace{\SOURCE\unitlength}\basicwisO[\ARROWLENGTH]}}%

% west equality
\let\weql=\eeql%

% west equality with upper name
\let\Weql=\Eeql%

% west equality with lower name
\let\weqL=\eeqL%

% basic pair of west arrows
\def\basicwbiar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\WBIAR}{\Z}}%

% pair of west arrows
\newcommand{\wbiar}{\@ifnextchar[{\basicwbiar}%
{\hspace{\SOURCE\unitlength}\basicwbiar[\ARROWLENGTH]}}%

% basic pair of west arrows with names
\def\basicWbiar[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\WBIAR}{#2}{#3}{\Z}}%

% pair of west arrows with names
\newcommand{\Wbiar}{\@ifnextchar[{\basicWbiar}%
{\hspace{\SOURCE\unitlength}\basicWbiar[\ARROWLENGTH]}}%
\let\wbiaR=\Wbiar

% basic pair of west distributors
\def\basicwbidist[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\WBIDIST}{\Z}}%

% pair of west distributors
\newcommand{\wbidist}{\@ifnextchar[{\basicwbidist}%
{\hspace{\SOURCE\unitlength}\basicwbidist[\ARROWLENGTH]}}%

% basic pair of west distributors with names
\def\basicWbidist[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\WBIDIST}{\DUP{#2}}{\DDOWN{#3}}{\Z}}%

% pair of west distributors with names
\newcommand{\Wbidist}{\@ifnextchar[{\basicWbidist}%
{\hspace{\SOURCE\unitlength}\basicWbidist[\ARROWLENGTH]}}%
\let\wbidisT=\Wbidist

% basic pair of west adjoint arrows
\def\basicwadjar[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\WADJAR}{\Z}}%

% pair of west adjoint arrows
\newcommand{\wadjar}{\@ifnextchar[{\basicwadjar}%
{\hspace{\SOURCE\unitlength}\basicwadjar[\ARROWLENGTH]}}%

% basic pair of west adjoint arrows with names
\def\basicWadjar[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\WADJAR}{#2}{#3}{\Z}}%

% pair of west adjoint arrows with names
\newcommand{\Wadjar}{\@ifnextchar[{\basicWadjar}%
{\hspace{\SOURCE\unitlength}\basicWadjar[\ARROWLENGTH]}}%
\let\wadjaR=\Wadjar

% basic pair of west adjoint distributors
\def\basicwadjdist[#1]{%
\Z=#1%
\multiply \Z by 100%
\hbicase{\WADJDIST}{\Z}}%

% pair of west adjoint distributors
\newcommand{\wadjdist}{\@ifnextchar[{\basicwadjdist}%
{\hspace{\SOURCE\unitlength}\basicwadjdist[\ARROWLENGTH]}}%

% basic pair of west adjoint distributors with names
\def\basicWadjdist[#1]#2#3{%
\Z=#1%
\multiply \Z by 100%
\Hbicase{\WADJDIST}{\DUP{#2}}{\DDOWN{#3}}{\Z}}%

% pair of west adjoint distributors with names
\newcommand{\Wadjdist}{\@ifnextchar[{\basicWadjdist}%
{\hspace{\SOURCE\unitlength}\basicWadjdist[\ARROWLENGTH]}}%
\let\wadjdisT=\Wadjdist


% MACROS FOR DRAWING VERTICAL PICTURES

% \vcase{P}{n} draws the vertical picture P with length n units.
\newcommand{\vcase}[2]{\testdiagrammode#1{#2}}%

% \Vcase{P}{f}{n} draws the vertical picture P
% with left name f and length n units.
\newcommand{\Vcase}[3]{\testdiagrammode\makebox[0pt]%
{\makebox[0pt][r]{\raisebox{0pt}[0pt][0pt]{${#2}\hspace{2pt}$}}}#1{#3}}%

% \vcasE{P}{f}{n} draws the vertical picture P
% with right name f and length n units.
\newcommand{\vcasE}[3]{\testdiagrammode\makebox[0pt]%
{#1{#3}\makebox[0pt][l]{\raisebox{0pt}[0pt][0pt]{\hspace{2pt}$#2$}}}}%

% \Visocase{P}{f}{g}{n} draws the vertical picture P
% with names f, g and length n units.
\newcommand{\Visocase}[4]{\testdiagrammode\makebox[0pt]%
{\makebox[0pt][r]{\raisebox{0pt}[0pt][0pt]{$#2$\hspace{2pt}}}#1{#4}%
\makebox[0pt][l]{\raisebox{0pt}[0pt][0pt]{\hspace{2pt}$#3$}}}}%

% \vbicase{P}{n} draws the vertical bi-picture P with length n units.
\newcommand{\vbicase}[2]{\testdiagrammode\makebox[0pt]{{#1{#2}}}}%

% \Vbicase{P}{f}{g}{n} draws the vertical bi-picture P
% with names f, g and length n units.
\newcommand{\Vbicase}[4]{\testdiagrammode\makebox[0pt]%
{\makebox[0pt][r]{\raisebox{0pt}[0pt][0pt]{$#2$\hspace{5.5pt}}}#1{#4}%
\makebox[0pt][l]{\raisebox{0pt}[0pt][0pt]{\hspace{6.5pt}$#3$}}}}%



% SOUTH ARROWS

% \SAR{n} draws a south arrow of length n units
% and centers it in a box of width  0pt and height 0pt
\newcommand{\SAR}[1]%
{\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,#1){\line(0,-1){#1}}%
\put(0,0){\shead}%
\end{picture}}}\end{picture}}%

% \SDIST{n} draws a south distributor of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SDIST}[1]%
{\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,#1){\line(0,-1){#1}}%
\put(0,0){\shead}%
\end{picture}}}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\end{picture}}%

% \SDOTAR{n} draws a south dotted arrow of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SDOTAR}[1]%
{\truex{100}\truey{300}%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\multiput(0,#1)(0,-\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(0,0){\shead}%
\end{picture}}}\end{picture}}%

% \SMONO{n} draws a south monomorphism of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SMONO}[1]%
{\truetail%
\monolength=#1%
\advance\monolength by -\truemonotail%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,\monolength){\line(0,-1){\monolength}}%
\put(0,\monolength){\shead}%
\put(0,0){\shead}%
\end{picture}}}\end{picture}}%


% \SEPI{n} draws a south epimorphism of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SEPI}[1]%
{\truehead%
\epilength=#1%
\advance\epilength by -\trueepihead%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,#1){\line(0,-1){\epilength}}%
\put(0,\trueepihead){\shead}%
\put(0,0){\shead}%
\end{picture}}}\end{picture}}%

% \SBIMO{n} draws a south bimorphism of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SBIMO}[1]%
{\truehead\truetail%
\monolength=#1%
\advance\monolength by -\truemonotail%
\epilength=\monolength%
\advance\epilength by -\trueepihead%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,\monolength){\line(0,-1){\epilength}}%
\put(0,\monolength){\shead}%
\put(0,\trueepihead){\shead}%
\put(0,0){\shead}%
\end{picture}}}\end{picture}}%

% \SBIAR{n} draws a pair of south arrows of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SBIAR}[1]%
{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(-\value{x},#1){\line(0,-1){#1}}%
\put(-\value{x},0){\shead}%
\put(\value{x},#1){\line(0,-1){#1}}%
\put(\value{x},0){\shead}%
\end{picture}}}\end{picture}}%

% \SBIDIST{n} draws a pair of south distributors of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SBIDIST}[1]%
{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(-\value{x},#1){\line(0,-1){#1}}%
\put(-\value{x},0){\shead}%
\put(\value{x},#1){\line(0,-1){#1}}%
\put(\value{x},0){\shead}%
\end{picture}}}%
\truey{400}%
\put(-\value{x},0){\circle{\value{y}}}%
\put(\value{x},0){\circle{\value{y}}}%
\end{picture}}%

% \SEQL{n} draws a vertical equality of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SEQL}[1]%
{\begin{picture}(0,0)%
\truex{100}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)\put(-\value{x},#1){\line(0,-1){#1}}%
\put(\value{x},#1){\line(0,-1){#1}}%
\end{picture}}}\end{picture}}%

% \SADJAR{n} draws a pair of vertical adjoint arrows of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SADJAR}[1]{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(-\value{x},#1){\line(0,-1){#1}}%
\put(-\value{x},0){\shead}%
\put(\value{x},0){\line(0,1){#1}}%
\put(\value{x},#1){\nhead}%
\end{picture}}}\end{picture}}%

% \SADJDIST{n} draws a pair of vertical adjoint distributors of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\SADJDIST}[1]{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(-\value{x},#1){\line(0,-1){#1}}%
\put(-\value{x},0){\shead}%
\put(\value{x},0){\line(0,1){#1}}%
\put(\value{x},#1){\nhead}%
\end{picture}}}%
\truey{400}%
\put(-\value{x},0){\circle{\value{y}}}%
\put(\value{x},0){\circle{\value{y}}}%
\end{picture}}%


% All the following commands produce south arrows

% basic south arrow
\def\basicsar[#1]{\vcase{\SAR}{#100}}%

% south arrow
\newcommand{\sar}{\@ifnextchar[{\basicsar}{\basicsar[50]}}%

% basic south arrow with left name
\def\basicSar[#1]#2{\Vcase{\SAR}{#2}{#100}}%

% south arrow with left name
\newcommand{\Sar}{\@ifnextchar[{\basicSar}{\basicSar[50]}}%

% basic south arrow with right name
\def\basicsaR[#1]#2{\vcasE{\SAR}{#2}{#100}}%

% south arrow with right name
\newcommand{\saR}{\@ifnextchar[{\basicsaR}{\basicsaR[50]}}%

% basic south distributor
\def\basicsdist[#1]{\vcase{\SDIST}{#100}}%

% south distributor
\newcommand{\sdist}{\@ifnextchar[{\basicsdist}{\basicsdist[50]}}%

% basic south distributor with left name
\def\basicSdist[#1]#2{\Vcase{\SDIST}{#2\hspace*{2pt}}{#100}}%

% south distributor with left name
\newcommand{\Sdist}{\@ifnextchar[{\basicSdist}{\basicSdist[50]}}%

% basic south distributor with right name
\def\basicsdisT[#1]#2{\vcasE{\SDIST}{\hspace*{2pt}#2}{#100}}%

% south distributor with right name
\newcommand{\sdisT}{\@ifnextchar[{\basicsdisT}{\basicsdisT[50]}}%

% basic south dotted arrow
\def\basicsdotar[#1]{\vcase{\SDOTAR}{#100}}%

% south dotted arrow
\newcommand{\sdotar}{\@ifnextchar[{\basicsdotar}{\basicsdotar[50]}}%

% basic south dotted arrow with left name
\def\basicSdotar[#1]#2{\Vcase{\SDOTAR}{#2}{#100}}%

% south dotted arrow with left name
\newcommand{\Sdotar}{\@ifnextchar[{\basicSdotar}{\basicSdotar[50]}}%

% basic south dotted arrow with right name
\def\basicsdotaR[#1]#2{\vcasE{\SDOTAR}{#2}{#100}}%

% south dotted arrow with right name
\newcommand{\sdotaR}{\@ifnextchar[{\basicsdotaR}{\basicsdotaR[50]}}%

% basic south monomorphism
\def\basicsmono[#1]{\vcase{\SMONO}{#100}}%

% south arrow
\newcommand{\smono}{\@ifnextchar[{\basicsmono}{\basicsmono[50]}}%

% basic south monomorphism with left name
\def\basicSmono[#1]#2{\Vcase{\SMONO}{#2}{#100}}%

% south monomorphism with left name
\newcommand{\Smono}{\@ifnextchar[{\basicSmono}{\basicSmono[50]}}%

% basic south monomorphism with right name
\def\basicsmonO[#1]#2{\vcasE{\SMONO}{#2}{#100}}%

% south monomorphism with right name
\newcommand{\smonO}{\@ifnextchar[{\basicsmonO}{\basicsmonO[50]}}%

% basic south epimorphism
\def\basicsepi[#1]{\vcase{\SEPI}{#100}}%

% south epimorphism
\newcommand{\sepi}{\@ifnextchar[{\basicsepi}{\basicsepi[50]}}%

% basic south epimorphism with left name
\def\basicSepi[#1]#2{\Vcase{\SEPI}{#2}{#100}}%

% south epimorphism with left name
\newcommand{\Sepi}{\@ifnextchar[{\basicSepi}{\basicSepi[50]}}%

% basic south epimorphism with right name
\def\basicsepI[#1]#2{\vcasE{\SEPI}{#2}{#100}}%

% south epimorphism with right name
\newcommand{\sepI}{\@ifnextchar[{\basicsepI}{\basicsepI[50]}}%

% basic south bimorphism
\def\basicsbimo[#1]{\vcase{\SBIMO}{#100}}%

% south bimorphism
\newcommand{\sbimo}{\@ifnextchar[{\basicsbimo}{\basicsbimo[50]}}%

% basic south bimorphism with left name
\def\basicSbimo[#1]#2{\Vcase{\SBIMO}{#2}{#100}}%

% south bimorphism with left name
\newcommand{\Sbimo}{\@ifnextchar[{\basicSbimo}{\basicSbimo[50]}}%

% basic south bimorphism with right name
\def\basicsbimO[#1]#2{\vcasE{\SBIMO}{#2}{#100}}%

% south bimorphism with right name
\newcommand{\sbimO}{\@ifnextchar[{\basicsbimO}{\basicsbimO[50]}}%

% basic south isomorphism
\def\basicsiso[#1]{\Visocase{\SAR}{\cong}{}{#100}}%

% south isomorphism
\newcommand{\siso}{\@ifnextchar[{\basicsiso}{\basicsiso[50]}}%

% basic south isomorphism with left name
\def\basicSiso[#1]#2{\Visocase{\SAR}{#2}{\cong}{#100}}%

% south isomorphism with left name
\newcommand{\Siso}{\@ifnextchar[{\basicSiso}{\basicSiso[50]}}%

% basic south isomorphism with right name
\def\basicsisO[#1]#2{\Visocase{\SAR}{\cong}{#2}{#100}}%

% south isomorphism with right name
\newcommand{\sisO}{\@ifnextchar[{\basicsisO}{\basicsisO[50]}}%

% basic south equality
\def\basicseql[#1]{\vcase{\SEQL}{#100}}%

% south equality
\newcommand{\seql}{\@ifnextchar[{\basicseql}{\basicseql[50]}}%

% basic south equality with left name
\def\basicSeql[#1]#2{\Vcase{\SEQL}{#2\hspace*{2pt}}{#100}}%

% south equality with left name
\newcommand{\Seql}{\@ifnextchar[{\basicSeql}{\basicSeql[50]}}%

% basic south equality with right name
\def\basicseqL[#1]#2{\vcasE{\SEQL}{\hspace*{2pt}#2}{#100}}%

% south equality with right name
\newcommand{\seqL}{\@ifnextchar[{\basicseqL}{\basicseqL[50]}}%

% basic pair of south arrows
\def\basicsbiar[#1]{\vbicase{\SBIAR}{#100}}%

% pair of south arrows
\newcommand{\sbiar}{\@ifnextchar[{\basicsbiar}{\basicsbiar[50]}}%

% basic pair of south arrows with names
\def\basicSbiar[#1]#2#3{\Vbicase{\SBIAR}{#2}{#3}{#100}}%

% pair of south arrows with names
\newcommand{\Sbiar}{\@ifnextchar[{\basicSbiar}{\basicSbiar[50]}}%
\let\sbiaR=\Sbiar

% basic pair of south distributors
\def\basicsbidist[#1]{\vbicase{\SBIDIST}{#100}}%

% pair of south distributors
\newcommand{\sbidist}{\@ifnextchar[{\basicsbidist}{\basicsbidist[50]}}%

% basic pair of south distributors with names
\def\basicSbidist[#1]#2#3%
{\Vbicase{\SBIDIST}{#2\hspace*{2pt}}{\hspace*{2pt}#3}{#100}}%

% pair of south distributors with names
\newcommand{\Sbidist}{\@ifnextchar[{\basicSbidist}{\basicSbidist[50]}}%
\let\sbidisT=\Sbidist

% basic pair of south adjoint arrows
\def\basicsadjar[#1]{\vbicase{\SADJAR}{#100}}%

% pair of south adjoint arrows
\newcommand{\sadjar}{\@ifnextchar[{\basicsadjar}{\basicsadjar[50]}}%

% basic pair of south adjoint arrows with names
\def\basicSadjar[#1]#2#3{\Vbicase{\SADJAR}{#2}{#3}{#100}}%

% pair of south adjoint arrows with names
\newcommand{\Sadjar}{\@ifnextchar[{\basicSadjar}{\basicSadjar[50]}}%
\let\sadjaR=\Sadjar

% basic pair of south adjoint distributors
\def\basicsadjdist[#1]{\vbicase{\SADJDIST}{#100}}%

% pair of south adjoint distributors
\newcommand{\sadjdist}{\@ifnextchar[{\basicsadjdist}{\basicsadjdist[50]}}%

% basic pair of south adjoint distributors with names
\def\basicSadjdist[#1]#2#3%
{\Vbicase{\SADJDIST}{#2\hspace*{2pt}}{\hspace*{2pt}#3}{#100}}%

% pair of south adjoint distributors with names
\newcommand{\Sadjdist}{\@ifnextchar[{\basicSadjdist}{\basicSadjdist[50]}}%
\let\sadjdisT=\Sadjdist


% NORTH ARROWS

% \NAR{n} draws a north arrow of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NAR}[1]%
{\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,0){\line(0,1){#1}}%
\put(0,#1){\nhead}%
\end{picture}}}\end{picture}}%

% \NDIST{n} draws a north distributor of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NDIST}[1]%
{\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,0){\line(0,1){#1}}%
\put(0,#1){\nhead}%
\end{picture}}}
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\end{picture}}%

% \NDOTAR{n} draws a north dotted arrow of length n units
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NDOTAR}[1]%
{\truex{100}\truey{300}%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\multiput(0,0)(0,\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(0,#1){\nhead}%
\end{picture}}}\end{picture}}%


% \NMONO{n} draws a north monomorphism of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NMONO}[1]%
{\truetail%
\monolength=#1%
\advance\monolength by -\truemonotail%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,\truemonotail){\line(0,1){\monolength}}%
\put(0,#1){\nhead}%
\put(0,\truemonotail){\nhead}%
\end{picture}}}\end{picture}}%

% \NEPI{n} draws a north epimorphism of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NEPI}[1]%
{\truehead%
\epilength=#1%
\advance\epilength by -\trueepihead%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,0){\line(0,1){\epilength}}%
\put(0,#1){\nhead}%
\put(0,\epilength){\nhead}%
\end{picture}}}\end{picture}}%

% \NBIMO{n} draws a north bimorphism of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NBIMO}[1]%
{\truehead\truetail%
\epilength=#1%
\advance\epilength by -\trueepihead%
\monolength=\epilength%
\advance\monolength by -\truemonotail%
\begin{picture}(0,0)%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(0,\truemonotail){\line(0,1){\monolength}}%
\put(0,#1){\nhead}%
\put(0,\truemonotail){\nhead}%
\put(0,\epilength){\nhead}%
\end{picture}}}\end{picture}}%

% \NBIAR{n} draws a pair of north arrows of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NBIAR}[1]%
{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(-\value{x},0){\line(0,1){#1}}%
\put(-\value{x},#1){\nhead}%
\put(\value{x},0){\line(0,1){#1}}%
\put(\value{x},#1){\nhead}%
\end{picture}}}\end{picture}}%

% \NBIDIST{n} draws a pair of north distributors of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NBIDIST}[1]%
{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(-\value{x},0){\line(0,1){#1}}%
\put(-\value{x},#1){\nhead}%
\put(\value{x},0){\line(0,1){#1}}%
\put(\value{x},#1){\nhead}%
\end{picture}}}
\truey{400}%
\put(-\value{x},0){\circle{\value{y}}}%
\put(\value{x},0){\circle{\value{y}}}%
\end{picture}}%

% \NADJAR{n} draws a pair of vertical adjoint arrows of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NADJAR}[1]{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(\value{x},#1){\line(0,-1){#1}}%
\put(\value{x},0){\shead}%
\put(-\value{x},0){\line(0,1){#1}}%
\put(-\value{x},#1){\nhead}%
\end{picture}}}\end{picture}}%

% \NADJDIST{n} draws a pair of vertical adjoint distributors of length n pt
% and centers it in a box of width 0pt and height 0pt
\newcommand{\NADJDIST}[1]{\begin{picture}(0,0)%
\truex{350}%
\put(0,0){\makebox(0,0)%
{\begin{picture}(0,#1)%
\put(\value{x},#1){\line(0,-1){#1}}%
\put(\value{x},0){\shead}%
\put(-\value{x},0){\line(0,1){#1}}%
\put(-\value{x},#1){\nhead}%
\end{picture}}}
\truey{400}%
\put(-\value{x},0){\circle{\value{y}}}%
\put(\value{x},0){\circle{\value{y}}}%
\end{picture}}%


% All the following commands produce north arrows

% basic north arrow
\def\basicnar[#1]{\vcase{\NAR}{#100}}%

% north arrow
\newcommand{\nar}{\@ifnextchar[{\basicnar}{\basicnar[50]}}%

% basic north arrow with left name
\def\basicNar[#1]#2{\Vcase{\NAR}{#2}{#100}}%

% north arrow with left name
\newcommand{\Nar}{\@ifnextchar[{\basicNar}{\basicNar[50]}}%

% basic north arrow with right name
\def\basicnaR[#1]#2{\vcasE{\NAR}{#2}{#100}}%

% north arrow with right name
\newcommand{\naR}{\@ifnextchar[{\basicnaR}{\basicnaR[50]}}%

% basic north distributor
\def\basicndist[#1]{\vcase{\NDIST}{#100}}%

% north distributor
\newcommand{\ndist}{\@ifnextchar[{\basicndist}{\basicndist[50]}}%

% basic north distributor with left name
\def\basicNdist[#1]#2{\Vcase{\NDIST}{#2\hspace*{2pt}}{#100}}%

% north distributor with left name
\newcommand{\Ndist}{\@ifnextchar[{\basicNdist}{\basicNdist[50]}}%

% basic north distributor with right name
\def\basicndisT[#1]#2{\vcasE{\NDIST}{\hspace*{2pt}#2}{#100}}%

% north distributor with right name
\newcommand{\ndisT}{\@ifnextchar[{\basicndisT}{\basicndisT[50]}}%

% basic north dotted arrow
\def\basicndotar[#1]{\vcase{\NDOTAR}{#100}}%

% north dotted arrow
\newcommand{\ndotar}{\@ifnextchar[{\basicndotar}{\basicndotar[50]}}%

% basic north dotted arrow with left name
\def\basicNdotar[#1]#2{\Vcase{\NDOTAR}{#2}{#100}}%

% north dotted arrow with left name
\newcommand{\Ndotar}{\@ifnextchar[{\basicNdotar}{\basicNdotar[50]}}%

% basic north dotted arrow with right name
\def\basicndotaR[#1]#2{\vcasE{\NDOTAR}{#2}{#100}}%

% north dotted arrow with right name
\newcommand{\ndotaR}{\@ifnextchar[{\basicndotaR}{\basicndotaR[50]}}%

% basic north monomorphism
\def\basicnmono[#1]{\vcase{\NMONO}{#100}}%

% north arrow
\newcommand{\nmono}{\@ifnextchar[{\basicnmono}%
{\basicnmono[50]}}%

% basic north monomorphism with left name
\def\basicNmono[#1]#2{\Vcase{\NMONO}{#2}{#100}}%

% north monomorphism with left name
\newcommand{\Nmono}{\@ifnextchar[{\basicNmono}{\basicNmono[50]}}%

% basic north monomorphism with right name
\def\basicnmonO[#1]#2{\vcasE{\NMONO}{#2}{#100}}%

% north monomorphism with right name
\newcommand{\nmonO}{\@ifnextchar[{\basicnmonO}{\basicnmonO[50]}}%

% basic north epimorphism
\def\basicnepi[#1]{\vcase{\NEPI}{#100}}%

% north epimorphism
\newcommand{\nepi}{\@ifnextchar[{\basicnepi}{\basicnepi[50]}}%

% basic north epimorphism with left name
\def\basicNepi[#1]#2{\Vcase{\NEPI}{#2}{#100}}%

% north epimorphism with left name
\newcommand{\Nepi}{\@ifnextchar[{\basicNepi}{\basicNepi[50]}}%

% basic north epimorphism with right name
\def\basicnepI[#1]#2{\vcasE{\NEPI}{#2}{#100}}%

% north epimorphism with right name
\newcommand{\nepI}{\@ifnextchar[{\basicnepI}{\basicnepI[50]}}%

% basic north bimorphism
\def\basicnbimo[#1]{\vcase{\NBIMO}{#100}}%

% north bimorphism
\newcommand{\nbimo}{\@ifnextchar[{\basicnbimo}{\basicnbimo[50]}}%

% basic north bimorphism with left name
\def\basicNbimo[#1]#2{\Vcase{\NBIMO}{#2}{#100}}%

% north bimorphism with left name
\newcommand{\Nbimo}{\@ifnextchar[{\basicNbimo}{\basicNbimo[50]}}%

% basic north bimorphism with right name
\def\basicnbimO[#1]#2{\vcasE{\NBIMO}{#2}{#100}}%

% north bimorphism with right name
\newcommand{\nbimO}{\@ifnextchar[{\basicnbimO}{\basicnbimO[50]}}%

% basic north isomorphism
\def\basicniso[#1]{\Visocase{\NAR}{\cong}{}{#100}}%

% north isomorphism
\newcommand{\niso}{\@ifnextchar[{\basicniso}{\basicniso[50]}}%

% basic north isomorphism with left name
\def\basicNiso[#1]#2{\Visocase{\NAR}{#2}{\cong}{#100}}%

% north isomorphism with left name
\newcommand{\Niso}{\@ifnextchar[{\basicNiso}{\basicNiso[50]}}%

% basic north isomorphism with right name
\def\basicnisO[#1]#2{\Visocase{\NAR}{\cong}{#2}{#100}}%

% north isomorphism with right name
\newcommand{\nisO}{\@ifnextchar[{\basicnisO}{\basicnisO[50]}}%

% north equality
\let\neql=\seql%

% north equality with left name
\let\Neql=\Seql%

% north equality with right name
\let\neqL=\seqL%

% basic pair of north arrows
\def\basicnbiar[#1]{\vbicase{\NBIAR}{#100}}%

% pair of north arrows
\newcommand{\nbiar}{\@ifnextchar[{\basicnbiar}{\basicnbiar[50]}}%

% basic pair of north arrows with names
\def\basicNbiar[#1]#2#3{\Vbicase{\NBIAR}{#2}{#3}{#100}}%

% pair of north arrows with names
\newcommand{\Nbiar}{\@ifnextchar[{\basicNbiar}{\basicNbiar[50]}}%
\let\nbiaR=\Nbiar

% basic pair of north distributors
\def\basicnbidist[#1]{\vbicase{\NBIDIST}{#100}}%

% pair of north distributors
\newcommand{\nbidist}{\@ifnextchar[{\basicnbidist}{\basicnbidist[50]}}%

% basic pair of north distributors with names
\def\basicNbidist[#1]#2#3%
{\Vbicase{\NBIDIST}{#2\hspace*{2pt}}{\hspace*{2pt}#3}{#100}}%

% pair of north distributors with names
\newcommand{\Nbidist}{\@ifnextchar[{\basicNbidist}{\basicNbidist[50]}}%
\let\nbidisT=\Nbidist

% basic pair of north adjoint arrows
\def\basicnadjar[#1]{\vbicase{\NADJAR}{#100}}%

% pair of north adjoint arrows
\newcommand{\nadjar}{\@ifnextchar[{\basicnadjar}{\basicnadjar[50]}}%

% basic pair of north adjoint arrows with names
\def\basicNadjar[#1]#2#3{\Vbicase{\NADJAR}{#2}{#3}{#100}}%

% pair of north adjoint arrows with names
\newcommand{\Nadjar}{\@ifnextchar[{\basicNadjar}{\basicNadjar[50]}}%
\let\nadjaR=\Nadjar

% basic pair of north adjoint distributors
\def\basicnadjdist[#1]{\vbicase{\NADJDIST}{#100}}%

% pair of north adjoint distributors
\newcommand{\nadjdist}{\@ifnextchar[{\basicnadjdist}{\basicnadjdist[50]}}%

% basic pair of north adjoint distributors with names
\def\basicNadjdist[#1]#2#3%
{\Vbicase{\NADJDIST}{#2\hspace*{2pt}}{\hspace*{2pt}#3}{#100}}%

% pair of north adjoint distributors with names
\newcommand{\Nadjdist}{\@ifnextchar[{\basicNadjdist}{\basicNadjdist[50]}}%
\let\nadjdisT=\Nadjdist



% MACROS FOR  FIRST DIAGONAL PICTURES


% \fdcase{P}{f}{g}{n} draws the picture P with names f, g
% and length n units
\newcommand{\fdcase}[4]{\testdiagrammode\begin{picture}(0,0)%
\put(0,0){#1{#4}}%
\truex{200}\truey{600}\truez{600}%
\put(-\value{x},-\value{x}){\makebox(0,\value{z})[r]{${#2}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#3}$}}%
\end{picture}}%

% \fdbicase{P}{f}{g}{n} draws the bipicture P with names f, g
% and length n units
\newcommand{\fdbicase}[4]{\testdiagrammode\begin{picture}(0,0)%
\put(0,0){#1{#4}}%
\truex{900}\truey{150}%
\put(-\value{x},\value{y}){${#2}$}%
\truex{300}\truey{1050}%
\put(\value{x},-\value{y}){${#3}$}%
\end{picture}}%


% NORTH-EAST ARROWS

% \NEAR{n} draws a north-east arrow of length nx100 units
\newcommand{\NEAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\line(1,1){#1}}%
\put(\Y,\Y){\nehead}%
\end{picture}}%

% \NEDIST{n} draws a north-east distributor of length n units
\newcommand{\NEDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\line(1,1){#1}}%
\put(\Y,\Y){\nehead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\end{picture}}%

% \NEDOTAR{n} draws a north-east dotted arrow of length n units
\newcommand{\NEDOTAR}[1]%
{\truex{100}\truey{212}%
\Y=#1%
\divide\Y by 2%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(-\Y,-\Y)(\value{y},\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(\Y,\Y){\nehead}%
\end{picture}}%

% \NEMONO{n} draws a north-east monomorphism of length n units
\newcommand{\NEMONO}[1]{%
\Y=#1%
\divide \Y by 2%
\Truetail%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\begin{picture}(0,0)%
\put(-\monolength,-\monolength){\line(1,1){\bimolength}}%
\put(-\monolength,-\monolength){\nehead}%
\put(\Y,\Y){\nehead}%
\end{picture}}%

% \NEEPI{n} draws a north-east epimorphism of length n units
\newcommand{\NEEPI}[1]{%
\Y=#1%
\divide\Y by 2%
\Truehead%
\bimolength=#1%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\line(1,1){\bimolength}}%
\put(\epilength,\epilength){\nehead}%
\put(\Y,\Y){\nehead}%
\end{picture}}%

% \NEBIMO{n} draws a north-east bimorphism of length n units
\newcommand{\NEBIMO}[1]{%
\Y=#1%
\divide\Y by 2%
\Truetail\Truehead%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\begin{picture}(0,0)%
\put(-\monolength,-\monolength){\line(1,1){\bimolength}}%
\put(-\monolength,-\monolength){\nehead}%
\put(\epilength,\epilength){\nehead}%
\put(\Y,\Y){\nehead}%
\end{picture}}%

% \NEBIAR{n} draws a pair of north-east arrows of length n units
\newcommand{\NEBIAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\put(-\value{x},\value{x}){\line(1,1){#1}}%
\put(\value{x},-\value{x}){\line(1,1){#1}}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\monolength,\epilength){\nehead}%
\put(\epilength,\monolength){\nehead}%
\end{picture}}\end{picture}}%

% \NEBIDIST{n} draws a pair of north-east distributors of length n units
\newcommand{\NEBIDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},-\value{x}){\line(1,1){#1}}%
\put(\epilength,\monolength){\nehead}%
\end{picture}}%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by \value{x}%
\epilength=#1%
\advance\epilength by -\value{x}%
\put(-\value{x},\value{x}){\line(1,1){#1}}%
\put(\epilength,\monolength){\nehead}%
\end{picture}}%
\put(-\value{x},\value{x}){\circle{\value{y}}}%
\put(\value{x},-\value{x}){\circle{\value{y}}}%
\end{picture}}%

% \NEEQL{n} draws a north-east equality of length n units
\newcommand{\NEEQL}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{70}%
\put(-\value{x},\value{x}){\line(1,1){#1}}%
\put(\value{x},-\value{x}){\line(1,1){#1}}%
\end{picture}}\end{picture}}%

% \NEADJAR{n} draws a north-east pair of adjoint arrows of length n units
\newcommand{\NEADJAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},-\value{x}){\line(1,1){#1}}%
\put(\epilength,\monolength){\nehead}%
\end{picture}}%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},\value{x}){\line(-1,-1){#1}}%
\put(-\epilength,-\monolength){\swhead}%
\end{picture}}\end{picture}}%

% \NEADJDIST{n} draws a north-east pair of adjoint distributors of length n units
\newcommand{\NEADJDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},-\value{x}){\line(1,1){#1}}%
\put(\epilength,\monolength){\nehead}%
\end{picture}}%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},\value{x}){\line(-1,-1){#1}}%
\put(-\epilength,-\monolength){\swhead}%
\end{picture}}%
\put(-\value{x},\value{x}){\circle{\value{y}}}%
\put(\value{x},-\value{x}){\circle{\value{y}}}%
\end{picture}}%


% All the following commands draw north-east arrows

% north-east arrow of length nx100 units
\def\basicnear[#1]{\fdcase{\NEAR}{}{}{#100}}%

% north-east arrow
\newcommand{\near}{\@ifnextchar[{\basicnear}{\basicnear[59]}}%

% north-east arrow with upper name [1] and length nx100 units
\def\basicNear[#1]#2{\fdcase{\NEAR}{#2}{}{#100}}%

% north-east arrow with upper name
\newcommand{\Near}{\@ifnextchar[{\basicNear}{\basicNear[59]}}%

% north-east arrow with lower name [1]  and length nx100 units
\def\basicneaR[#1]#2{\fdcase{\NEAR}{}{#2}{#100}}%

% north-east arrow with lower name [1]
\newcommand{\neaR}{\@ifnextchar[{\basicneaR}{\basicneaR[59]}}%

% north-east distributor of length nx100 units
\def\basicnedist[#1]{\fdcase{\NEDIST}{}{}{#100}}%

% north-east distributor
\newcommand{\nedist}{\@ifnextchar[{\basicnedist}{\basicnedist[59]}}%

% north-east distributor with upper name [1] and length nx100 units
\def\basicNedist[#1]#2{\fdcase{\NEDIST}{#2}{}{#100}}%

% north-east distributor with upper name
\newcommand{\Nedist}{\@ifnextchar[{\basicNedist}{\basicNedist[59]}}%

% north-east distributor with lower name [1]  and length nx100 units
\def\basicnedisT[#1]#2{\fdcase{\NEDIST}{}{#2}{#100}}%

% north-east distributor with lower name [1]
\newcommand{\nedisT}{\@ifnextchar[{\basicnedisT}{\basicnedisT[59]}}%

% north-east dotted arrow of length nx100 units
\def\basicnedotar[#1]{\fdcase{\NEDOTAR}{}{}{#100}}%

% north-east dotted arrow
\newcommand{\nedotar}{\@ifnextchar[{\basicnedotar}{\basicnedotar[59]}}%

% north-east dotted arrow with upper name [1] and length nx100 units
\def\basicNedotar[#1]#2{\fdcase{\NEDOTAR}{#2}{}{#100}}%

% north-east dotted arrow with upper name
\newcommand{\Nedotar}{\@ifnextchar[{\basicNedotar}{\basicNedotar[59]}}%

% north-east dotted arrow with lower name [1]  and length nx100 units
\def\basicnedotaR[#1]#2{\fdcase{\NEDOTAR}{}{#2}{#100}}%

% north-east dotted arrow with lower name [1]
\newcommand{\nedotaR}{\@ifnextchar[{\basicnedotaR}{\basicnedotaR[59]}}%

% north-east monomorphism of length nx100 units
\def\basicnemono[#1]{\fdcase{\NEMONO}{}{}{#100}}%

% north-east monomorphism
\newcommand{\nemono}{\@ifnextchar[{\basicnemono}{\basicnemono[59]}}%

% north-east monomorphism with upper name [1] and length nx100 units
\def\basicNemono[#1]#2{\fdcase{\NEMONO}{#2}{}{#100}}%

% north-east monomophism with upper name
\newcommand{\Nemono}{\@ifnextchar[{\basicNemono}{\basicNemono[59]}}%

% north-east monomorphism with lower name [1]  and length nx100 units
\def\basicnemonO[#1]#2{\fdcase{\NEMONO}{}{#2}{#100}}%

% north-east monomorphism with lower name [1]
\newcommand{\nemonO}{\@ifnextchar[{\basicnemonO}{\basicnemonO[59]}}%

% north-east epimorphism of length nx100 units
\def\basicneepi[#1]{\fdcase{\NEEPI}{}{}{#100}}%

% north-east epimorphism
\newcommand{\neepi}{\@ifnextchar[{\basicneepi}{\basicneepi[59]}}%

% north-east epimorphism with upper name [1] and length nx100 units
\def\basicNeepi[#1]#2{\fdcase{\NEEPI}{#2}{}{#100}}%

% north-east epimorphism with upper name
\newcommand{\Neepi}{\@ifnextchar[{\basicNeepi}{\basicNeepi[59]}}%

% north-east epimorphism with lower name [1]  and length nx100 units
\def\basicneepI[#1]#2{\fdcase{\NEEPI}{}{#2}{#100}}%

% north-east epimorphism with lower name [1]
\newcommand{\neepI}{\@ifnextchar[{\basicneepI}{\basicneepI[59]}}%

% north-east bimorphism of length nx100 units
\def\basicnebimo[#1]{\fdcase{\NEBIMO}{}{}{#100}}%

% north-east bimorphism
\newcommand{\nebimo}{\@ifnextchar[{\basicnebimo}{\basicnebimo[59]}}%

% north-east bimorphism with upper name [1] and length nx100 units
\def\basicNebimo[#1]#2{\fdcase{\NEBIMO}{#2}{}{#100}}%

% north-east bimorphism with upper name
\newcommand{\Nebimo}{\@ifnextchar[{\basicNebimo}{\basicNebimo[59]}}%

% north-east bimorphism with lower name [1]  and length nx100 units
\def\basicnebimO[#1]#2{\fdcase{\NEBIMO}{}{#2}{#100}}%

% north-east bimorphism with lower name [1]
\newcommand{\nebimO}{\@ifnextchar[{\basicnebimO}{\basicnebimO[59]}}%

% north-east isomorphism of length nx100 units
\def\basicneiso[#1]{\fdcase{\NEAR}{\hspace{-2pt}\cong}{}{#100}}%

% north-east isomorphism
\newcommand{\neiso}{\@ifnextchar[{\basicneiso}{\basicneiso[59]}}%

% north-east isomorphism with upper name [1] and length nx100 units
\def\basicNeiso[#1]#2{\fdcase{\NEAR}{#2}{\cong}{#100}}%

% north-east isomorphism with upper name
\newcommand{\Neiso}{\@ifnextchar[{\basicNeiso}{\basicNeiso[59]}}%

% north-east isomorphism with lower name [1]  and length nx100 units
\def\basicneisO[#1]#2{\fdcase{\NEAR}{\hspace{-2pt}\cong}{#2}{#100}}%

% north-east isomorphism with lower name [1]
\newcommand{\neisO}{\@ifnextchar[{\basicneisO}{\basicneisO[59]}}%

% north-east equality of length nx100 units
\def\basicneeql[#1]{\fdcase{\NEEQL}{}{}{#100}}%

% north-east equality
\newcommand{\neeql}{\@ifnextchar[{\basicneeql}{\basicneeql[59]}}%

% north-east equality with upper name [1] and length nx100 units
\def\basicNeeql[#1]#2{\fdcase{\NEEQL}{#2}{}{#100}}%

% north-east equality with upper name
\newcommand{\Neeql}{\@ifnextchar[{\basicNeeql}{\basicNeeql[59]}}%

% north-east equality with lower name [1]  and length nx100 units
\def\basicneeqL[#1]#2{\fdcase{\NEEQL}{}{#2}{#100}}%

% north-east equality with lower name [1]
\newcommand{\neeqL}{\@ifnextchar[{\basicneeqL}{\basicneeqL[59]}}%

% pair of north-east arrows of length nx100 units
\def\basicnebiar[#1]{\fdbicase{\NEBIAR}{}{}{#100}}%

% pair of north-east arrows
\newcommand{\nebiar}{\@ifnextchar[{\basicnebiar}{\basicnebiar[59]}}%

% pair of north-east arrows with names [1][2] and length nx100 units
\def\basicNebiar[#1]#2#3{\fdbicase{\NEBIAR}{#2}{#3}{#100}}%

% pair of north-east arrows with names
\newcommand{\Nebiar}{\@ifnextchar[{\basicNebiar}{\basicNebiar[59]}}%
\let\nebiaR=\Nebiar

% pair of north-east adjoint arrows of length nx100 units
\def\basicneadjar[#1]{\fdbicase{\NEADJAR}{}{}{#100}}%

% pair of north-east adjoint arrows
\newcommand{\neadjar}{\@ifnextchar[{\basicneadjar}{\basicneadjar[59]}}%

% pair of north-east adjoint arrows with names [1][2] and length nx100 units
\def\basicNeadjar[#1]#2#3{\fdbicase{\NEADJAR}{#2}{#3}{#100}}%

% pair of north-east adjoint arrows with names
\newcommand{\Neadjar}{\@ifnextchar[{\basicNeadjar}{\basicNeadjar[59]}}%
\let\neadjaR=\Neadjar

% pair of north-east distributors of length nx100 units
\def\basicnebidist[#1]{\fdbicase{\NEBIDIST}{}{}{#100}}%

% pair of north-east distributors
\newcommand{\nebidist}{\@ifnextchar[{\basicnebidist}{\basicnebidist[59]}}%

% pair of north-east distributors with names [1][2] and length nx100 units
\def\basicNebidist[#1]#2#3{\fdbicase{\NEBIDIST}{#2}{#3}{#100}}%

% pair of north-east distributors with names
\newcommand{\Nebidist}{\@ifnextchar[{\basicNebidist}{\basicNebidist[59]}}%
\let\nebidisT=\Nebidist

% pair of north-east adjoint distributors of length nx100 units
\def\basicneadjdist[#1]{\fdbicase{\NEADJDIST}{}{}{#100}}%

% pair of north-east adjoint distributors
\newcommand{\neadjdist}{\@ifnextchar[{\basicneadjdist}{\basicneadjdist[59]}}%

% pair of north-east adjoint distributors with names [1][2] and length nx100 units
\def\basicNeadjdist[#1]#2#3{\fdbicase{\NEADJDIST}{#2}{#3}{#100}}%

% pair of north-east adjoint distributors with names
\newcommand{\Neadjdist}{\@ifnextchar[{\basicNeadjdist}{\basicNeadjdist[59]}}%
\let\neadjdisT=\Neadjdist



% SOUT-WEST ARROWS

% \SWAR{n} draws a south-west arrow of length nx100 units
\newcommand{\SWAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,\Y){\line(-1,-1){#1}}%
\put(-\Y,-\Y){\swhead}%
\end{picture}}%

% \SWDIST{n} draws a south-west distributor of length n units
\newcommand{\SWDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,\Y){\line(-1,-1){#1}}%
\put(-\Y,-\Y){\swhead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\end{picture}}%

% \SWDOTAR{n} draws a south-west dotted arrow of length n units
\newcommand{\SWDOTAR}[1]%
{\truex{100}\truey{212}%
\Y=#1%
\divide\Y by 2%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(\Y,\Y)(-\value{y},-\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(-\Y,-\Y){\swhead}%
\end{picture}}%

% \SWMONO{n} draws a south-west monomorphism of length n units
\newcommand{\SWMONO}[1]{%
\Y=#1%
\divide \Y by 2%
\Truetail%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\begin{picture}(0,0)%
\put(\monolength,\monolength){\line(-1,-1){\bimolength}}%
\put(\monolength,\monolength){\swhead}%
\put(-\Y,-\Y){\swhead}%
\end{picture}}%

% \SWEPI{n} draws a south-west epimorphism of length n units
\newcommand{\SWEPI}[1]{%
\Y=#1%
\divide\Y by 2%
\Truehead%
\bimolength=#1%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\begin{picture}(0,0)%
\put(\Y,\Y){\line(-1,-1){\bimolength}}%
\put(-\epilength,-\epilength){\swhead}%
\put(-\Y,-\Y){\swhead}%
\end{picture}}%

% \SWBIMO{n} draws a south-west bimorphism of length n units
\newcommand{\SWBIMO}[1]{%
\Y=#1%
\divide\Y by 2%
\Truetail\Truehead%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\begin{picture}(0,0)%
\put(\monolength,\monolength){\line(-1,-1){\bimolength}}%
\put(\monolength,\monolength){\swhead}%
\put(-\epilength,-\epilength){\swhead}%
\put(-\Y,-\Y){\swhead}%
\end{picture}}%

% \SWBIAR{n} draws a pair of south-west arrows of length n units
\newcommand{\SWBIAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\put(\value{x},-\value{x}){\line(-1,-1){#1}}%
\put(-\value{x},\value{x}){\line(-1,-1){#1}}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\monolength,-\epilength){\swhead}%
\put(-\epilength,-\monolength){\swhead}%
\end{picture}}\end{picture}}%

% \SWBIDIST{n} draws a pair of south-west distributors of length n units
\newcommand{\SWBIDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},\value{x}){\line(-1,-1){#1}}%
\put(-\epilength,-\monolength){\swhead}%
\end{picture}}%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by \value{x}%
\epilength=#1%
\advance\epilength by -\value{x}%
\put(\value{x},-\value{x}){\line(-1,-1){#1}}%
\put(-\epilength,-\monolength){\swhead}%
\end{picture}}%
\put(\value{x},-\value{x}){\circle{\value{y}}}%
\put(-\value{x},\value{x}){\circle{\value{y}}}%
\end{picture}}%

% \SWADJAR{n} draws a south-west pair of adjoint arrows of length n units
\newcommand{\SWADJAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},-\value{x}){\line(-1,-1){#1}}%
\put(-\monolength,-\epilength){\swhead}%
\end{picture}}%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},\value{x}){\line(1,1){#1}}%
\put(\monolength,\epilength){\nehead}%
\end{picture}}\end{picture}}%

% \SWADJDIST{n} draws a south-west pair of adjoint distributors of length n units
\newcommand{\SWADJDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},-\value{x}){\line(-1,-1){#1}}%
\put(-\monolength,-\epilength){\swhead}%
\end{picture}}%
\put(-\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},\value{x}){\line(1,1){#1}}%
\put(\monolength,\epilength){\nehead}%
\end{picture}}%
\put(-\value{x},\value{x}){\circle{\value{y}}}%
\put(\value{x},-\value{x}){\circle{\value{y}}}%
\end{picture}}%


% All the following commands draw south-west arrows

% south-west arrow of length nx100 units
\def\basicswar[#1]{\fdcase{\SWAR}{}{}{#100}}%

% south-west arrow
\newcommand{\swar}{\@ifnextchar[{\basicswar}{\basicswar[59]}}%

% south-west arrow with upper name [1] and length nx100 units
\def\basicSwar[#1]#2{\fdcase{\SWAR}{#2}{}{#100}}%

% south-west arrow with upper name
\newcommand{\Swar}{\@ifnextchar[{\basicSwar}{\basicSwar[59]}}%

% south-west arrow with lower name [1]  and length nx100 units
\def\basicswaR[#1]#2{\fdcase{\SWAR}{}{#2}{#100}}%

% south-west arrow with lower name [1]
\newcommand{\swaR}{\@ifnextchar[{\basicswaR}{\basicswaR[59]}}%

% south-west distributor of length nx100 units
\def\basicswdist[#1]{\fdcase{\SWDIST}{}{}{#100}}%

% south-west distributor
\newcommand{\swdist}{\@ifnextchar[{\basicswdist}{\basicswdist[59]}}%

% south-west distributor with upper name [1] and length nx100 units
\def\basicSwdist[#1]#2{\fdcase{\SWDIST}{#2}{}{#100}}%

% south-west distributor with upper name
\newcommand{\Swdist}{\@ifnextchar[{\basicSwdist}{\basicSwdist[59]}}%

% south-west distributor with lower name [1]  and length nx100 units
\def\basicswdisT[#1]#2{\fdcase{\SWDIST}{}{#2}{#100}}%

% south-west distributor with lower name [1]
\newcommand{\swdisT}{\@ifnextchar[{\basicswdisT}{\basicswdisT[59]}}%

% south-west dotted arrow of length nx100 units
\def\basicswdotar[#1]{\fdcase{\SWDOTAR}{}{}{#100}}%

% south-west dotted arrow
\newcommand{\swdotar}{\@ifnextchar[{\basicswdotar}{\basicswdotar[59]}}%

% south-west dotted arrow with upper name [1] and length nx100 units
\def\basicSwdotar[#1]#2{\fdcase{\SWDOTAR}{#2}{}{#100}}%

% south-west dotted arrow with upper name
\newcommand{\Swdotar}{\@ifnextchar[{\basicSwdotar}{\basicSwdotar[59]}}%

% south-west dotted arrow with lower name [1]  and length nx100 units
\def\basicswdotaR[#1]#2{\fdcase{\SWDOTAR}{}{#2}{#100}}%

% south-west dotted arrow with lower name [1]
\newcommand{\swdotaR}{\@ifnextchar[{\basicswdotaR}{\basicswdotaR[59]}}%

% south-west monomorphism of length nx100 units
\def\basicswmono[#1]{\fdcase{\SWMONO}{}{}{#100}}%

% south-west monomorphism
\newcommand{\swmono}{\@ifnextchar[{\basicswmono}{\basicswmono[59]}}%

% south-west monomorphism with upper name [1] and length nx100 units
\def\basicSwmono[#1]#2{\fdcase{\SWMONO}{#2}{}{#100}}%

% south-west monomophism with upper name
\newcommand{\Swmono}{\@ifnextchar[{\basicSwmono}{\basicSwmono[59]}}%

% south-west monomorphism with lower name [1]  and length nx100 units
\def\basicswmonO[#1]#2{\fdcase{\SWMONO}{}{#2}{#100}}%

% south-west monomorphism with lower name [1]
\newcommand{\swmonO}{\@ifnextchar[{\basicswmonO}{\basicswmonO[59]}}%

% south-west epimorphism of length nx100 units
\def\basicswepi[#1]{\fdcase{\SWEPI}{}{}{#100}}%

% south-west epimorphism
\newcommand{\swepi}{\@ifnextchar[{\basicswepi}{\basicswepi[59]}}%

% south-west epimorphism with upper name [1] and length nx100 units
\def\basicSwepi[#1]#2{\fdcase{\SWEPI}{#2}{}{#100}}%

% south-west epimorphism with upper name
\newcommand{\Swepi}{\@ifnextchar[{\basicSwepi}{\basicSwepi[59]}}%

% south-west epimorphism with lower name [1]  and length nx100 units
\def\basicswepI[#1]#2{\fdcase{\SWEPI}{}{#2}{#100}}%

% south-west epimorphism with lower name [1]
\newcommand{\swepI}{\@ifnextchar[{\basicswepI}{\basicswepI[59]}}%

% south-west bimorphism of length nx100 units
\def\basicswbimo[#1]{\fdcase{\SWBIMO}{}{}{#100}}%

% south-west bimorphism
\newcommand{\swbimo}{\@ifnextchar[{\basicswbimo}{\basicswbimo[59]}}%

% south-west bimorphism with upper name [1] and length nx100 units
\def\basicSwbimo[#1]#2{\fdcase{\SWBIMO}{#2}{}{#100}}%

% south-west bimorphism with upper name
\newcommand{\Swbimo}{\@ifnextchar[{\basicSwbimo}{\basicSwbimo[59]}}%

% south-west bimorphism with lower name [1]  and length nx100 units
\def\basicswbimO[#1]#2{\fdcase{\SWBIMO}{}{#2}{#100}}%

% south-west bimorphism with lower name [1]
\newcommand{\swbimO}{\@ifnextchar[{\basicswbimO}{\basicswbimO[59]}}%

% south-west isomorphism of length nx100 units
\def\basicswiso[#1]{\fdcase{\SWAR}{\hspace{-2pt}\cong}{}{#100}}%

% south-west isomorphism
\newcommand{\swiso}{\@ifnextchar[{\basicswiso}{\basicswiso[59]}}%

% south-west isomorphism with upper name [1] and length nx100 units
\def\basicSwiso[#1]#2{\fdcase{\SWAR}{#2}{\cong}{#100}}%

% south-west isomorphism with upper name
\newcommand{\Swiso}{\@ifnextchar[{\basicSwiso}{\basicSwiso[59]}}%

% south-west isomorphism with lower name [1]  and length nx100 units
\def\basicswisO[#1]#2{\fdcase{\SWAR}{\hspace{-2pt}\cong}{#2}{#100}}%

% south-west isomorphism with lower name [1]
\newcommand{\swisO}{\@ifnextchar[{\basicswisO}{\basicswisO[59]}}%

% south-west equality
\let\sweql\neeql%

% south-west equality with upper name [1]
\let\Sweql=\Neeql%

% south-west equality with lower name [1]
\let\sweqL=\neeqL%

% pair of south-west arrows of length nx100 units
\def\basicswbiar[#1]{\fdbicase{\SWBIAR}{}{}{#100}}%

% pair of south-west arrows
\newcommand{\swbiar}{\@ifnextchar[{\basicswbiar}{\basicswbiar[59]}}%

% pair of south-west arrows with names [1][2] and length nx100 units
\def\basicSwbiar[#1]#2#3{\fdbicase{\SWBIAR}{#2}{#3}{#100}}%

% pair of south-west arrows with names
\newcommand{\Swbiar}{\@ifnextchar[{\basicSwbiar}{\basicSwbiar[59]}}%
\let\swbiaR=\Swbiar

% pair of south-west adjoint arrows of length nx100 units
\def\basicswadjar[#1]{\fdbicase{\SWADJAR}{}{}{#100}}%

% pair of south-west adjoint arrows
\newcommand{\swadjar}{\@ifnextchar[{\basicswadjar}{\basicswadjar[59]}}%

% pair of south-west adjoint arrows with names [1][2] and length nx100 units
\def\basicSwadjar[#1]#2#3{\fdbicase{\SWADJAR}{#2}{#3}{#100}}%

% pair of south-west adjoint arrows with names
\newcommand{\Swadjar}{\@ifnextchar[{\basicSwadjar}{\basicSwadjar[59]}}%
\let\swadjaR=\Swadjar

% pair of south-west distributors of length nx100 units
\def\basicswbidist[#1]{\fdbicase{\SWBIDIST}{}{}{#100}}%

% pair of south-west distributors
\newcommand{\swbidist}{\@ifnextchar[{\basicswbidist}{\basicswbidist[59]}}%

% pair of south-west distributors with names [1][2] and length nx100 units
\def\basicSwbidist[#1]#2#3{\fdbicase{\SWBIDIST}{#2}{#3}{#100}}%

% pair of south-west distributors with names
\newcommand{\Swbidist}{\@ifnextchar[{\basicSwbidist}{\basicSwbidist[59]}}%
\let\swbidisT=\Swbidist

% pair of south-west adjoint distributors of length nx100 units
\def\basicswadjdist[#1]{\fdbicase{\SWADJDIST}{}{}{#100}}%

% pair of south-west adjoint distributors
\newcommand{\swadjdist}{\@ifnextchar[{\basicswadjdist}{\basicswadjdist[59]}}%

% pair of south-west adjoint distributors with names [1][2] and length nx100 units
\def\basicSwadjdist[#1]#2#3{\fdbicase{\SWADJDIST}{#2}{#3}{#100}}%

% pair of south-west adjoint distributors with names
\newcommand{\Swadjdist}{\@ifnextchar[{\basicSwadjdist}{\basicSwadjdist[59]}}%
\let\swadjdisT=\Swadjdist



% MACROS FOR  SECOND DIAGONAL PICTURES

% \sdcase{P}{f}{g}{n} draws the picture P with names f, g
% and length n units
\newcommand{\sdcase}[4]{\testdiagrammode\begin{picture}(0,0)%
\put(0,0){#1{#4}}%
\truex{100}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#2}$}}%
\truex{300}\truey{800}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#3}$}}%
\end{picture}}%

% \sdbicase{P}{f}{g}{n} draws the bipicture P with names f, g
% and length n units
\newcommand{\sdbicase}[4]{\testdiagrammode\begin{picture}(0,0)%
\put(0,0){#1{#4}}%
\truex{350}\truey{600}\truez{950}%
\put(\value{x},\value{x}){\makebox(0,\value{y})[l]{${#2}$}}%
\truex{450}\truey{600}\truez{1050}%
\put(-\value{x},-\value{z}){\makebox(0,\value{y})[r]{${#3}$}}%
\end{picture}}%


% SOUTH-EAST ARROWS

% \SEAR{n} draws a south-east arrow of length nx100 units
\newcommand{\SEAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,\Y){\line(1,-1){#1}}%
\put(\Y,-\Y){\sehead}%
\end{picture}}%

% \SEDIST{n} draws a south-east distributor of length n units
\newcommand{\SEDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,\Y){\line(1,-1){#1}}%
\put(\Y,-\Y){\sehead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\end{picture}}%

% \SEDOTAR{n} draws a south-east dotted arrow of length n units
\newcommand{\SEDOTAR}[1]%
{\truex{100}\truey{212}%
\Y=#1%
\divide\Y by 2%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(-\Y,\Y)(\value{y},-\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(\Y,-\Y){\sehead}%
\end{picture}}%

% \SEMONO{n} draws a south-east monomorphism of length n units
\newcommand{\SEMONO}[1]{%
\Y=#1%
\divide \Y by 2%
\Truetail%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\begin{picture}(0,0)%
\put(-\monolength,\monolength){\line(1,-1){\bimolength}}%
\put(-\monolength,\monolength){\sehead}%
\put(\Y,-\Y){\sehead}%
\end{picture}}%

% \SEEPI{n} draws a south-east epimorphism of length n units
\newcommand{\SEEPI}[1]{%
\Y=#1%
\divide\Y by 2%
\Truehead%
\bimolength=#1%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\begin{picture}(0,0)%
\put(-\Y,\Y){\line(1,-1){\bimolength}}%
\put(\epilength,-\epilength){\sehead}%
\put(\Y,-\Y){\sehead}%
\end{picture}}%

% \SEBIMO{n} draws a south-east bimorphism of length n units
\newcommand{\SEBIMO}[1]{%
\Y=#1%
\divide\Y by 2%
\Truetail\Truehead%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\begin{picture}(0,0)%
\put(-\monolength,\monolength){\line(1,-1){\bimolength}}%
\put(-\monolength,\monolength){\sehead}%
\put(\epilength,-\epilength){\sehead}%
\put(\Y,-\Y){\sehead}%
\end{picture}}%

% \SEBIAR{n} draws a pair of south-east arrows of length n units
\newcommand{\SEBIAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\put(-\value{x},-\value{x}){\line(1,-1){#1}}%
\put(\value{x},\value{x}){\line(1,-1){#1}}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\monolength,-\epilength){\sehead}%
\put(\epilength,-\monolength){\sehead}%
\end{picture}}\end{picture}}%

% \SEBIDIST{n} draws a pair of south-east distributors of length n units
\newcommand{\SEBIDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},\value{x}){\line(1,-1){#1}}%
\put(\epilength,-\monolength){\sehead}%
\end{picture}}%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by \value{x}%
\epilength=#1%
\advance\epilength by -\value{x}%
\put(-\value{x},-\value{x}){\line(1,-1){#1}}%
\put(\epilength,-\monolength){\sehead}%
\end{picture}}%
\put(-\value{x},-\value{x}){\circle{\value{y}}}%
\put(\value{x},\value{x}){\circle{\value{y}}}%
\end{picture}}%

% \SEEQL{n} draws a south-east equality of length n units
\newcommand{\SEEQL}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{70}%
\put(-\value{x},-\value{x}){\line(1,-1){#1}}%
\put(\value{x},\value{x}){\line(1,-1){#1}}%
\end{picture}}\end{picture}}%

% \SEADJAR{n} draws a south-east pair of adjoint arrows of length n units
\newcommand{\SEADJAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},-\value{x}){\line(1,-1){#1}}%
\put(\monolength,-\epilength){\sehead}%
\end{picture}}%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},\value{x}){\line(-1,1){#1}}%
\put(-\monolength,\epilength){\nwhead}%
\end{picture}}\end{picture}}%

% \SEADJDIST{n} draws a south-east pair of adjoint distributors of length n units
\newcommand{\SEADJDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},-\value{x}){\line(1,-1){#1}}%
\put(\monolength,-\epilength){\sehead}%
\end{picture}}%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},\value{x}){\line(-1,1){#1}}%
\put(-\monolength,\epilength){\nwhead}%
\end{picture}}%
\put(-\value{x},-\value{x}){\circle{\value{y}}}%
\put(\value{x},\value{x}){\circle{\value{y}}}%
\end{picture}}%


% All the following commands draw south-east arrows

% south-east arrow of length nx100 units
\def\basicsear[#1]{\sdcase{\SEAR}{}{}{#100}}%

% south-east arrow
\newcommand{\sear}{\@ifnextchar[{\basicsear}{\basicsear[59]}}%

% south-east arrow with upper name [1] and length nx100 units
\def\basicSear[#1]#2{\sdcase{\SEAR}{#2}{}{#100}}%

% south-east arrow with upper name
\newcommand{\Sear}{\@ifnextchar[{\basicSear}{\basicSear[59]}}%

% south-east arrow with lower name [1]  and length nx100 units
\def\basicseaR[#1]#2{\sdcase{\SEAR}{}{#2}{#100}}%

% south-east arrow with lower name [1]
\newcommand{\seaR}{\@ifnextchar[{\basicseaR}{\basicseaR[59]}}%

% south-east distributor of length nx100 units
\def\basicsedist[#1]{\sdcase{\SEDIST}{}{}{#100}}%

% south-east distributor
\newcommand{\sedist}{\@ifnextchar[{\basicsedist}{\basicsedist[59]}}%

% south-east distributor with upper name [1] and length nx100 units
\def\basicSedist[#1]#2{\sdcase{\SEDIST}{#2}{}{#100}}%

% south-east distributor with upper name
\newcommand{\Sedist}{\@ifnextchar[{\basicSedist}{\basicSedist[59]}}%

% south-east distributor with lower name [1]  and length nx100 units
\def\basicsedisT[#1]#2{\sdcase{\SEDIST}{}{#2}{#100}}%

% south-east distributor with lower name [1]
\newcommand{\sedisT}{\@ifnextchar[{\basicsedisT}{\basicsedisT[59]}}%

% south-east dotted arrow of length nx100 units
\def\basicsedotar[#1]{\sdcase{\SEDOTAR}{}{}{#100}}%

% south-east dotted arrow
\newcommand{\sedotar}{\@ifnextchar[{\basicsedotar}{\basicsedotar[59]}}%

% south-east dotted arrow with upper name [1] and length nx100 units
\def\basicSedotar[#1]#2{\sdcase{\SEDOTAR}{#2}{}{#100}}%

% south-east dotted arrow with upper name
\newcommand{\Sedotar}{\@ifnextchar[{\basicSedotar}{\basicSedotar[59]}}%

% south-east dotted arrow with lower name [1]  and length nx100 units
\def\basicsedotaR[#1]#2{\sdcase{\SEDOTAR}{}{#2}{#100}}%

% south-east dotted arrow with lower name [1]
\newcommand{\sedotaR}{\@ifnextchar[{\basicsedotaR}{\basicsedotaR[59]}}%

% south-east monomorphism of length nx100 units
\def\basicsemono[#1]{\sdcase{\SEMONO}{}{}{#100}}%

% south-east monomorphism
\newcommand{\semono}{\@ifnextchar[{\basicsemono}{\basicsemono[59]}}%

% south-east monomorphism with upper name [1] and length nx100 units
\def\basicSemono[#1]#2{\sdcase{\SEMONO}{#2}{}{#100}}%

% south-east monomophism with upper name
\newcommand{\Semono}{\@ifnextchar[{\basicSemono}{\basicSemono[59]}}%

% south-east monomorphism with lower name [1]  and length nx100 units
\def\basicsemonO[#1]#2{\sdcase{\SEMONO}{}{#2}{#100}}%

% south-east monomorphism with lower name [1]
\newcommand{\semonO}{\@ifnextchar[{\basicsemonO}{\basicsemonO[59]}}%

% south-east epimorphism of length nx100 units
\def\basicseepi[#1]{\sdcase{\SEEPI}{}{}{#100}}%

% south-east epimorphism
\newcommand{\seepi}{\@ifnextchar[{\basicseepi}{\basicseepi[59]}}%

% south-east epimorphism with upper name [1] and length nx100 units
\def\basicSeepi[#1]#2{\sdcase{\SEEPI}{#2}{}{#100}}%

% south-east epimorphism with upper name
\newcommand{\Seepi}{\@ifnextchar[{\basicSeepi}{\basicSeepi[59]}}%

% south-east epimorphism with lower name [1]  and length nx100 units
\def\basicseepI[#1]#2{\sdcase{\SEEPI}{}{#2}{#100}}%

% south-east epimorphism with lower name [1]
\newcommand{\seepI}{\@ifnextchar[{\basicseepI}{\basicseepI[59]}}%

% south-east bimorphism of length nx100 units
\def\basicsebimo[#1]{\sdcase{\SEBIMO}{}{}{#100}}%

% south-east bimorphism
\newcommand{\sebimo}{\@ifnextchar[{\basicsebimo}{\basicsebimo[59]}}%

% south-east bimorphism with upper name [1] and length nx100 units
\def\basicSebimo[#1]#2{\sdcase{\SEBIMO}{#2}{}{#100}}%

% south-east bimorphism with upper name
\newcommand{\Sebimo}{\@ifnextchar[{\basicSebimo}{\basicSebimo[59]}}%

% south-east bimorphism with lower name [1]  and length nx100 units
\def\basicsebimO[#1]#2{\sdcase{\SEBIMO}{}{#2}{#100}}%

% south-east bimorphism with lower name [1]
\newcommand{\sebimO}{\@ifnextchar[{\basicsebimO}{\basicsebimO[59]}}%

% south-east isomorphism of length nx100 units
\def\basicseiso[#1]{\sdcase{\SEAR}{\hspace{-2pt}\cong}{}{#100}}%

% south-east isomorphism
\newcommand{\seiso}{\@ifnextchar[{\basicseiso}{\basicseiso[59]}}%

% south-east isomorphism with upper name [1] and length nx100 units
\def\basicSeiso[#1]#2{\sdcase{\SEAR}{#2}{\cong}{#100}}%

% south-east isomorphism with upper name
\newcommand{\Seiso}{\@ifnextchar[{\basicSeiso}{\basicSeiso[59]}}%

% south-east isomorphism with lower name [1]  and length nx100 units
\def\basicseisO[#1]#2{\sdcase{\SEAR}{\hspace{-2pt}\cong}{#2}{#100}}%

% south-east isomorphism with lower name [1]
\newcommand{\seisO}{\@ifnextchar[{\basicseisO}{\basicseisO[59]}}%

% south-east equality of length nx100 units
\def\basicseeql[#1]{\sdcase{\SEEQL}{}{}{#100}}%

% south-east equality
\newcommand{\seeql}{\@ifnextchar[{\basicseeql}{\basicseeql[59]}}%

% south-east equality with upper name [1] and length nx100 units
\def\basicSeeql[#1]#2{\sdcase{\SEEQL}{#2}{}{#100}}%

% south-east equality with upper name
\newcommand{\Seeql}{\@ifnextchar[{\basicSeeql}{\basicSeeql[59]}}%

% south-east equality with lower name [1]  and length nx100 units
\def\basicseeqL[#1]#2{\sdcase{\SEEQL}{}{#2}{#100}}%

% south-east equality with lower name [1]
\newcommand{\seeqL}{\@ifnextchar[{\basicseeqL}{\basicseeqL[59]}}%

% pair of south-east arrows of length nx100 units
\def\basicsebiar[#1]{\sdbicase{\SEBIAR}{}{}{#100}}%

% pair of south-east arrows
\newcommand{\sebiar}{\@ifnextchar[{\basicsebiar}{\basicsebiar[59]}}%

% pair of south-east arrows with names [1][2] and length nx100 units
\def\basicSebiar[#1]#2#3{\sdbicase{\SEBIAR}{#2}{#3}{#100}}%

% pair of south-east arrows with names
\newcommand{\Sebiar}{\@ifnextchar[{\basicSebiar}{\basicSebiar[59]}}%
\let\sebiaR=\Sebiar

% pair of south-east adjoint arrows of length nx100 units
\def\basicseadjar[#1]{\sdbicase{\SEADJAR}{}{}{#100}}%

% pair of south-east adjoint arrows
\newcommand{\seadjar}{\@ifnextchar[{\basicseadjar}{\basicseadjar[59]}}%

% pair of south-east adjoint arrows with names [1][2] and length nx100 units
\def\basicSeadjar[#1]#2#3{\sdbicase{\SEADJAR}{#2}{#3}{#100}}%

% pair of south-east adjoint arrows with names
\newcommand{\Seadjar}{\@ifnextchar[{\basicSeadjar}{\basicSeadjar[59]}}%
\let\seadjaR=\Seadjar

% pair of south-east distributors of length nx100 units
\def\basicsebidist[#1]{\sdbicase{\SEBIDIST}{}{}{#100}}%

% pair of south-east distributors
\newcommand{\sebidist}{\@ifnextchar[{\basicsebidist}{\basicsebidist[59]}}%

% pair of south-east distributors with names [1][2] and length nx100 units
\def\basicSebidist[#1]#2#3{\sdbicase{\SEBIDIST}{#2}{#3}{#100}}%

% pair of south-east distributors with names
\newcommand{\Sebidist}{\@ifnextchar[{\basicSebidist}{\basicSebidist[59]}}%
\let\sebidisT=\Sebidist

% pair of south-east adjoint distributors of length nx100 units
\def\basicseadjdist[#1]{\sdbicase{\SEADJDIST}{}{}{#100}}%

% pair of south-east adjoint distributors
\newcommand{\seadjdist}{\@ifnextchar[{\basicseadjdist}{\basicseadjdist[59]}}%

% pair of south-east adjoint distributors with names [1][2] and length nx100 units
\def\basicSeadjdist[#1]#2#3{\sdbicase{\SEADJDIST}{#2}{#3}{#100}}%

% pair of south-east adjoint distributors with names
\newcommand{\Seadjdist}{\@ifnextchar[{\basicSeadjdist}{\basicSeadjdist[59]}}%
\let\seadjdisT=\Seadjdist


% NORTH-WEST ARROWS

% \NWAR{n} draws a north-west arrow of length nx100 units
\newcommand{\NWAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,-\Y){\line(-1,1){#1}}%
\put(-\Y,\Y){\nwhead}%
\end{picture}}%

% \NWDIST{n} draws a north-west distributor of length n units
\newcommand{\NWDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,-\Y){\line(-1,1){#1}}%
\put(-\Y,\Y){\nwhead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\end{picture}}%

% \NWDOTAR{n} draws a north-west dotted arrow of length n units
\newcommand{\NWDOTAR}[1]%
{\truex{100}\truey{212}%
\Y=#1%
\divide\Y by 2%
\NUMBEROFDOTS=#1%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(\Y,-\Y)(-\value{y},\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(-\Y,\Y){\nwhead}%
\end{picture}}%

% \NWMONO{n} draws a north-west monomorphism of length n units
\newcommand{\NWMONO}[1]{%
\Y=#1%
\divide \Y by 2%
\Truetail%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\begin{picture}(0,0)%
\put(\monolength,-\monolength){\line(-1,1){\bimolength}}%
\put(\monolength,-\monolength){\nwhead}%
\put(-\Y,\Y){\nwhead}%
\end{picture}}%

% \NWEPI{n} draws a north-west epimorphism of length n units
\newcommand{\NWEPI}[1]{%
\Y=#1%
\divide\Y by 2%
\Truehead%
\bimolength=#1%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\begin{picture}(0,0)%
\put(\Y,-\Y){\line(-1,1){\bimolength}}%
\put(-\epilength,\epilength){\nwhead}%
\put(-\Y,\Y){\nwhead}%
\end{picture}}%

% \NWBIMO{n} draws a north-west bimorphism of length n units
\newcommand{\NWBIMO}[1]{%
\Y=#1%
\divide\Y by 2%
\Truetail\Truehead%
\bimolength=#1%
\advance\bimolength by -\Truemonotail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\Trueepihead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\begin{picture}(0,0)%
\put(\monolength,-\monolength){\line(-1,1){\bimolength}}%
\put(\monolength,-\monolength){\nwhead}%
\put(-\epilength,\epilength){\nwhead}%
\put(-\Y,\Y){\nwhead}%
\end{picture}}%

% \NWBIAR{n} draws a pair of north-west arrows of length n units
\newcommand{\NWBIAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\put(-\value{x},-\value{x}){\line(-1,1){#1}}%
\put(\value{x},\value{x}){\line(-1,1){#1}}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\monolength,\epilength){\nwhead}%
\put(-\epilength,\monolength){\nwhead}%
\end{picture}}\end{picture}}%

% \NWBIDIST{n} draws a pair of north-west distributors of length n units
\newcommand{\NWBIDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},-\value{x}){\line(-1,1){#1}}%
\put(-\epilength,\monolength){\nwhead}%
\end{picture}}%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by \value{x}%
\epilength=#1%
\advance\epilength by -\value{x}%
\put(\value{x},\value{x}){\line(-1,1){#1}}%
\put(-\epilength,\monolength){\nwhead}%
\end{picture}}%
\put(-\value{x},-\value{x}){\circle{\value{y}}}%
\put(\value{x},\value{x}){\circle{\value{y}}}%
\end{picture}}%

% \NWADJAR{n} draws a north-west pair of adjoint arrows of length n units
\newcommand{\NWADJAR}[1]{%
\Y=#1%
\divide\Y by 2%
\begin{picture}(0,0)%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},-\value{x}){\line(-1,1){#1}}%
\put(-\epilength,\monolength){\nwhead}%
\end{picture}}%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},\value{x}){\line(1,-1){#1}}%
\put(\epilength,-\monolength){\sehead}%
\end{picture}}\end{picture}}%

% \NWADJDIST{n} draws a north-west pair of adjoint distributors of length n units
\newcommand{\NWADJDIST}[1]{%
\Y=#1%
\divide\Y by 2%
\truey{400}%
\begin{picture}(0,0)%
\put(\Y,-\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(-\value{x},-\value{x}){\line(-1,1){#1}}%
\put(-\epilength,\monolength){\nwhead}%
\end{picture}}%
\put(-\Y,\Y){\begin{picture}(0,0)%
\truex{247}%
\monolength=#1%
\advance\monolength by -\value{x}%
\epilength=#1%
\advance\epilength by \value{x}%
\put(\value{x},\value{x}){\line(1,-1){#1}}%
\put(\epilength,-\monolength){\sehead}%
\end{picture}}%
\put(-\value{x},-\value{x}){\circle{\value{y}}}%
\put(\value{x},\value{x}){\circle{\value{y}}}%
\end{picture}}%


% All the following commands draw north-west arrows

% north-west arrow of length nx100 units
\def\basicnwar[#1]{\sdcase{\NWAR}{}{}{#100}}%

% north-west arrow
\newcommand{\nwar}{\@ifnextchar[{\basicnwar}{\basicnwar[59]}}%

% north-west arrow with upper name [1] and length nx100 units
\def\basicNwar[#1]#2{\sdcase{\NWAR}{#2}{}{#100}}%

% north-west arrow with upper name
\newcommand{\Nwar}{\@ifnextchar[{\basicNwar}{\basicNwar[59]}}%

% north-west arrow with lower name [1]  and length nx100 units
\def\basicnwaR[#1]#2{\sdcase{\NWAR}{}{#2}{#100}}%

% north-west arrow with lower name [1]
\newcommand{\nwaR}{\@ifnextchar[{\basicnwaR}{\basicnwaR[59]}}%

% north-west distributor of length nx100 units
\def\basicnwdist[#1]{\sdcase{\NWDIST}{}{}{#100}}%

% north-west distributor
\newcommand{\nwdist}{\@ifnextchar[{\basicnwdist}{\basicnwdist[59]}}%

% north-west distributor with upper name [1] and length nx100 units
\def\basicNwdist[#1]#2{\sdcase{\NWDIST}{#2}{}{#100}}%

% north-west distributor with upper name
\newcommand{\Nwdist}{\@ifnextchar[{\basicNwdist}{\basicNwdist[59]}}%

% north-west distributor with lower name [1]  and length nx100 units
\def\basicnwdisT[#1]#2{\sdcase{\NWDIST}{}{#2}{#100}}%

% north-west distributor with lower name [1]
\newcommand{\nwdisT}{\@ifnextchar[{\basicnwdisT}{\basicnwdisT[59]}}%

% north-west dotted arrow of length nx100 units
\def\basicnwdotar[#1]{\sdcase{\NWDOTAR}{}{}{#100}}%

% north-west dotted arrow
\newcommand{\nwdotar}{\@ifnextchar[{\basicnwdotar}{\basicnwdotar[59]}}%

% north-west dotted arrow with upper name [1] and length nx100 units
\def\basicNwdotar[#1]#2{\sdcase{\NWDOTAR}{#2}{}{#100}}%

% north-west dotted arrow with upper name
\newcommand{\Nwdotar}{\@ifnextchar[{\basicNwdotar}{\basicNwdotar[59]}}%

% north-west dotted arrow with lower name [1]  and length nx100 units
\def\basicnwdotaR[#1]#2{\sdcase{\NWDOTAR}{}{#2}{#100}}%

% north-west dotted arrow with lower name [1]
\newcommand{\nwdotaR}{\@ifnextchar[{\basicnwdotaR}{\basicnwdotaR[59]}}%

% north-west monomorphism of length nx100 units
\def\basicnwmono[#1]{\sdcase{\NWMONO}{}{}{#100}}%

% north-west monomorphism
\newcommand{\nwmono}{\@ifnextchar[{\basicnwmono}{\basicnwmono[59]}}%

% north-west monomorphism with upper name [1] and length nx100 units
\def\basicNwmono[#1]#2{\sdcase{\NWMONO}{#2}{}{#100}}%

% north-west monomophism with upper name
\newcommand{\Nwmono}{\@ifnextchar[{\basicNwmono}{\basicNwmono[59]}}%

% north-west monomorphism with lower name [1]  and length nx100 units
\def\basicnwmonO[#1]#2{\sdcase{\NWMONO}{}{#2}{#100}}%

% north-west monomorphism with lower name [1]
\newcommand{\nwmonO}{\@ifnextchar[{\basicnwmonO}{\basicnwmonO[59]}}%

% north-west epimorphism of length nx100 units
\def\basicnwepi[#1]{\sdcase{\NWEPI}{}{}{#100}}%

% north-west epimorphism
\newcommand{\nwepi}{\@ifnextchar[{\basicnwepi}{\basicnwepi[59]}}%

% north-west epimorphism with upper name [1] and length nx100 units
\def\basicNwepi[#1]#2{\sdcase{\NWEPI}{#2}{}{#100}}%

% north-west epimorphism with upper name
\newcommand{\Nwepi}{\@ifnextchar[{\basicNwepi}{\basicNwepi[59]}}%

% north-west epimorphism with lower name [1]  and length nx100 units
\def\basicnwepI[#1]#2{\sdcase{\NWEPI}{}{#2}{#100}}%

% north-west epimorphism with lower name [1]
\newcommand{\nwepI}{\@ifnextchar[{\basicnwepI}{\basicnwepI[59]}}%

% north-west bimorphism of length nx100 units
\def\basicnwbimo[#1]{\sdcase{\NWBIMO}{}{}{#100}}%

% north-west bimorphism
\newcommand{\nwbimo}{\@ifnextchar[{\basicnwbimo}{\basicnwbimo[59]}}%

% north-west bimorphism with upper name [1] and length nx100 units
\def\basicNwbimo[#1]#2{\sdcase{\NWBIMO}{#2}{}{#100}}%

% north-west bimorphism with upper name
\newcommand{\Nwbimo}{\@ifnextchar[{\basicNwbimo}{\basicNwbimo[59]}}%

% north-west bimorphism with lower name [1]  and length nx100 units
\def\basicnwbimO[#1]#2{\sdcase{\NWBIMO}{}{#2}{#100}}%

% north-west bimorphism with lower name [1]
\newcommand{\nwbimO}{\@ifnextchar[{\basicnwbimO}{\basicnwbimO[59]}}%

% north-west isomorphism of length nx100 units
\def\basicnwiso[#1]{\sdcase{\NWAR}{\hspace{-2pt}\cong}{}{#100}}%

% north-west isomorphism
\newcommand{\nwiso}{\@ifnextchar[{\basicnwiso}{\basicnwiso[59]}}%

% north-west isomorphism with upper name [1] and length nx100 units
\def\basicNwiso[#1]#2{\sdcase{\NWAR}{#2}{\cong}{#100}}%

% north-west isomorphism with upper name
\newcommand{\Nwiso}{\@ifnextchar[{\basicNwiso}{\basicNwiso[59]}}%

% north-west isomorphism with lower name [1]  and length nx100 units
\def\basicnwisO[#1]#2{\sdcase{\NWAR}{\hspace{-2pt}\cong}{#2}{#100}}%

% north-west isomorphism with lower name [1]
\newcommand{\nwisO}{\@ifnextchar[{\basicnwisO}{\basicnwisO[59]}}%

% north-west equality
\let\nweql=\seeql%

% north-west equality with upper name
\let\Nweql=\Seeql%

% north-west equality with lower name [1]
\let\nweqL=\seeqL%

% pair of north-west arrows of length nx100 units
\def\basicnwbiar[#1]{\sdbicase{\NWBIAR}{}{}{#100}}%

% pair of north-west arrows
\newcommand{\nwbiar}{\@ifnextchar[{\basicnwbiar}{\basicnwbiar[59]}}%

% pair of north-west arrows with names [1][2] and length nx100 units
\def\basicNwbiar[#1]#2#3{\sdbicase{\NWBIAR}{#2}{#3}{#100}}%

% pair of north-west arrows with names
\newcommand{\Nwbiar}{\@ifnextchar[{\basicNwbiar}{\basicNwbiar[59]}}%
\let\nwbiaR=\Nwbiar

% pair of north-west adjoint arrows of length nx100 units
\def\basicnwadjar[#1]{\sdbicase{\NWADJAR}{}{}{#100}}%

% pair of north-west adjoint arrows
\newcommand{\nwadjar}{\@ifnextchar[{\basicnwadjar}{\basicnwadjar[59]}}%

% pair of north-west adjoint arrows with names [1][2] and length nx100 units
\def\basicNwadjar[#1]#2#3{\sdbicase{\NWADJAR}{#2}{#3}{#100}}%

% pair of north-west adjoint arrows with names
\newcommand{\Nwadjar}{\@ifnextchar[{\basicNwadjar}{\basicNwadjar[59]}}%
\let\nwadjaR=\Nwadjar

% pair of north-west distributors of length nx100 units
\def\basicnwbidist[#1]{\sdbicase{\NWBIDIST}{}{}{#100}}%

% pair of north-west distributors
\newcommand{\nwbidist}{\@ifnextchar[{\basicnwbidist}{\basicnwbidist[59]}}%

% pair of north-west distributors with names [1][2] and length nx100 units
\def\basicNwbidist[#1]#2#3{\sdbicase{\NWBIDIST}{#2}{#3}{#100}}%

% pair of north-west distributors with names
\newcommand{\Nwbidist}{\@ifnextchar[{\basicNwbidist}{\basicNwbidist[59]}}%
\let\nwbidisT=\Nwbidist

% pair of north-west adjoint distributors of length nx100 units
\def\basicnwadjdist[#1]{\sdbicase{\NWADJDIST}{}{}{#100}}%

% pair of north-west adjoint distributors
\newcommand{\nwadjdist}{\@ifnextchar[{\basicnwadjdist}{\basicnwadjdist[59]}}%

% pair of north-west adjoint distributors with names [1][2] and length nx100 units
\def\basicNwadjdist[#1]#2#3{\sdbicase{\NWADJDIST}{#2}{#3}{#100}}%

% pair of north-west adjoint distributors with names
\newcommand{\Nwadjdist}{\@ifnextchar[{\basicNwadjdist}{\basicNwadjdist[59]}}%
\let\nwadjdisT=\Nwadjdist


% EAST-NORTH-EAST ARROWS

% The following commands produce east-north-east arrows
% of horizontal extent n units

% \ENEAR{f}{g}{n} draws a east-north-east arrow with names f, g
% and length n units
\newcommand{\ENEAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(2,1){#3}}%
\put(\Y,\Z){\enehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEDIST{f}{g}{n} draws a east-north-east distributor
% with names f, g and length n units
\newcommand{\ENEDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(2,1){#3}}%
\put(\Y,\Z){\enehead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\ENEDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(-\Y,-\Z)(\value{y},\value{z}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(\Y,\Z){\enehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEMONO{f}{g}{n} draws a east-north-east monomorphism
% with names f,g and length n units
\newcommand{\ENEMONO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\begin{picture}(0,0)%
\put(-\monolength,-\secondmonolength){\line(2,1){\bimolength}}%
\put(-\monolength,-\secondmonolength){\enehead}%
\put(\Y,\Z){\enehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEEPI{f}{g}{n} draws a east-north-east epimorphism
% with names f, g and length n units
\newcommand{\ENEEPI}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(2,1){\bimolength}}%
\put(\epilength,\secondepilength){\enehead}%
\put(\Y,\Z){\enehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEBIMO{f}{g}{n} draws a east-north-east bimorphism
% with names f,g and length n units
\newcommand{\ENEBIMO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\monolength,-\secondmonolength){\line(2,1){\bimolength}}%
\put(-\monolength,-\secondmonolength){\enehead}%
\put(\epilength,\secondepilength){\enehead}%
\put(\Y,\Z){\enehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEEQL{f}{g}{n} draws a east-north-east equality
% with names f,g and length n units
\newcommand{\ENEEQL}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\begin{picture}(0,0)%
\truex{44}\truey{89}%
\put(-\value{x},\value{y}){\line(2,1){#3}}%
\put(\value{x},-\value{y}){\line(2,1){#3}}%
\end{picture}}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEBIAR{f}{g}{n} draws a pair of east-north-east arrows
% with names f,g and length n units
\newcommand{\ENEBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\put(-\value{x},\value{y}){\line(2,1){#3}}%
\put(\value{x},-\value{y}){\line(2,1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\monolength,\secondepilength){\enehead}%
\put(\epilength,\secondmonolength){\enehead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEBIDIST{f}{g}{n} draws a pair of east-north-east distributors
% with names f,g and length n units
\newcommand{\ENEBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(-\Y,-\Z){\begin{picture}(0,0)%
\put(-\value{x},\value{y}){\line(2,1){#3}}%
\put(\value{x},-\value{y}){\line(2,1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\monolength,\secondepilength){\enehead}%
\put(\epilength,\secondmonolength){\enehead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEADJAR{f}{g}{n} draws a east-north-east pair of adjoint arrows
% with names f,g and length n units
\newcommand{\ENEADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(2,1){#3}}%
\put(\epilength,\secondmonolength){\enehead}%
\put(\monolength,\secondepilength){\line(-2,-1){#3}}%
\put(-\value{x},\value{y}){\wswhead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \ENEADJDIST{f}{g}{n} draws a east-north-east pair of adjoint distributors
% with names f,g and length n units
\newcommand{\ENEADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(-\Y,-\Z){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(2,1){#3}}%
\put(\epilength,\secondmonolength){\enehead}%
\put(\monolength,\secondepilength){\line(-2,-1){#3}}%
\put(-\value{x},\value{y}){\wswhead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% The following commands produce east-north-east arrows;
% the default length is 13300 units

% basic east-north-east arrow
\def\basicenear[#1]{\ENEAR{}{}{#100}}%

% east-north-east arrow
\newcommand{\enear}{\@ifnextchar[{\basicenear}{\basicenear[133]}}%

% basic east-north-east arrow with upper name
\def\basicEnear[#1]#2{\ENEAR{#2}{}{#100}}%

% east-north-east arrow with upper name
\newcommand{\Enear}{\@ifnextchar[{\basicEnear}{\basicEnear[133]}}%

% basic east-north-east arrow with lower name
\def\basiceneaR[#1]#2{\ENEAR{}{#2}{#100}}%

% east-north-east arrow with lower name
\newcommand{\eneaR}{\@ifnextchar[{\basiceneaR}{\basiceneaR[133]}}%

% basic east-north-east distributor
\def\basicenedist[#1]{\ENEDIST{}{}{#100}}%

% east-north-east distributor
\newcommand{\enedist}{\@ifnextchar[{\basicenedist}{\basicenedist[133]}}%

% basic east-north-east distributor with upper name
\def\basicEnedist[#1]#2{\ENEDIST{#2}{}{#100}}%

% east-north-east distributor with upper name
\newcommand{\Enedist}{\@ifnextchar[{\basicEnedist}{\basicEnedist[133]}}%

% basic east-north-east distributor with lower name
\def\basicenedisT[#1]#2{\ENEDIST{}{#2}{#100}}%

% east-north-east distributor with lower name
\newcommand{\enedisT}{\@ifnextchar[{\basicenedisT}{\basicenedisT[133]}}%

% basic east-north-east dotted arrow
\def\basicenedotar[#1]{\ENEDOTAR{}{}{#100}}%

% east-north-east dotted arrow
\newcommand{\enedotar}{\@ifnextchar[{\basicenedotar}{\basicenedotar[133]}}%

% basic east-north-east dotted arrow with upper name
\def\basicEnedotar[#1]#2{\ENEDOTAR{#2}{}{#100}}%

% east-north-east dotted arrow with upper name
\newcommand{\Enedotar}{\@ifnextchar[{\basicEnedotar}{\basicEnedotar[133]}}%

% basic east-north-east dotted arrow with lower name
\def\basicenedotaR[#1]#2{\ENEDOTAR{}{#2}{#100}}%

% east-north-east dotted arrow with lower name
\newcommand{\enedotaR}{\@ifnextchar[{\basicenedotaR}{\basicenedotaR[133]}}%

% basic east-north-east monomorphism
\def\basicenemono[#1]{\ENEMONO{}{}{#100}}%

% east-north-east monomorphism
\newcommand{\enemono}{\@ifnextchar[{\basicenemono}{\basicenemono[133]}}%

% basic east-north-east monomorphism with upper name
\def\basicEnemono[#1]#2{\ENEMONO{#2}{}{#100}}%

% east-north-east monomorphism with upper name
\newcommand{\Enemono}{\@ifnextchar[{\basicEnemono}{\basicEnemono[133]}}%

% basic east-north-east monomorphism with lower name
\def\basicenemonO[#1]#2{\ENEMONO{}{#2}{#100}}%

% east-north-east monomorphism with lower name
\newcommand{\enemonO}{\@ifnextchar[{\basicenemonO}{\basicenemonO[133]}}%

% basic east-north-east epimorphism
\def\basiceneepi[#1]{\ENEEPI{}{}{#100}}%

% east-north-east epimorphism
\newcommand{\eneepi}{\@ifnextchar[{\basiceneepi}{\basiceneepi[133]}}%

% basic east-north-east epimorphism with upper name
\def\basicEneepi[#1]#2{\ENEEPI{#2}{}{#100}}%

% east-north-east epimorphism with upper name
\newcommand{\Eneepi}{\@ifnextchar[{\basicEneepi}{\basicEneepi[133]}}%

% basic east-north-east epimorphism with lower name
\def\basiceneepI[#1]#2{\ENEEPI{}{#2}{#100}}%

% east-north-east epimorphism with lower name
\newcommand{\eneepI}{\@ifnextchar[{\basiceneepI}{\basiceneepI[133]}}%

% basic east-north-east bimorphism
\def\basicenebimo[#1]{\ENEBIMO{}{}{#100}}%

% east-north-east bimorphism
\newcommand{\enebimo}{\@ifnextchar[{\basicenebimo}{\basicenebimo[133]}}%

% basic east-north-east bimorphism with upper name
\def\basicEnebimo[#1]#2{\ENEBIMO{#2}{}{#100}}%

% east-north-east bimorphism with upper name
\newcommand{\Enebimo}{\@ifnextchar[{\basicEnebimo}{\basicEnebimo[133]}}%

% basic east-north-east bimorphism with lower name
\def\basicenebimO[#1]#2{\ENEBIMO{}{#2}{#100}}%

% east-north-east bimorphism with lower name
\newcommand{\enebimO}{\@ifnextchar[{\basicenebimO}{\basicenebimO[133]}}%

% basic east-north-east isomorphism
\def\basiceneiso[#1]{\ENEAR{\cong}{}{#100}}%

% east-north-east isomorphism
\newcommand{\eneiso}{\@ifnextchar[{\basiceneiso}{\basiceneiso[133]}}%

% basic east-north-east isomorphism with upper name
\def\basicEneiso[#1]#2{\ENEAR{#2}{\cong}{#100}}%

% east-north-east isomorphism with upper name
\newcommand{\Eneiso}{\@ifnextchar[{\basicEneiso}{\basicEneiso[133]}}%

% basic east-north-east isomorphism with lower name
\def\basiceneisO[#1]#2{\ENEAR{\cong}{#2}{#100}}%

% east-north-east isomorphism with lower name
\newcommand{\eneisO}{\@ifnextchar[{\basiceneisO}{\basiceneisO[133]}}%

% basic east-north-east equality
\def\basiceneeql[#1]{\ENEEQL{}{}{#100}}%

% east-north-east equality
\newcommand{\eneeql}{\@ifnextchar[{\basiceneeql}{\basiceneeql[133]}}%

% basic east-north-east equality with upper name
\def\basicEneeql[#1]#2{\ENEEQL{#2}{}{#100}}%

% east-north-east equality with upper name
\newcommand{\Eneeql}{\@ifnextchar[{\basicEneeql}{\basicEneeql[133]}}%

% basic east-north-east equality with lower name
\def\basiceneeqL[#1]#2{\ENEEQL{}{#2}{#100}}%

% east-north-east equality with lower name
\newcommand{\eneeqL}{\@ifnextchar[{\basiceneeqL}{\basiceneeqL[133]}}%

% basic east-north-east pair of arrows
\def\basicenebiar[#1]{\ENEBIAR{}{}{#100}}%

% east-north-east pair of arrows
\newcommand{\enebiar}{\@ifnextchar[{\basicenebiar}{\basicenebiar[133]}}%

% basic east-north-east pair of arrows with names
\def\basicEnebiar[#1]#2#3{\ENEBIAR{#2}{#3}{#100}}%

% east-north-east pair of arrows with names
\newcommand{\Enebiar}{\@ifnextchar[{\basicEnebiar}{\basicEnebiar[133]}}%
\let\enebiaR=\Enebiar

% basic east-north-east pair of distributors
\def\basicenebidist[#1]{\ENEBIDIST{}{}{#100}}%

% east-north-east pair of distributors
\newcommand{\enebidist}{\@ifnextchar[{\basicenebidist}{\basicenebidist[133]}}%

% basic east-north-east pair of distributors with names
\def\basicEnebidist[#1]#2#3{\ENEBIDIST{#2}{#3}{#100}}%

% east-north-east pair of distributors with names
\newcommand{\Enebidist}{\@ifnextchar[{\basicEnebidist}{\basicEnebidist[133]}}%
\let\enebidisT=\Enebidist

% basic east-north-east pair of adjoint arrows
\def\basiceneadjar[#1]{\ENEADJAR{}{}{#100}}%

% east-north-east pair of adjoint arrows
\newcommand{\eneadjar}{\@ifnextchar[{\basiceneadjar}{\basiceneadjar[133]}}%

% basic east-north-east pair of adjoint  arrows with names
\def\basicEneadjar[#1]#2#3{\ENEADJAR{#2}{#3}{#100}}%

% east-north-east pair of adjoint arrows with names
\newcommand{\Eneadjar}{\@ifnextchar[{\basicEneadjar}{\basicEneadjar[133]}}%
\let\eneadjaR=\Eneadjar

% basic east-north-east pair of adjoint distributors
\def\basiceneadjdist[#1]{\ENEADJDIST{}{}{#100}}%

% east-north-east pair of adjoint distributors
\newcommand{\eneadjdist}{\@ifnextchar[{\basiceneadjdist}{\basiceneadjdist[133]}}%

% basic east-north-east pair of adjoint distributors with names
\def\basicEneadjdist[#1]#2#3{\ENEADJDIST{#2}{#3}{#100}}%

% east-north-east pair of adjoint distributors with names
\newcommand{\Eneadjdist}{\@ifnextchar[{\basicEneadjdist}{\basicEneadjdist[133]}}%
\let\eneadjdisT=\Eneadjdist


% EAST-SOUTH-EAST ARROWS

% The following commands produce east-south-east arrows
% of horizontal extent n units

% \ESEAR{f}{g}{n} draws a east-south-east arrow with names f, g
% and length n units
\newcommand{\ESEAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(2,-1){#3}}%
\put(\Y,-\Z){\esehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEDIST{f}{g}{n} draws a east-south-east distributor
% with names f, g and length n units
\newcommand{\ESEDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(2,-1){#3}}%
\put(\Y,-\Z){\esehead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\ESEDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(-\Y,\Z)(\value{y},-\value{z}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(\Y,-\Z){\esehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEMONO{f}{g}{n} draws a east-south-east monomorphism
% with names f,g and length n units
\newcommand{\ESEMONO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\begin{picture}(0,0)%
\put(-\monolength,\secondmonolength){\line(2,-1){\bimolength}}%
\put(-\monolength,\secondmonolength){\esehead}%
\put(\Y,-\Z){\esehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEEPI{f}{g}{n} draws a east-south-east epimorphism
% with names f, g and length n units
\newcommand{\ESEEPI}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(2,-1){\bimolength}}%
\put(\epilength,-\secondepilength){\esehead}%
\put(\Y,-\Z){\esehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEBIMO{f}{g}{n} draws a east-south-east bimorphism
% with names f,g and length n units
\newcommand{\ESEBIMO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\monolength,\secondmonolength){\line(2,-1){\bimolength}}%
\put(-\monolength,\secondmonolength){\esehead}%
\put(\epilength,-\secondepilength){\esehead}%
\put(\Y,-\Z){\esehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEEQL{f}{g}{n} draws a east-south-east equality
% with names f,g and length n units
\newcommand{\ESEEQL}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,\Z){\begin{picture}(0,0)%
\truex{44}\truey{89}%
\put(-\value{x},-\value{y}){\line(2,-1){#3}}%
\put(\value{x},\value{y}){\line(2,-1){#3}}%
\end{picture}}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEBIAR{f}{g}{n} draws a pair of east-south-east arrows
% with names f,g and length n units
\newcommand{\ESEBIAR}[3]{%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\put(-\value{x},-\value{y}){\line(2,-1){#3}}%
\put(\value{x},\value{y}){\line(2,-1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\monolength,-\secondepilength){\esehead}%
\put(\epilength,-\secondmonolength){\esehead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEBIDIST{f}{g}{n} draws a pair of east-south-east distributors
% with names f,g and length n units
\newcommand{\ESEBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(-\Y,\Z){\begin{picture}(0,0)%
\put(-\value{x},-\value{y}){\line(2,-1){#3}}%
\put(\value{x},\value{y}){\line(2,-1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\monolength,-\secondepilength){\esehead}%
\put(\epilength,-\secondmonolength){\esehead}%
\end{picture}}
\put(\value{x},\value{y}){\circle{\value{z}}}%
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEADJAR{f}{g}{n} draws a east-south-east pair of adjoint arrows
% with names f,g and length n units
\newcommand{\ESEADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Y,\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(2,-1){#3}}%
\put(\monolength,-\secondepilength){\esehead}%
\put(\epilength,-\secondmonolength){\line(-2,1){#3}}%
\put(\value{x},\value{y}){\wnwhead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \ESEADJDIST{f}{g}{n} draws a east-south-east pair of adjoint distributors
% with names f,g and length n units
\newcommand{\ESEADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(-\Y,\Z){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(2,-1){#3}}%
\put(\monolength,-\secondepilength){\esehead}%
\put(\epilength,-\secondmonolength){\line(-2,1){#3}}%
\put(\value{x},\value{y}){\wnwhead}%
\end{picture}}
\put(\value{x},\value{y}){\circle{\value{z}}}%
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% The following commands produce east-south-east arrows;
% the default length is 13300 units

% basic east-south-east arrow
\def\basicesear[#1]{\ESEAR{}{}{#100}}%

% east-south-east arrow
\newcommand{\esear}{\@ifnextchar[{\basicesear}{\basicesear[133]}}%

% basic east-south-east arrow with upper name
\def\basicEsear[#1]#2{\ESEAR{#2}{}{#100}}%

% east-south-east arrow with upper name
\newcommand{\Esear}{\@ifnextchar[{\basicEsear}{\basicEsear[133]}}%

% basic east-south-east arrow with lower name
\def\basiceseaR[#1]#2{\ESEAR{}{#2}{#100}}%

% east-south-east arrow with lower name
\newcommand{\eseaR}{\@ifnextchar[{\basiceseaR}{\basiceseaR[133]}}%

% basic east-south-east distributor
\def\basicesedist[#1]{\ESEDIST{}{}{#100}}%

% east-south-east distributor
\newcommand{\esedist}{\@ifnextchar[{\basicesedist}{\basicesedist[133]}}%

% basic east-south-east distributor with upper name
\def\basicEsedist[#1]#2{\ESEDIST{#2}{}{#100}}%

% east-south-east distributor with upper name
\newcommand{\Esedist}{\@ifnextchar[{\basicEsedist}{\basicEsedist[133]}}%

% basic east-south-east distributor with lower name
\def\basicesedisT[#1]#2{\ESEDIST{}{#2}{#100}}%

% east-south-east distributor with lower name
\newcommand{\esedisT}{\@ifnextchar[{\basicesedisT}{\basicesedisT[133]}}%

% basic east-south-east dotted arrow
\def\basicesedotar[#1]{\ESEDOTAR{}{}{#100}}%

% east-south-east dotted arrow
\newcommand{\esedotar}{\@ifnextchar[{\basicesedotar}{\basicesedotar[133]}}%

% basic east-south-east dotted arrow with upper name
\def\basicEsedotar[#1]#2{\ESEDOTAR{#2}{}{#100}}%

% east-south-east dotted arrow with upper name
\newcommand{\Esedotar}{\@ifnextchar[{\basicEsedotar}{\basicEsedotar[133]}}%

% basic east-south-east dotted arrow with lower name
\def\basicesedotaR[#1]#2{\ESEDOTAR{}{#2}{#100}}%

% east-south-east dotted arrow with lower name
\newcommand{\esedotaR}{\@ifnextchar[{\basicesedotaR}{\basicesedotaR[133]}}%

% basic east-south-east monomorphism
\def\basicesemono[#1]{\ESEMONO{}{}{#100}}%

% east-south-east monomorphism
\newcommand{\esemono}{\@ifnextchar[{\basicesemono}{\basicesemono[133]}}%

% basic east-south-east monomorphism with upper name
\def\basicEsemono[#1]#2{\ESEMONO{#2}{}{#100}}%

% east-south-east monomorphism with upper name
\newcommand{\Esemono}{\@ifnextchar[{\basicEsemono}{\basicEsemono[133]}}%

% basic east-south-east monomorphism with lower name
\def\basicesemonO[#1]#2{\ESEMONO{}{#2}{#100}}%

% east-south-east monomorphism with lower name
\newcommand{\esemonO}{\@ifnextchar[{\basicesemonO}{\basicesemonO[133]}}%

% basic east-south-east epimorphism
\def\basiceseepi[#1]{\ESEEPI{}{}{#100}}%

% east-south-east epimorphism
\newcommand{\eseepi}{\@ifnextchar[{\basiceseepi}{\basiceseepi[133]}}%

% basic east-south-east epimorphism with upper name
\def\basicEseepi[#1]#2{\ESEEPI{#2}{}{#100}}%

% east-south-east epimorphism with upper name
\newcommand{\Eseepi}{\@ifnextchar[{\basicEseepi}{\basicEseepi[133]}}%

% basic east-south-east epimorphism with lower name
\def\basiceseepI[#1]#2{\ESEEPI{}{#2}{#100}}%

% east-south-east epimorphism with lower name
\newcommand{\eseepI}{\@ifnextchar[{\basiceseepI}{\basiceseepI[133]}}%

% basic east-south-east bimorphism
\def\basicesebimo[#1]{\ESEBIMO{}{}{#100}}%

% east-south-east bimorphism
\newcommand{\esebimo}{\@ifnextchar[{\basicesebimo}{\basicesebimo[133]}}%

% basic east-south-east bimorphism with upper name
\def\basicEsebimo[#1]#2{\ESEBIMO{#2}{}{#100}}%

% east-south-east bimorphism with upper name
\newcommand{\Esebimo}{\@ifnextchar[{\basicEsebimo}{\basicEsebimo[133]}}%

% basic east-south-east bimorphism with lower name
\def\basicesebimO[#1]#2{\ESEBIMO{}{#2}{#100}}%

% east-south-east bimorphism with lower name
\newcommand{\esebimO}{\@ifnextchar[{\basicesebimO}{\basicesebimO[133]}}%

% basic east-south-east isomorphism
\def\basiceseiso[#1]{\ESEAR{\cong}{}{#100}}%

% east-south-east isomorphism
\newcommand{\eseiso}{\@ifnextchar[{\basiceseiso}{\basiceseiso[133]}}%

% basic east-south-east isomorphism with upper name
\def\basicEseiso[#1]#2{\ESEAR{#2}{\cong}{#100}}%

% east-south-east isomorphism with upper name
\newcommand{\Eseiso}{\@ifnextchar[{\basicEseiso}{\basicEseiso[133]}}%

% basic east-south-east isomorphism with lower name
\def\basiceseisO[#1]#2{\ESEAR{\cong}{#2}{#100}}%

% east-south-east isomorphism with lower name
\newcommand{\eseisO}{\@ifnextchar[{\basiceseisO}{\basiceseisO[133]}}%

% basic east-south-east equality
\def\basiceseeql[#1]{\ESEEQL{}{}{#100}}%

% east-south-east equality
\newcommand{\eseeql}{\@ifnextchar[{\basiceseeql}{\basiceseeql[133]}}%

% basic east-south-east equality with upper name
\def\basicEseeql[#1]#2{\ESEEQL{#2}{}{#100}}%

% east-south-east equality with upper name
\newcommand{\Eseeql}{\@ifnextchar[{\basicEseeql}{\basicEseeql[133]}}%

% basic east-south-east equality with lower name
\def\basiceseeqL[#1]#2{\ESEEQL{}{#2}{#100}}%

% east-south-east equality with lower name
\newcommand{\eseeqL}{\@ifnextchar[{\basiceseeqL}{\basiceseeqL[133]}}%

% basic east-south-east pair of arrows
\def\basicesebiar[#1]{\ESEBIAR{}{}{#100}}%

% east-south-east pair of arrows
\newcommand{\esebiar}{\@ifnextchar[{\basicesebiar}{\basicesebiar[133]}}%

% basic east-south-east pair of arrows with names
\def\basicEsebiar[#1]#2#3{\ESEBIAR{#2}{#3}{#100}}%

% east-south-east pair of arrows with names
\newcommand{\Esebiar}{\@ifnextchar[{\basicEsebiar}{\basicEsebiar[133]}}%
\let\esebiaR=\Esebiar

% basic east-south-east pair of distributors
\def\basicesebidist[#1]{\ESEBIDIST{}{}{#100}}%

% east-south-east pair of distributors
\newcommand{\esebidist}{\@ifnextchar[{\basicesebidist}{\basicesebidist[133]}}%

% basic east-south-east pair of distributors with names
\def\basicEsebidist[#1]#2#3{\ESEBIDIST{#2}{#3}{#100}}%

% east-south-east pair of distributors with names
\newcommand{\Esebidist}{\@ifnextchar[{\basicEsebidist}{\basicEsebidist[133]}}%
\let\esebidisT=\Esebidist

% basic east-south-east pair of adjoint arrows
\def\basiceseadjar[#1]{\ESEADJAR{}{}{#100}}%

% east-south-east pair of adjoint arrows
\newcommand{\eseadjar}{\@ifnextchar[{\basiceseadjar}{\basiceseadjar[133]}}%

% basic east-south-east pair of adjoint  arrows with names
\def\basicEseadjar[#1]#2#3{\ESEADJAR{#2}{#3}{#100}}%

% east-south-east pair of adjoint arrows with names
\newcommand{\Eseadjar}{\@ifnextchar[{\basicEseadjar}{\basicEseadjar[133]}}%
\let\eseadjaR=\Eseadjar

% basic east-south-east pair of adjoint distributors
\def\basiceseadjdist[#1]{\ESEADJDIST{}{}{#100}}%

% east-south-east pair of adjoint distributors
\newcommand{\eseadjdist}{\@ifnextchar[{\basiceseadjdist}{\basiceseadjdist[133]}}%

% basic east-south-east pair of adjoint distributors with names
\def\basicEseadjdist[#1]#2#3{\ESEADJDIST{#2}{#3}{#100}}%

% east-south-east pair of adjoint distributors with names
\newcommand{\Eseadjdist}{\@ifnextchar[{\basicEseadjdist}{\basicEseadjdist[133]}}%
\let\eseadjdisT=\Eseadjdist

% WEST-SOUTH-WEST ARROWS

% The following commands produce west-south-west arrows
% of horizontal extent n units

% \WSWAR{f}{g}{n} draws a west-south-west arrow with names f, g
% and length n units
\newcommand{\WSWAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-2,-1){#3}}%
\put(-\Y,-\Z){\wswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWDIST{f}{g}{n} draws a west-south-west distributor
% with names f, g and length n units
\newcommand{\WSWDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-2,-1){#3}}%
\put(-\Y,-\Z){\wswhead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\WSWDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(\Y,\Z)(-\value{y},-\value{z}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(-\Y,-\Z){\wswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWMONO{f}{g}{n} draws a west-south-west monomorphism
% with names f,g and length n units
\newcommand{\WSWMONO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\begin{picture}(0,0)%
\put(\monolength,\secondmonolength){\line(-2,-1){\bimolength}}%
\put(\monolength,\secondmonolength){\wswhead}%
\put(-\Y,-\Z){\wswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWEPI{f}{g}{n} draws a west-south-west epimorphism
% with names f, g and length n units
\newcommand{\WSWEPI}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-2,-1){\bimolength}}%
\put(-\epilength,-\secondepilength){\wswhead}%
\put(-\Y,-\Z){\wswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWBIMO{f}{g}{n} draws a west-south-west bimorphism
% with names f,g and length n units
\newcommand{\WSWBIMO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(\monolength,\secondmonolength){\line(-2,-1){\bimolength}}%
\put(\monolength,\secondmonolength){\wswhead}%
\put(-\epilength,-\secondepilength){\wswhead}%
\put(-\Y,-\Z){\wswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWBIAR{f}{g}{n} draws a pair of west-south-west arrows
% with names f,g and length n units
\newcommand{\WSWBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\put(-\value{x},\value{y}){\line(-2,-1){#3}}%
\put(\value{x},-\value{y}){\line(-2,-1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\monolength,-\secondepilength){\wswhead}%
\put(-\epilength,-\secondmonolength){\wswhead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWBIDIST{f}{g}{n} draws a pair of west-south-west distributors
% with names f,g and length n units
\newcommand{\WSWBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(\Y,\Z){\begin{picture}(0,0)%
\put(-\value{x},\value{y}){\line(-2,-1){#3}}%
\put(\value{x},-\value{y}){\line(-2,-1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\monolength,-\secondepilength){\wswhead}%
\put(-\epilength,-\secondmonolength){\wswhead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWADJAR{f}{g}{n} draws a west-south-west pair of adjoint arrows
% with names f,g and length n units
\newcommand{\WSWADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(-2,-1){#3}}%
\put(-\monolength,-\secondepilength){\wswhead}%
\put(-\epilength,-\secondmonolength){\line(2,1){#3}}%
\put(-\value{x},\value{y}){\enehead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \WSWADJDIST{f}{g}{n} draws a west-south-west pair of adjoint distributors
% with names f,g and length n units
\newcommand{\WSWADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(\Y,\Z){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(-2,-1){#3}}%
\put(-\monolength,-\secondepilength){\wswhead}%
\put(-\epilength,-\secondmonolength){\line(2,1){#3}}%
\put(-\value{x},\value{y}){\enehead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% The following commands produce west-south-west arrows;
% the default length is 13300 units

% basic west-south-west arrow
\def\basicwswar[#1]{\WSWAR{}{}{#100}}%

% west-south-west arrow
\newcommand{\wswar}{\@ifnextchar[{\basicwswar}{\basicwswar[133]}}%

% basic west-south-west arrow with upper name
\def\basicWswar[#1]#2{\WSWAR{#2}{}{#100}}%

% west-south-west arrow with upper name
\newcommand{\Wswar}{\@ifnextchar[{\basicWswar}{\basicWswar[133]}}%

% basic west-south-west arrow with lower name
\def\basicwswaR[#1]#2{\WSWAR{}{#2}{#100}}%

% west-south-west arrow with lower name
\newcommand{\wswaR}{\@ifnextchar[{\basicwswaR}{\basicwswaR[133]}}%

% basic west-south-west distributor
\def\basicwswdist[#1]{\WSWDIST{}{}{#100}}%

% west-south-west distributor
\newcommand{\wswdist}{\@ifnextchar[{\basicwswdist}{\basicwswdist[133]}}%

% basic west-south-west distributor with upper name
\def\basicWswdist[#1]#2{\WSWDIST{#2}{}{#100}}%

% west-south-west distributor with upper name
\newcommand{\Wswdist}{\@ifnextchar[{\basicWswdist}{\basicWswdist[133]}}%

% basic west-south-west distributor with lower name
\def\basicwswdisT[#1]#2{\WSWDIST{}{#2}{#100}}%

% west-south-west distributor with lower name
\newcommand{\wswdisT}{\@ifnextchar[{\basicwswdisT}{\basicwswdisT[133]}}%

% basic west-south-west dotted arrow
\def\basicwswdotar[#1]{\WSWDOTAR{}{}{#100}}%

% west-south-west dotted arrow
\newcommand{\wswdotar}{\@ifnextchar[{\basicwswdotar}{\basicwswdotar[133]}}%

% basic west-south-west dotted arrow with upper name
\def\basicWswdotar[#1]#2{\WSWDOTAR{#2}{}{#100}}%

% west-south-west dotted arrow with upper name
\newcommand{\Wswdotar}{\@ifnextchar[{\basicWswdotar}{\basicWswdotar[133]}}%

% basic west-south-west dotted arrow with lower name
\def\basicwswdotaR[#1]#2{\WSWDOTAR{}{#2}{#100}}%

% west-south-west dotted arrow with lower name
\newcommand{\wswdotaR}{\@ifnextchar[{\basicwswdotaR}{\basicwswdotaR[133]}}%

% basic west-south-west monomorphism
\def\basicwswmono[#1]{\WSWMONO{}{}{#100}}%

% west-south-west monomorphism
\newcommand{\wswmono}{\@ifnextchar[{\basicwswmono}{\basicwswmono[133]}}%

% basic west-south-west monomorphism with upper name
\def\basicWswmono[#1]#2{\WSWMONO{#2}{}{#100}}%

% west-south-west monomorphism with upper name
\newcommand{\Wswmono}{\@ifnextchar[{\basicWswmono}{\basicWswmono[133]}}%

% basic west-south-west monomorphism with lower name
\def\basicwswmonO[#1]#2{\WSWMONO{}{#2}{#100}}%

% west-south-west monomorphism with lower name
\newcommand{\wswmonO}{\@ifnextchar[{\basicwswmonO}{\basicwswmonO[133]}}%

% basic west-south-west epimorphism
\def\basicwswepi[#1]{\WSWEPI{}{}{#100}}%

% west-south-west epimorphism
\newcommand{\wswepi}{\@ifnextchar[{\basicwswepi}{\basicwswepi[133]}}%

% basic west-south-west epimorphism with upper name
\def\basicWswepi[#1]#2{\WSWEPI{#2}{}{#100}}%

% west-south-west epimorphism with upper name
\newcommand{\Wswepi}{\@ifnextchar[{\basicWswepi}{\basicWswepi[133]}}%

% basic west-south-west epimorphism with lower name
\def\basicwswepI[#1]#2{\WSWEPI{}{#2}{#100}}%

% west-south-west epimorphism with lower name
\newcommand{\wswepI}{\@ifnextchar[{\basicwswepI}{\basicwswepI[133]}}%

% basic west-south-west bimorphism
\def\basicwswbimo[#1]{\WSWBIMO{}{}{#100}}%

% west-south-west bimorphism
\newcommand{\wswbimo}{\@ifnextchar[{\basicwswbimo}{\basicwswbimo[133]}}%

% basic west-south-west bimorphism with upper name
\def\basicWswbimo[#1]#2{\WSWBIMO{#2}{}{#100}}%

% west-south-west bimorphism with upper name
\newcommand{\Wswbimo}{\@ifnextchar[{\basicWswbimo}{\basicWswbimo[133]}}%

% basic west-south-west bimorphism with lower name
\def\basicwswbimO[#1]#2{\WSWBIMO{}{#2}{#100}}%

% west-south-west bimorphism with lower name
\newcommand{\wswbimO}{\@ifnextchar[{\basicwswbimO}{\basicwswbimO[133]}}%

% basic west-south-west isomorphism
\def\basicwswiso[#1]{\WSWAR{\cong}{}{#100}}%

% west-south-west isomorphism
\newcommand{\wswiso}{\@ifnextchar[{\basicwswiso}{\basicwswiso[133]}}%

% basic west-south-west isomorphism with upper name
\def\basicWswiso[#1]#2{\WSWAR{#2}{\cong}{#100}}%

% west-south-west isomorphism with upper name
\newcommand{\Wswiso}{\@ifnextchar[{\basicWswiso}{\basicWswiso[133]}}%

% basic west-south-west isomorphism with lower name
\def\basicwswisO[#1]#2{\WSWAR{\cong}{#2}{#100}}%

% west-south-west isomorphism with lower name
\newcommand{\wswisO}{\@ifnextchar[{\basicwswisO}{\basicwswisO[133]}}%

% west-south-west equality
\let\wsweql=\eneeql%

% west-south-west equality with upper name
\let\Wsweql=\Eneeql%

% west-south-west equality with lower name
\let\wsweqL=\eneeqL%

% basic west-south-west pair of arrows
\def\basicwswbiar[#1]{\WSWBIAR{}{}{#100}}%

% west-south-west pair of arrows
\newcommand{\wswbiar}{\@ifnextchar[{\basicwswbiar}{\basicwswbiar[133]}}%

% basic west-south-west pair of arrows with names
\def\basicWswbiar[#1]#2#3{\WSWBIAR{#2}{#3}{#100}}%

% west-south-west pair of arrows with names
\newcommand{\Wswbiar}{\@ifnextchar[{\basicWswbiar}{\basicWswbiar[133]}}%
\let\wswbiaR=\Wswbiar

% basic west-south-west pair of distributors
\def\basicwswbidist[#1]{\WSWBIDIST{}{}{#100}}%

% west-south-west pair of distributors
\newcommand{\wswbidist}{\@ifnextchar[{\basicwswbidist}{\basicwswbidist[133]}}%

% basic west-south-west pair of distributors with names
\def\basicWswbidist[#1]#2#3{\WSWBIDIST{#2}{#3}{#100}}%

% west-south-west pair of distributors with names
\newcommand{\Wswbidist}{\@ifnextchar[{\basicWswbidist}{\basicWswbidist[133]}}%
\let\wswbidisT=\Wswbidist

% basic west-south-west pair of adjoint arrows
\def\basicwswadjar[#1]{\WSWADJAR{}{}{#100}}%

% west-south-west pair of adjoint arrows
\newcommand{\wswadjar}{\@ifnextchar[{\basicwswadjar}{\basicwswadjar[133]}}%

% basic west-south-west pair of adjoint  arrows with names
\def\basicWswadjar[#1]#2#3{\WSWADJAR{#2}{#3}{#100}}%

% west-south-west pair of adjoint arrows with names
\newcommand{\Wswadjar}{\@ifnextchar[{\basicWswadjar}{\basicWswadjar[133]}}%
\let\wswadjaR=\Wswadjar

% basic west-south-west pair of adjoint distributors
\def\basicwswadjdist[#1]{\WSWADJDIST{}{}{#100}}%

% west-south-west pair of adjoint distributors
\newcommand{\wswadjdist}{\@ifnextchar[{\basicwswadjdist}{\basicwswadjdist[133]}}%

% basic west-south-west pair of adjoint distributors with names
\def\basicWswadjdist[#1]#2#3{\WSWADJDIST{#2}{#3}{#100}}%

% west-south-west pair of adjoint distributors with names
\newcommand{\Wswadjdist}{\@ifnextchar[{\basicWswadjdist}{\basicWswadjdist[133]}}%
\let\wswadjdisT=\Wswadjdist


% WEST-NORTH-WEST ARROWS

% The following commands produce west-north-west arrows
% of horizontal extent n units

% \WNWAR{f}{g}{n} draws a west-north-west arrow with names f, g
% and length n units
\newcommand{\WNWAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-2,1){#3}}%
\put(-\Y,\Z){\wnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWDIST{f}{g}{n} draws a west-north-west distributor
% with names f, g and length n units
\newcommand{\WNWDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-2,1){#3}}%
\put(-\Y,\Z){\wnwhead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\WNWDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{y}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(\Y,-\Z)(-\value{y},\value{z}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(-\Y,\Z){\wnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWMONO{f}{g}{n} draws a west-north-west monomorphism
% with names f,g and length n units
\newcommand{\WNWMONO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\begin{picture}(0,0)%
\put(\monolength,-\secondmonolength){\line(-2,1){\bimolength}}%
\put(\monolength,-\secondmonolength){\wnwhead}%
\put(-\Y,\Z){\wnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWEPI{f}{g}{n} draws a west-north-west epimorphism
% with names f, g and length n units
\newcommand{\WNWEPI}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\Y%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-2,1){\bimolength}}%
\put(-\epilength,\secondepilength){\wnwhead}%
\put(-\Y,\Z){\wnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWBIMO{f}{g}{n} draws a west-north-west bimorphism
% with names f,g and length n units
\newcommand{\WNWBIMO}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\TrueTail\TrueHead%
\bimolength=#3%
\advance\bimolength by -\TrueMonoTail%
\monolength=\bimolength%
\advance\monolength by -\Y%
\advance\bimolength by -\TrueEpiHead%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\divide\secondmonolength by 2%
\secondepilength=\epilength%
\divide\secondepilength by 2%
\begin{picture}(0,0)%
\put(\monolength,-\secondmonolength){\line(-2,1){\bimolength}}%
\put(\monolength,-\secondmonolength){\wnwhead}%
\put(-\epilength,\secondepilength){\wnwhead}%
\put(-\Y,\Z){\wnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWBIAR{f}{g}{n} draws a pair of west-north-west arrows
% with names f,g and length n units
\newcommand{\WNWBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,-\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\put(-\value{x},-\value{y}){\line(-2,1){#3}}%
\put(\value{x},\value{y}){\line(-2,1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\monolength,\secondepilength){\wnwhead}%
\put(-\epilength,\secondmonolength){\wnwhead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWBIDIST{f}{g}{n} draws a pair of west-north-west distributors
% with names f,g and length n units
\newcommand{\WNWBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(\Y,-\Z){\begin{picture}(0,0)%
\put(-\value{x},-\value{y}){\line(-2,1){#3}}%
\put(\value{x},\value{y}){\line(-2,1){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\monolength,\secondepilength){\wnwhead}%
\put(-\epilength,\secondmonolength){\wnwhead}%
\end{picture}}
\put(\value{x},\value{y}){\circle{\value{z}}}%
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWADJAR{f}{g}{n} draws a west-north-west pair of adjoint arrows
% with names f,g and length n units
\newcommand{\WNWADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Y,-\Z){\begin{picture}(0,0)%
\truex{156}\truey{313}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(-2,1){#3}}%
\put(-\epilength,\secondmonolength){\wnwhead}%
\put(-\monolength,\secondepilength){\line(2,-1){#3}}%
\put(\value{x},\value{y}){\esehead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \WNWADJDIST{f}{g}{n} draws a west-north-west pair of adjoint distributors
% with names f,g and length n units
\newcommand{\WNWADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=\Y%
\divide\Z by 2%
\begin{picture}(0,0)%
\truex{156}\truey{313}\truez{400}%
\put(\Y,-\Z){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Y%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Y%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(-2,1){#3}}%
\put(-\epilength,\secondmonolength){\wnwhead}%
\put(-\monolength,\secondepilength){\line(2,-1){#3}}%
\put(\value{x},\value{y}){\esehead}%
\end{picture}}
\put(\value{x},\value{y}){\circle{\value{z}}}%
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% The following commands produce west-north-west arrows;
% the default length is 13300 units

% basic west-north-west arrow
\def\basicwnwar[#1]{\WNWAR{}{}{#100}}%

% west-north-west arrow
\newcommand{\wnwar}{\@ifnextchar[{\basicwnwar}{\basicwnwar[133]}}%

% basic west-north-west arrow with upper name
\def\basicWnwar[#1]#2{\WNWAR{#2}{}{#100}}%

% west-north-west arrow with upper name
\newcommand{\Wnwar}{\@ifnextchar[{\basicWnwar}{\basicWnwar[133]}}%

% basic west-north-west arrow with lower name
\def\basicwnwaR[#1]#2{\WNWAR{}{#2}{#100}}%

% west-north-west arrow with lower name
\newcommand{\wnwaR}{\@ifnextchar[{\basicwnwaR}{\basicwnwaR[133]}}%

% basic west-north-west distributor
\def\basicwnwdist[#1]{\WNWDIST{}{}{#100}}%

% west-north-west distributor
\newcommand{\wnwdist}{\@ifnextchar[{\basicwnwdist}{\basicwnwdist[133]}}%

% basic west-north-west distributor with upper name
\def\basicWnwdist[#1]#2{\WNWDIST{#2}{}{#100}}%

% west-north-west distributor with upper name
\newcommand{\Wnwdist}{\@ifnextchar[{\basicWnwdist}{\basicWnwdist[133]}}%

% basic west-north-west distributor with lower name
\def\basicwnwdisT[#1]#2{\WNWDIST{}{#2}{#100}}%

% west-north-west distributor with lower name
\newcommand{\wnwdisT}{\@ifnextchar[{\basicwnwdisT}{\basicwnwdisT[133]}}%

% basic west-north-west dotted arrow
\def\basicwnwdotar[#1]{\WNWDOTAR{}{}{#100}}%

% west-north-west dotted arrow
\newcommand{\wnwdotar}{\@ifnextchar[{\basicwnwdotar}{\basicwnwdotar[133]}}%

% basic west-north-west dotted arrow with upper name
\def\basicWnwdotar[#1]#2{\WNWDOTAR{#2}{}{#100}}%

% west-north-west dotted arrow with upper name
\newcommand{\Wnwdotar}{\@ifnextchar[{\basicWnwdotar}{\basicWnwdotar[133]}}%

% basic west-north-west dotted arrow with lower name
\def\basicwnwdotaR[#1]#2{\WNWDOTAR{}{#2}{#100}}%

% west-north-west dotted arrow with lower name
\newcommand{\wnwdotaR}{\@ifnextchar[{\basicwnwdotaR}{\basicwnwdotaR[133]}}%

% basic west-north-west monomorphism
\def\basicwnwmono[#1]{\WNWMONO{}{}{#100}}%

% west-north-west monomorphism
\newcommand{\wnwmono}{\@ifnextchar[{\basicwnwmono}{\basicwnwmono[133]}}%

% basic west-north-west monomorphism with upper name
\def\basicWnwmono[#1]#2{\WNWMONO{#2}{}{#100}}%

% west-north-west monomorphism with upper name
\newcommand{\Wnwmono}{\@ifnextchar[{\basicWnwmono}{\basicWnwmono[133]}}%

% basic west-north-west monomorphism with lower name
\def\basicwnwmonO[#1]#2{\WNWMONO{}{#2}{#100}}%

% west-north-west monomorphism with lower name
\newcommand{\wnwmonO}{\@ifnextchar[{\basicwnwmonO}{\basicwnwmonO[133]}}%

% basic west-north-west epimorphism
\def\basicwnwepi[#1]{\WNWEPI{}{}{#100}}%

% west-north-west epimorphism
\newcommand{\wnwepi}{\@ifnextchar[{\basicwnwepi}{\basicwnwepi[133]}}%

% basic west-north-west epimorphism with upper name
\def\basicWnwepi[#1]#2{\WNWEPI{#2}{}{#100}}%

% west-north-west epimorphism with upper name
\newcommand{\Wnwepi}{\@ifnextchar[{\basicWnwepi}{\basicWnwepi[133]}}%

% basic west-north-west epimorphism with lower name
\def\basicwnwepI[#1]#2{\WNWEPI{}{#2}{#100}}%

% west-north-west epimorphism with lower name
\newcommand{\wnwepI}{\@ifnextchar[{\basicwnwepI}{\basicwnwepI[133]}}%

% basic west-north-west bimorphism
\def\basicwnwbimo[#1]{\WNWBIMO{}{}{#100}}%

% west-north-west bimorphism
\newcommand{\wnwbimo}{\@ifnextchar[{\basicwnwbimo}{\basicwnwbimo[133]}}%

% basic west-north-west bimorphism with upper name
\def\basicWnwbimo[#1]#2{\WNWBIMO{#2}{}{#100}}%

% west-north-west bimorphism with upper name
\newcommand{\Wnwbimo}{\@ifnextchar[{\basicWnwbimo}{\basicWnwbimo[133]}}%

% basic west-north-west bimorphism with lower name
\def\basicwnwbimO[#1]#2{\WNWBIMO{}{#2}{#100}}%

% west-north-west bimorphism with lower name
\newcommand{\wnwbimO}{\@ifnextchar[{\basicwnwbimO}{\basicwnwbimO[133]}}%

% basic west-north-west isomorphism
\def\basicwnwiso[#1]{\WNWAR{\cong}{}{#100}}%

% west-north-west isomorphism
\newcommand{\wnwiso}{\@ifnextchar[{\basicwnwiso}{\basicwnwiso[133]}}%

% basic west-north-west isomorphism with upper name
\def\basicWnwiso[#1]#2{\WNWAR{#2}{\cong}{#100}}%

% west-north-west isomorphism with upper name
\newcommand{\Wnwiso}{\@ifnextchar[{\basicWnwiso}{\basicWnwiso[133]}}%

% basic west-north-west isomorphism with lower name
\def\basicwnwisO[#1]#2{\WNWAR{\cong}{#2}{#100}}%

% west-north-west isomorphism with lower name
\newcommand{\wnwisO}{\@ifnextchar[{\basicwnwisO}{\basicwnwisO[133]}}%

% west-north-west equality
\let\wnweql=\eseeql%

% west-north-west equality with upper name
\let\Wnweql=\Eseeql%

% west-north-west equality with lower name
\let\wnweqL=\eseeqL%

% basic west-north-west pair of arrows
\def\basicwnwbiar[#1]{\WNWBIAR{}{}{#100}}%

% west-north-west pair of arrows
\newcommand{\wnwbiar}{\@ifnextchar[{\basicwnwbiar}{\basicwnwbiar[133]}}%

% basic west-north-west pair of arrows with names
\def\basicWnwbiar[#1]#2#3{\WNWBIAR{#2}{#3}{#100}}%

% west-north-west pair of arrows with names
\newcommand{\Wnwbiar}{\@ifnextchar[{\basicWnwbiar}{\basicWnwbiar[133]}}%
\let\wnwbiaR=\Wnwbiar

% basic west-north-west pair of distributors
\def\basicwnwbidist[#1]{\WNWBIDIST{}{}{#100}}%

% west-north-west pair of distributors
\newcommand{\wnwbidist}{\@ifnextchar[{\basicwnwbidist}{\basicwnwbidist[133]}}%

% basic west-north-west pair of distributors with names
\def\basicWnwbidist[#1]#2#3{\WNWBIDIST{#2}{#3}{#100}}%

% west-north-west pair of distributors with names
\newcommand{\Wnwbidist}{\@ifnextchar[{\basicWnwbidist}{\basicWnwbidist[133]}}%
\let\wnwbidisT=\Wnwbidist

% basic west-north-west pair of adjoint arrows
\def\basicwnwadjar[#1]{\WNWADJAR{}{}{#100}}%

% west-north-west pair of adjoint arrows
\newcommand{\wnwadjar}{\@ifnextchar[{\basicwnwadjar}{\basicwnwadjar[133]}}%

% basic west-north-west pair of adjoint  arrows with names
\def\basicWnwadjar[#1]#2#3{\WNWADJAR{#2}{#3}{#100}}%

% west-north-west pair of adjoint arrows with names
\newcommand{\Wnwadjar}{\@ifnextchar[{\basicWnwadjar}{\basicWnwadjar[133]}}%
\let\wnwadjaR=\Wnwadjar

% basic west-north-west pair of adjoint distributors
\def\basicwnwadjdist[#1]{\WNWADJDIST{}{}{#100}}%

% west-north-west pair of adjoint distributors
\newcommand{\wnwadjdist}{\@ifnextchar[{\basicwnwadjdist}{\basicwnwadjdist[133]}}%

% basic west-north-west pair of adjoint distributors with names
\def\basicWnwadjdist[#1]#2#3{\WNWADJDIST{#2}{#3}{#100}}%

% west-north-west pair of adjoint distributors with names
\newcommand{\Wnwadjdist}{\@ifnextchar[{\basicWnwadjdist}{\basicWnwadjdist[133]}}%
\let\wnwadjdisT=\Wnwadjdist


% NORTH-NORTH-EAST ARROWS

% The following commands produce north-north-east arrows
% of horizontal extent n units

% \NNEAR{f}{g}{n} draws a north-north-east arrow with names f, g
% and length n units
\newcommand{\NNEAR}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Z,-#3){\line(1,2){#3}}%
\put(\Z,#3){\nnehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEDIST{f}{g}{n} draws a north-north-east distributor
% with names f, g and length n units
\newcommand{\NNEDIST}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Z,-#3){\line(1,2){#3}}%
\put(\Z,#3){\nnehead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\NNEDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Z=#3%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{z}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(-\Z,-#3)(\value{z},\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(\Z,#3){\nnehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEMONO{f}{g}{n} draws a north-north-east monomorphism
% with names f,g and length n units
\newcommand{\NNEMONO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\begin{picture}(0,0)%
\put(-\monolength,-\secondmonolength){\line(1,2){\bimolength}}%
\put(-\monolength,-\secondmonolength){\nnehead}%
\put(\Z,#3){\nnehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEEPI{f}{g}{n} draws a north-north-east epimorphism
% with names f, g and length n units
\newcommand{\NNEEPI}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\trueheaD%
\bimolength=#3%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\Z%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\Z,-#3){\line(1,2){\bimolength}}%
\put(\epilength,\secondepilength){\nnehead}%
\put(\Z,#3){\nnehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEBIMO{f}{g}{n} draws a north-north-east bimorphism
% with names f,g and length n units
\newcommand{\NNEBIMO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL\trueheaD%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\monolength,-\secondmonolength){\line(1,2){\bimolength}}%
\put(-\monolength,-\secondmonolength){\nnehead}%
\put(\epilength,\secondepilength){\nnehead}%
\put(\Z,#3){\nnehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEEQL{f}{g}{n} draws a north-north-east equality
% with names f,g and length n units
\newcommand{\NNEEQL}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Z,-#3){\begin{picture}(0,0)%
\truex{44}\truey{89}%
\put(-\value{y},\value{x}){\line(1,2){#3}}%
\put(\value{y},-\value{x}){\line(1,2){#3}}%
\end{picture}}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEBIAR{f}{g}{n} draws a pair of north-north-east arrows
% with names f,g and length n units
\newcommand{\NNEBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\put(-\value{x},\value{y}){\line(1,2){#3}}%
\put(\value{x},-\value{y}){\line(1,2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\monolength,\secondepilength){\nnehead}%
\put(\epilength,\secondmonolength){\nnehead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEBIDIST{f}{g}{n} draws a pair of north-north-east distributors
% with names f,g and length n units
\newcommand{\NNEBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(-\Y,-#3){\begin{picture}(0,0)%
\put(-\value{x},\value{y}){\line(1,2){#3}}%
\put(\value{x},-\value{y}){\line(1,2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\monolength,\secondepilength){\nnehead}%
\put(\epilength,\secondmonolength){\nnehead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEADJAR{f}{g}{n} draws a north-north-east pair of adjoint arrows
% with names f,g and length n units
\newcommand{\NNEADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(-\Y,-#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(1,2){#3}}%
\put(\epilength,\secondmonolength){\nnehead}%
\put(\monolength,\secondepilength){\line(-1,-2){#3}}%
\put(-\value{x},\value{y}){\sswhead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \NNEADJDIST{f}{g}{n} draws a north-north-east pair of adjoint distributors
% with names f,g and length n units
\newcommand{\NNEADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(-\Y,-#3){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(1,2){#3}}%
\put(\epilength,\secondmonolength){\nnehead}%
\put(\monolength,\secondepilength){\line(-1,-2){#3}}%
\put(-\value{x},\value{y}){\sswhead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% The following commands produce north-north-east arrows;
% the default length is 6700 units

% basic north-north-east arrow
\def\basicnnear[#1]{\NNEAR{}{}{#100}}%

% north-north-east arrow
\newcommand{\nnear}{\@ifnextchar[{\basicnnear}{\basicnnear[67]}}%

% basic north-north-east arrow with upper name
\def\basicNnear[#1]#2{\NNEAR{#2}{}{#100}}%

% north-north-east arrow with upper name
\newcommand{\Nnear}{\@ifnextchar[{\basicNnear}{\basicNnear[67]}}%

% basic north-north-east arrow with lower name
\def\basicnneaR[#1]#2{\NNEAR{}{#2}{#100}}%

% north-north-east arrow with lower name
\newcommand{\nneaR}{\@ifnextchar[{\basicnneaR}{\basicnneaR[67]}}%

% basic north-north-east distributor
\def\basicnnedist[#1]{\NNEDIST{}{}{#100}}%

% north-north-east distributor
\newcommand{\nnedist}{\@ifnextchar[{\basicnnedist}{\basicnnedist[67]}}%

% basic north-north-east distributor with upper name
\def\basicNnedist[#1]#2{\NNEDIST{#2}{}{#100}}%

% north-north-east distributor with upper name
\newcommand{\Nnedist}{\@ifnextchar[{\basicNnedist}{\basicNnedist[67]}}%

% basic north-north-east distributor with lower name
\def\basicnnedisT[#1]#2{\NNEDIST{}{#2}{#100}}%

% north-north-east distributor with lower name
\newcommand{\nnedisT}{\@ifnextchar[{\basicnnedisT}{\basicnnedisT[67]}}%

% basic north-north-east dotted arrow
\def\basicnnedotar[#1]{\NNEDOTAR{}{}{#100}}%

% north-north-east dotted arrow
\newcommand{\nnedotar}{\@ifnextchar[{\basicnnedotar}{\basicnnedotar[67]}}%

% basic north-north-east dotted arrow with upper name
\def\basicNnedotar[#1]#2{\NNEDOTAR{#2}{}{#100}}%

% north-north-east dotted arrow with upper name
\newcommand{\Nnedotar}{\@ifnextchar[{\basicNnedotar}{\basicNnedotar[67]}}%

% basic north-north-east dotted arrow with lower name
\def\basicnnedotaR[#1]#2{\NNEDOTAR{}{#2}{#100}}%

% north-north-east dotted arrow with lower name
\newcommand{\nnedotaR}{\@ifnextchar[{\basicnnedotaR}{\basicnnedotaR[67]}}%

% basic north-north-east monomorphism
\def\basicnnemono[#1]{\NNEMONO{}{}{#100}}%

% north-north-east monomorphism
\newcommand{\nnemono}{\@ifnextchar[{\basicnnemono}{\basicnnemono[67]}}%

% basic north-north-east monomorphism with upper name
\def\basicNnemono[#1]#2{\NNEMONO{#2}{}{#100}}%

% north-north-east monomorphism with upper name
\newcommand{\Nnemono}{\@ifnextchar[{\basicNnemono}{\basicNnemono[67]}}%

% basic north-north-east monomorphism with lower name
\def\basicnnemonO[#1]#2{\NNEMONO{}{#2}{#100}}%

% north-north-east monomorphism with lower name
\newcommand{\nnemonO}{\@ifnextchar[{\basicnnemonO}{\basicnnemonO[67]}}%

% basic north-north-east epimorphism
\def\basicnneepi[#1]{\NNEEPI{}{}{#100}}%

% north-north-east epimorphism
\newcommand{\nneepi}{\@ifnextchar[{\basicnneepi}{\basicnneepi[67]}}%

% basic north-north-east epimorphism with upper name
\def\basicNneepi[#1]#2{\NNEEPI{#2}{}{#100}}%

% north-north-east epimorphism with upper name
\newcommand{\Nneepi}{\@ifnextchar[{\basicNneepi}{\basicNneepi[67]}}%

% basic north-north-east epimorphism with lower name
\def\basicnneepI[#1]#2{\NNEEPI{}{#2}{#100}}%

% north-north-east epimorphism with lower name
\newcommand{\nneepI}{\@ifnextchar[{\basicnneepI}{\basicnneepI[67]}}%

% basic north-north-east bimorphism
\def\basicnnebimo[#1]{\NNEBIMO{}{}{#100}}%

% north-north-east bimorphism
\newcommand{\nnebimo}{\@ifnextchar[{\basicnnebimo}{\basicnnebimo[67]}}%

% basic north-north-east bimorphism with upper name
\def\basicNnebimo[#1]#2{\NNEBIMO{#2}{}{#100}}%

% north-north-east bimorphism with upper name
\newcommand{\Nnebimo}{\@ifnextchar[{\basicNnebimo}{\basicNnebimo[67]}}%

% basic north-north-east bimorphism with lower name
\def\basicnnebimO[#1]#2{\NNEBIMO{}{#2}{#100}}%

% north-north-east bimorphism with lower name
\newcommand{\nnebimO}{\@ifnextchar[{\basicnnebimO}{\basicnnebimO[67]}}%

% basic north-north-east isomorphism
\def\basicnneiso[#1]{\NNEAR{\cong}{}{#100}}%

% north-north-east isomorphism
\newcommand{\nneiso}{\@ifnextchar[{\basicnneiso}{\basicnneiso[67]}}%

% basic north-north-east isomorphism with upper name
\def\basicNneiso[#1]#2{\NNEAR{#2}{\cong}{#100}}%

% north-north-east isomorphism with upper name
\newcommand{\Nneiso}{\@ifnextchar[{\basicNneiso}{\basicNneiso[67]}}%

% basic north-north-east isomorphism with lower name
\def\basicnneisO[#1]#2{\NNEAR{\cong}{#2}{#100}}%

% north-north-east isomorphism with lower name
\newcommand{\nneisO}{\@ifnextchar[{\basicnneisO}{\basicnneisO[67]}}%

% basic north-north-east equality
\def\basicnneeql[#1]{\NNEEQL{}{}{#100}}%

% north-north-east equality
\newcommand{\nneeql}{\@ifnextchar[{\basicnneeql}{\basicnneeql[67]}}%

% basic north-north-east equality with upper name
\def\basicNneeql[#1]#2{\NNEEQL{#2}{}{#100}}%

% north-north-east equality with upper name
\newcommand{\Nneeql}{\@ifnextchar[{\basicNneeql}{\basicNneeql[67]}}%

% basic north-north-east equality with lower name
\def\basicnneeqL[#1]#2{\NNEEQL{}{#2}{#100}}%

% north-north-east equality with lower name
\newcommand{\nneeqL}{\@ifnextchar[{\basicnneeqL}{\basicnneeqL[67]}}%

% basic north-north-east pair of arrows
\def\basicnnebiar[#1]{\NNEBIAR{}{}{#100}}%

% north-north-east pair of arrows
\newcommand{\nnebiar}{\@ifnextchar[{\basicnnebiar}{\basicnnebiar[67]}}%

% basic north-north-east pair of arrows with names
\def\basicNnebiar[#1]#2#3{\NNEBIAR{#2}{#3}{#100}}%

% north-north-east pair of arrows with names
\newcommand{\Nnebiar}{\@ifnextchar[{\basicNnebiar}{\basicNnebiar[67]}}%
\let\nnebiaR=\Nnebiar

% basic north-north-east pair of distributors
\def\basicnnebidist[#1]{\NNEBIDIST{}{}{#100}}%

% north-north-east pair of distributors
\newcommand{\nnebidist}{\@ifnextchar[{\basicnnebidist}{\basicnnebidist[67]}}%

% basic north-north-east pair of distributors with names
\def\basicNnebidist[#1]#2#3{\NNEBIDIST{#2}{#3}{#100}}%

% north-north-east pair of distributors with names
\newcommand{\Nnebidist}{\@ifnextchar[{\basicNnebidist}{\basicNnebidist[67]}}%
\let\nnebidisT=\Nnebidist

% basic north-north-east pair of adjoint arrows
\def\basicnneadjar[#1]{\NNEADJAR{}{}{#100}}%

% north-north-east pair of adjoint arrows
\newcommand{\nneadjar}{\@ifnextchar[{\basicnneadjar}{\basicnneadjar[67]}}%

% basic north-north-east pair of adjoint  arrows with names
\def\basicNneadjar[#1]#2#3{\NNEADJAR{#2}{#3}{#100}}%

% north-north-east pair of adjoint arrows with names
\newcommand{\Nneadjar}{\@ifnextchar[{\basicNneadjar}{\basicNneadjar[67]}}%
\let\nneadjaR=\Nneadjar

% basic north-north-east pair of adjoint distributors
\def\basicnneadjdist[#1]{\NNEADJDIST{}{}{#100}}%

% north-north-east pair of adjoint distributors
\newcommand{\nneadjdist}{\@ifnextchar[{\basicnneadjdist}{\basicnneadjdist[67]}}%

% basic north-north-east pair of adjoint distributors with names
\def\basicNneadjdist[#1]#2#3{\NNEADJDIST{#2}{#3}{#100}}%

% north-north-east pair of adjoint distributors with names
\newcommand{\Nneadjdist}{\@ifnextchar[{\basicNneadjdist}{\basicNneadjdist[67]}}%
\let\nneadjdisT=\Nneadjdist


% SOUTH-SOUTH-EAST ARROWS

% The following commands produce south-south-east arrows
% of horizontal extent n units

% \SSEAR{f}{g}{n} draws a south-south-east arrow with names f, g
% and length n units
\newcommand{\SSEAR}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Z,#3){\line(1,-2){#3}}%
\put(\Z,-#3){\ssehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEDIST{f}{g}{n} draws a south-south-east distributor
% with names f, g and length n units
\newcommand{\SSEDIST}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Z,#3){\line(1,-2){#3}}%
\put(\Z,-#3){\ssehead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\SSEDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Z=#3%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{z}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(-\Z,#3)(\value{z},-\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(\Z,-#3){\ssehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEMONO{f}{g}{n} draws a south-south-east monomorphism
% with names f,g and length n units
\newcommand{\SSEMONO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\begin{picture}(0,0)%
\put(-\monolength,\secondmonolength){\line(1,-2){\bimolength}}%
\put(-\monolength,\secondmonolength){\ssehead}%
\put(\Z,-#3){\ssehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEEPI{f}{g}{n} draws a south-south-east epimorphism
% with names f, g and length n units
\newcommand{\SSEEPI}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\trueheaD%
\bimolength=#3%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\Z%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\Z,#3){\line(1,-2){\bimolength}}%
\put(\epilength,-\secondepilength){\ssehead}%
\put(\Z,-#3){\ssehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEBIMO{f}{g}{n} draws a south-south-east bimorphism
% with names f,g and length n units
\newcommand{\SSEBIMO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL\trueheaD%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(-\monolength,\secondmonolength){\line(1,-2){\bimolength}}%
\put(-\monolength,\secondmonolength){\ssehead}%
\put(\epilength,-\secondepilength){\ssehead}%
\put(\Z,-#3){\ssehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEEQL{f}{g}{n} draws a south-south-east equality
% with names f,g and length n units
\newcommand{\SSEEQL}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(-\Z,#3){\begin{picture}(0,0)%
\truex{44}\truey{89}%
\put(-\value{y},-\value{x}){\line(1,-2){#3}}%
\put(\value{y},\value{x}){\line(1,-2){#3}}%
\end{picture}}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEBIAR{f}{g}{n} draws a pair of south-south-east arrows
% with names f,g and length n units
\newcommand{\SSEBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(-\Y,#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\put(-\value{x},-\value{y}){\line(1,-2){#3}}%
\put(\value{x},\value{y}){\line(1,-2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\monolength,-\secondepilength){\ssehead}%
\put(\epilength,-\secondmonolength){\ssehead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEBIDIST{f}{g}{n} draws a pair of south-south-east distributors
% with names f,g and length n units
\newcommand{\SSEBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(-\Y,#3){\begin{picture}(0,0)%
\put(-\value{x},-\value{y}){\line(1,-2){#3}}%
\put(\value{x},\value{y}){\line(1,-2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\monolength,-\secondepilength){\ssehead}%
\put(\epilength,-\secondmonolength){\ssehead}%
\end{picture}}
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\put(\value{x},\value{y}){\circle{\value{z}}}%
\truex{500}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEADJAR{f}{g}{n} draws a south-south-east pair of adjoint arrows
% with names f,g and length n units
\newcommand{\SSEADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(-\Y,#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(1,-2){#3}}%
\put(\monolength,-\secondepilength){\ssehead}%
\put(\epilength,-\secondmonolength){\line(-1,2){#3}}%
\put(\value{x},\value{y}){\nnwhead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \SSEADJDIST{f}{g}{n} draws a south-south-east pair of adjoint distributors
% with names f,g and length n units
\newcommand{\SSEADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(-\Y,#3){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(1,-2){#3}}%
\put(\monolength,-\secondepilength){\ssehead}%
\put(\epilength,-\secondmonolength){\line(-1,2){#3}}%
\put(\value{x},\value{y}){\nnwhead}%
\end{picture}}
\put(\value{x},\value{y}){\circle{\value{z}}}%
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\truex{500}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%


% The following commands produce south-south-east arrows;
% the default length is 6700 units

% basic south-south-east arrow
\def\basicssear[#1]{\SSEAR{}{}{#100}}%

% south-south-east arrow
\newcommand{\ssear}{\@ifnextchar[{\basicssear}{\basicssear[67]}}%

% basic south-south-east arrow with upper name
\def\basicSsear[#1]#2{\SSEAR{#2}{}{#100}}%

% south-south-east arrow with upper name
\newcommand{\Ssear}{\@ifnextchar[{\basicSsear}{\basicSsear[67]}}%

% basic south-south-east arrow with lower name
\def\basicsseaR[#1]#2{\SSEAR{}{#2}{#100}}%

% south-south-east arrow with lower name
\newcommand{\sseaR}{\@ifnextchar[{\basicsseaR}{\basicsseaR[67]}}%

% basic south-south-east distributor
\def\basicssedist[#1]{\SSEDIST{}{}{#100}}%

% south-south-east distributor
\newcommand{\ssedist}{\@ifnextchar[{\basicssedist}{\basicssedist[67]}}%

% basic south-south-east distributor with upper name
\def\basicSsedist[#1]#2{\SSEDIST{#2}{}{#100}}%

% south-south-east distributor with upper name
\newcommand{\Ssedist}{\@ifnextchar[{\basicSsedist}{\basicSsedist[67]}}%

% basic south-south-east distributor with lower name
\def\basicssedisT[#1]#2{\SSEDIST{}{#2}{#100}}%

% south-south-east distributor with lower name
\newcommand{\ssedisT}{\@ifnextchar[{\basicssedisT}{\basicssedisT[67]}}%

% basic south-south-east dotted arrow
\def\basicssedotar[#1]{\SSEDOTAR{}{}{#100}}%

% south-south-east dotted arrow
\newcommand{\ssedotar}{\@ifnextchar[{\basicssedotar}{\basicssedotar[67]}}%

% basic south-south-east dotted arrow with upper name
\def\basicSsedotar[#1]#2{\SSEDOTAR{#2}{}{#100}}%

% south-south-east dotted arrow with upper name
\newcommand{\Ssedotar}{\@ifnextchar[{\basicSsedotar}{\basicSsedotar[67]}}%

% basic south-south-east dotted arrow with lower name
\def\basicssedotaR[#1]#2{\SSEDOTAR{}{#2}{#100}}%

% south-south-east dotted arrow with lower name
\newcommand{\ssedotaR}{\@ifnextchar[{\basicssedotaR}{\basicssedotaR[67]}}%

% basic south-south-east monomorphism
\def\basicssemono[#1]{\SSEMONO{}{}{#100}}%

% south-south-east monomorphism
\newcommand{\ssemono}{\@ifnextchar[{\basicssemono}{\basicssemono[67]}}%

% basic south-south-east monomorphism with upper name
\def\basicSsemono[#1]#2{\SSEMONO{#2}{}{#100}}%

% south-south-east monomorphism with upper name
\newcommand{\Ssemono}{\@ifnextchar[{\basicSsemono}{\basicSsemono[67]}}%

% basic south-south-east monomorphism with lower name
\def\basicssemonO[#1]#2{\SSEMONO{}{#2}{#100}}%

% south-south-east monomorphism with lower name
\newcommand{\ssemonO}{\@ifnextchar[{\basicssemonO}{\basicssemonO[67]}}%

% basic south-south-east epimorphism
\def\basicsseepi[#1]{\SSEEPI{}{}{#100}}%

% south-south-east epimorphism
\newcommand{\sseepi}{\@ifnextchar[{\basicsseepi}{\basicsseepi[67]}}%

% basic south-south-east epimorphism with upper name
\def\basicSseepi[#1]#2{\SSEEPI{#2}{}{#100}}%

% south-south-east epimorphism with upper name
\newcommand{\Sseepi}{\@ifnextchar[{\basicSseepi}{\basicSseepi[67]}}%

% basic south-south-east epimorphism with lower name
\def\basicsseepI[#1]#2{\SSEEPI{}{#2}{#100}}%

% south-south-east epimorphism with lower name
\newcommand{\sseepI}{\@ifnextchar[{\basicsseepI}{\basicsseepI[67]}}%

% basic south-south-east bimorphism
\def\basicssebimo[#1]{\SSEBIMO{}{}{#100}}%

% south-south-east bimorphism
\newcommand{\ssebimo}{\@ifnextchar[{\basicssebimo}{\basicssebimo[67]}}%

% basic south-south-east bimorphism with upper name
\def\basicSsebimo[#1]#2{\SSEBIMO{#2}{}{#100}}%

% south-south-east bimorphism with upper name
\newcommand{\Ssebimo}{\@ifnextchar[{\basicSsebimo}{\basicSsebimo[67]}}%

% basic south-south-east bimorphism with lower name
\def\basicssebimO[#1]#2{\SSEBIMO{}{#2}{#100}}%

% south-south-east bimorphism with lower name
\newcommand{\ssebimO}{\@ifnextchar[{\basicssebimO}{\basicssebimO[67]}}%

% basic south-south-east isomorphism
\def\basicsseiso[#1]{\SSEAR{\cong}{}{#100}}%

% south-south-east isomorphism
\newcommand{\sseiso}{\@ifnextchar[{\basicsseiso}{\basicsseiso[67]}}%

% basic south-south-east isomorphism with upper name
\def\basicSseiso[#1]#2{\SSEAR{#2}{\cong}{#100}}%

% south-south-east isomorphism with upper name
\newcommand{\Sseiso}{\@ifnextchar[{\basicSseiso}{\basicSseiso[67]}}%

% basic south-south-east isomorphism with lower name
\def\basicsseisO[#1]#2{\SSEAR{\cong}{#2}{#100}}%

% south-south-east isomorphism with lower name
\newcommand{\sseisO}{\@ifnextchar[{\basicsseisO}{\basicsseisO[67]}}%

% basic south-south-east equality
\def\basicsseeql[#1]{\SSEEQL{}{}{#100}}%

% south-south-east equality
\newcommand{\sseeql}{\@ifnextchar[{\basicsseeql}{\basicsseeql[67]}}%

% basic south-south-east equality with upper name
\def\basicSseeql[#1]#2{\SSEEQL{#2}{}{#100}}%

% south-south-east equality with upper name
\newcommand{\Sseeql}{\@ifnextchar[{\basicSseeql}{\basicSseeql[67]}}%

% basic south-south-east equality with lower name
\def\basicsseeqL[#1]#2{\SSEEQL{}{#2}{#100}}%

% south-south-east equality with lower name
\newcommand{\sseeqL}{\@ifnextchar[{\basicsseeqL}{\basicsseeqL[67]}}%

% basic south-south-east pair of arrows
\def\basicssebiar[#1]{\SSEBIAR{}{}{#100}}%

% south-south-east pair of arrows
\newcommand{\ssebiar}{\@ifnextchar[{\basicssebiar}{\basicssebiar[67]}}%

% basic south-south-east pair of arrows with names
\def\basicSsebiar[#1]#2#3{\SSEBIAR{#2}{#3}{#100}}%

% south-south-east pair of arrows with names
\newcommand{\Ssebiar}{\@ifnextchar[{\basicSsebiar}{\basicSsebiar[67]}}%
\let\ssebiaR=\Ssebiar

% basic south-south-east pair of distributors
\def\basicssebidist[#1]{\SSEBIDIST{}{}{#100}}%

% south-south-east pair of distributors
\newcommand{\ssebidist}{\@ifnextchar[{\basicssebidist}{\basicssebidist[67]}}%

% basic south-south-east pair of distributors with names
\def\basicSsebidist[#1]#2#3{\SSEBIDIST{#2}{#3}{#100}}%

% south-south-east pair of distributors with names
\newcommand{\Ssebidist}{\@ifnextchar[{\basicSsebidist}{\basicSsebidist[67]}}%
\let\ssebidisT=\Ssebidist

% basic south-south-east pair of adjoint arrows
\def\basicsseadjar[#1]{\SSEADJAR{}{}{#100}}%

% south-south-east pair of adjoint arrows
\newcommand{\sseadjar}{\@ifnextchar[{\basicsseadjar}{\basicsseadjar[67]}}%

% basic south-south-east pair of adjoint  arrows with names
\def\basicSseadjar[#1]#2#3{\SSEADJAR{#2}{#3}{#100}}%

% south-south-east pair of adjoint arrows with names
\newcommand{\Sseadjar}{\@ifnextchar[{\basicSseadjar}{\basicSseadjar[67]}}%
\let\sseadjaR=\Sseadjar

% basic south-south-east pair of adjoint distributors
\def\basicsseadjdist[#1]{\SSEADJDIST{}{}{#100}}%

% south-south-east pair of adjoint distributors
\newcommand{\sseadjdist}{\@ifnextchar[{\basicsseadjdist}{\basicsseadjdist[67]}}%

% basic south-south-east pair of adjoint distributors with names
\def\basicSseadjdist[#1]#2#3{\SSEADJDIST{#2}{#3}{#100}}%

% south-south-east pair of adjoint distributors with names
\newcommand{\Sseadjdist}{\@ifnextchar[{\basicSseadjdist}{\basicSseadjdist[67]}}%
\let\sseadjdisT=\Sseadjdist


% SOUTH-SOUTH-WEST ARROWS

% The following commands produce south-south-west arrows
% of horizontal extent n units

% \SSWAR{f}{g}{n} draws a south-south-west arrow with names f, g
% and length n units
\newcommand{\SSWAR}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Z,#3){\line(-1,-2){#3}}%
\put(-\Z,-#3){\sswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWDIST{f}{g}{n} draws a south-south-west distributor
% with names f, g and length n units
\newcommand{\SSWDIST}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Z,#3){\line(-1,-2){#3}}%
\put(-\Z,-#3){\sswhead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\SSWDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Z=#3%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{z}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(\Z,#3)(-\value{z},-\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(-\Z,-#3){\sswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWMONO{f}{g}{n} draws a south-south-west monomorphism
% with names f,g and length n units
\newcommand{\SSWMONO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\begin{picture}(0,0)%
\put(\monolength,\secondmonolength){\line(-1,-2){\bimolength}}%
\put(\monolength,\secondmonolength){\sswhead}%
\put(-\Z,-#3){\sswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWEPI{f}{g}{n} draws a south-south-west epimorphism
% with names f, g and length n units
\newcommand{\SSWEPI}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\trueheaD%
\bimolength=#3%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\Z%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(\Z,#3){\line(-1,-2){\bimolength}}%
\put(-\epilength,-\secondepilength){\sswhead}%
\put(-\Z,-#3){\sswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWBIMO{f}{g}{n} draws a south-south-west bimorphism
% with names f,g and length n units
\newcommand{\SSWBIMO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL\trueheaD%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(\monolength,\secondmonolength){\line(-1,-2){\bimolength}}%
\put(\monolength,\secondmonolength){\sswhead}%
\put(-\epilength,-\secondepilength){\sswhead}%
\put(-\Z,-#3){\sswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWBIAR{f}{g}{n} draws a pair of south-south-west arrows
% with names f,g and length n units
\newcommand{\SSWBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(\Y,#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\put(-\value{x},\value{y}){\line(-1,-2){#3}}%
\put(\value{x},-\value{y}){\line(-1,-2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\monolength,-\secondepilength){\sswhead}%
\put(-\epilength,-\secondmonolength){\sswhead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWBIDIST{f}{g}{n} draws a pair of south-south-west distributors
% with names f,g and length n units
\newcommand{\SSWBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(\Y,#3){\begin{picture}(0,0)%
\put(-\value{x},\value{y}){\line(-1,-2){#3}}%
\put(\value{x},-\value{y}){\line(-1,-2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\monolength,-\secondepilength){\sswhead}%
\put(-\epilength,-\secondmonolength){\sswhead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWADJAR{f}{g}{n} draws a south-south-west pair of adjoint arrows
% with names f,g and length n units
\newcommand{\SSWADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(\Y,#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(-1,-2){#3}}%
\put(-\monolength,-\secondepilength){\sswhead}%
\put(-\epilength,-\secondmonolength){\line(1,2){#3}}%
\put(-\value{x},\value{y}){\nnehead}%
\end{picture}}
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% \SSWADJDIST{f}{g}{n} draws a south-south-west pair of adjoint distributors
% with names f,g and length n units
\newcommand{\SSWADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(\Y,#3){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(\value{x},-\value{y}){\line(-1,-2){#3}}%
\put(-\monolength,-\secondepilength){\sswhead}%
\put(-\epilength,-\secondmonolength){\line(1,2){#3}}%
\put(-\value{x},\value{y}){\nnehead}%
\end{picture}}
\put(-\value{x},\value{y}){\circle{\value{z}}}%
\put(\value{x},-\value{y}){\circle{\value{z}}}%
\truex{300}\truey{1000}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% The following commands produce south-south-west arrows;
% the default length is 6700 units

% basic south-south-west arrow
\def\basicsswar[#1]{\SSWAR{}{}{#100}}%

% south-south-west arrow
\newcommand{\sswar}{\@ifnextchar[{\basicsswar}{\basicsswar[67]}}%

% basic south-south-west arrow with upper name
\def\basicSswar[#1]#2{\SSWAR{#2}{}{#100}}%

% south-south-west arrow with upper name
\newcommand{\Sswar}{\@ifnextchar[{\basicSswar}{\basicSswar[67]}}%

% basic south-south-west arrow with lower name
\def\basicsswaR[#1]#2{\SSWAR{}{#2}{#100}}%

% south-south-west arrow with lower name
\newcommand{\sswaR}{\@ifnextchar[{\basicsswaR}{\basicsswaR[67]}}%

% basic south-south-west distributor
\def\basicsswdist[#1]{\SSWDIST{}{}{#100}}%

% south-south-west distributor
\newcommand{\sswdist}{\@ifnextchar[{\basicsswdist}{\basicsswdist[67]}}%

% basic south-south-west distributor with upper name
\def\basicSswdist[#1]#2{\SSWDIST{#2}{}{#100}}%

% south-south-west distributor with upper name
\newcommand{\Sswdist}{\@ifnextchar[{\basicSswdist}{\basicSswdist[67]}}%

% basic south-south-west distributor with lower name
\def\basicsswdisT[#1]#2{\SSWDIST{}{#2}{#100}}%

% south-south-west distributor with lower name
\newcommand{\sswdisT}{\@ifnextchar[{\basicsswdisT}{\basicsswdisT[67]}}%

% basic south-south-west dotted arrow
\def\basicsswdotar[#1]{\SSWDOTAR{}{}{#100}}%

% south-south-west dotted arrow
\newcommand{\sswdotar}{\@ifnextchar[{\basicsswdotar}{\basicsswdotar[67]}}%

% basic south-south-west dotted arrow with upper name
\def\basicSswdotar[#1]#2{\SSWDOTAR{#2}{}{#100}}%

% south-south-west dotted arrow with upper name
\newcommand{\Sswdotar}{\@ifnextchar[{\basicSswdotar}{\basicSswdotar[67]}}%

% basic south-south-west dotted arrow with lower name
\def\basicsswdotaR[#1]#2{\SSWDOTAR{}{#2}{#100}}%

% south-south-west dotted arrow with lower name
\newcommand{\sswdotaR}{\@ifnextchar[{\basicsswdotaR}{\basicsswdotaR[67]}}%

% basic south-south-west monomorphism
\def\basicsswmono[#1]{\SSWMONO{}{}{#100}}%

% south-south-west monomorphism
\newcommand{\sswmono}{\@ifnextchar[{\basicsswmono}{\basicsswmono[67]}}%

% basic south-south-west monomorphism with upper name
\def\basicSswmono[#1]#2{\SSWMONO{#2}{}{#100}}%

% south-south-west monomorphism with upper name
\newcommand{\Sswmono}{\@ifnextchar[{\basicSswmono}{\basicSswmono[67]}}%

% basic south-south-west monomorphism with lower name
\def\basicsswmonO[#1]#2{\SSWMONO{}{#2}{#100}}%

% south-south-west monomorphism with lower name
\newcommand{\sswmonO}{\@ifnextchar[{\basicsswmonO}{\basicsswmonO[67]}}%

% basic south-south-west epimorphism
\def\basicsswepi[#1]{\SSWEPI{}{}{#100}}%

% south-south-west epimorphism
\newcommand{\sswepi}{\@ifnextchar[{\basicsswepi}{\basicsswepi[67]}}%

% basic south-south-west epimorphism with upper name
\def\basicSswepi[#1]#2{\SSWEPI{#2}{}{#100}}%

% south-south-west epimorphism with upper name
\newcommand{\Sswepi}{\@ifnextchar[{\basicSswepi}{\basicSswepi[67]}}%

% basic south-south-west epimorphism with lower name
\def\basicsswepI[#1]#2{\SSWEPI{}{#2}{#100}}%

% south-south-west epimorphism with lower name
\newcommand{\sswepI}{\@ifnextchar[{\basicsswepI}{\basicsswepI[67]}}%

% basic south-south-west bimorphism
\def\basicsswbimo[#1]{\SSWBIMO{}{}{#100}}%

% south-south-west bimorphism
\newcommand{\sswbimo}{\@ifnextchar[{\basicsswbimo}{\basicsswbimo[67]}}%

% basic south-south-west bimorphism with upper name
\def\basicSswbimo[#1]#2{\SSWBIMO{#2}{}{#100}}%

% south-south-west bimorphism with upper name
\newcommand{\Sswbimo}{\@ifnextchar[{\basicSswbimo}{\basicSswbimo[67]}}%

% basic south-south-west bimorphism with lower name
\def\basicsswbimO[#1]#2{\SSWBIMO{}{#2}{#100}}%

% south-south-west bimorphism with lower name
\newcommand{\sswbimO}{\@ifnextchar[{\basicsswbimO}{\basicsswbimO[67]}}%

% basic south-south-west isomorphism
\def\basicsswiso[#1]{\SSWAR{\cong}{}{#100}}%

% south-south-west isomorphism
\newcommand{\sswiso}{\@ifnextchar[{\basicsswiso}{\basicsswiso[67]}}%

% basic south-south-west isomorphism with upper name
\def\basicSswiso[#1]#2{\SSWAR{#2}{\cong}{#100}}%

% south-south-west isomorphism with upper name
\newcommand{\Sswiso}{\@ifnextchar[{\basicSswiso}{\basicSswiso[67]}}%

% basic south-south-west isomorphism with lower name
\def\basicsswisO[#1]#2{\SSWAR{\cong}{#2}{#100}}%

% south-south-west isomorphism with lower name
\newcommand{\sswisO}{\@ifnextchar[{\basicsswisO}{\basicsswisO[67]}}%

% south-south-west equality
\let\ssweql=\nneeql%

% south-south-west equality with upper name
\let\Ssweql=\Nneeql%

% south-south-west equality with lower name
\let\ssweqL=\nneeqL%

% basic south-south-west pair of arrows
\def\basicsswbiar[#1]{\SSWBIAR{}{}{#100}}%

% south-south-west pair of arrows
\newcommand{\sswbiar}{\@ifnextchar[{\basicsswbiar}{\basicsswbiar[67]}}%

% basic south-south-west pair of arrows with names
\def\basicSswbiar[#1]#2#3{\SSWBIAR{#2}{#3}{#100}}%

% south-south-west pair of arrows with names
\newcommand{\Sswbiar}{\@ifnextchar[{\basicSswbiar}{\basicSswbiar[67]}}%
\let\sswbiaR=\Sswbiar

% basic south-south-west pair of distributors
\def\basicsswbidist[#1]{\SSWBIDIST{}{}{#100}}%

% south-south-west pair of distributors
\newcommand{\sswbidist}{\@ifnextchar[{\basicsswbidist}{\basicsswbidist[67]}}%

% basic south-south-west pair of distributors with names
\def\basicSswbidist[#1]#2#3{\SSWBIDIST{#2}{#3}{#100}}%

% south-south-west pair of distributors with names
\newcommand{\Sswbidist}{\@ifnextchar[{\basicSswbidist}{\basicSswbidist[67]}}%
\let\sswbidisT=\Sswbidist

% basic south-south-west pair of adjoint arrows
\def\basicsswadjar[#1]{\SSWADJAR{}{}{#100}}%

% south-south-west pair of adjoint arrows
\newcommand{\sswadjar}{\@ifnextchar[{\basicsswadjar}{\basicsswadjar[67]}}%

% basic south-south-west pair of adjoint  arrows with names
\def\basicSswadjar[#1]#2#3{\SSWADJAR{#2}{#3}{#100}}%

% south-south-west pair of adjoint arrows with names
\newcommand{\Sswadjar}{\@ifnextchar[{\basicSswadjar}{\basicSswadjar[67]}}%
\let\sswadjaR=\Sswadjar

% basic south-south-west pair of adjoint distributors
\def\basicsswadjdist[#1]{\SSWADJDIST{}{}{#100}}%

% south-south-west pair of adjoint distributors
\newcommand{\sswadjdist}{\@ifnextchar[{\basicsswadjdist}{\basicsswadjdist[67]}}%

% basic south-south-west pair of adjoint distributors with names
\def\basicSswadjdist[#1]#2#3{\SSWADJDIST{#2}{#3}{#100}}%

% south-south-west pair of adjoint distributors with names
\newcommand{\Sswadjdist}{\@ifnextchar[{\basicSswadjdist}{\basicSswadjdist[67]}}%
\let\sswadjdisT=\Sswadjdist


% NORTH-NORTH-WEST ARROWS

% The following commands produce north-north-west arrows
% of horizontal extent n units

% \NNWAR{f}{g}{n} draws a north-north-west arrow with names f, g
% and length n units
\newcommand{\NNWAR}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Z,-#3){\line(-1,2){#3}}%
\put(-\Z,#3){\nnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWDIST{f}{g}{n} draws a north-north-west distributor
% with names f, g and length n units
\newcommand{\NNWDIST}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\begin{picture}(0,0)%
\put(\Z,-#3){\line(-1,2){#3}}%
\put(-\Z,#3){\nnwhead}%
\truex{400}%
\put(0,0){\circle{\value{x}}}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWDOTAR{f}{g}{n} draws a north-east dotted arrow
% with names f,g and length n units
\newcommand{\NNWDOTAR}[3]{\testdiagrammode%
\truex{100}\truey{268}\truez{134}%
\Z=#3%
\divide\Z by 2%
\NUMBEROFDOTS=#3%
\divide\NUMBEROFDOTS by \value{z}%
\advance\NUMBEROFDOTS by 1%
\begin{picture}(0,0)%
\multiput(\Z,-#3)(-\value{z},\value{y}){\NUMBEROFDOTS}%
{\circle*{\value{x}}}%
\put(-\Z,#3){\nnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWMONO{f}{g}{n} draws a north-north-west monomorphism
% with names f,g and length n units
\newcommand{\NNWMONO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\begin{picture}(0,0)%
\put(\monolength,-\secondmonolength){\line(-1,2){\bimolength}}%
\put(\monolength,-\secondmonolength){\nnwhead}%
\put(-\Z,#3){\nnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWEPI{f}{g}{n} draws a north-north-west epimorphism
% with names f, g and length n units
\newcommand{\NNWEPI}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\trueheaD%
\bimolength=#3%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\Z%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(\Z,-#3){\line(-1,2){\bimolength}}%
\put(-\epilength,\secondepilength){\nnwhead}%
\put(-\Z,#3){\nnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWBIMO{f}{g}{n} draws a north-north-west bimorphism
% with names f,g and length n units
\newcommand{\NNWBIMO}[3]{\testdiagrammode%
\Z=#3%
\divide\Z by 2%
\truetaiL\trueheaD%
\bimolength=#3%
\advance\bimolength by -\truemonotaiL%
\monolength=\bimolength%
\advance\monolength by -\Z%
\advance\bimolength by -\trueepiheaD%
\epilength=\bimolength%
\advance\epilength by -\monolength%
\secondmonolength=\monolength%
\multiply\secondmonolength by 2%
\secondepilength=\epilength%
\multiply\secondepilength by 2%
\begin{picture}(0,0)%
\put(\monolength,-\secondmonolength){\line(-1,2){\bimolength}}%
\put(\monolength,-\secondmonolength){\nnwhead}%
\put(-\epilength,\secondepilength){\nnwhead}%
\put(-\Z,#3){\nnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWBIAR{f}{g}{n} draws a pair of north-north-west arrows
% with names f,g and length n units
\newcommand{\NNWBIAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(\Y,-#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\put(-\value{x},-\value{y}){\line(-1,2){#3}}%
\put(\value{x},\value{y}){\line(-1,2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\monolength,\secondepilength){\nnwhead}%
\put(-\epilength,\secondmonolength){\nnwhead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWBIDIST{f}{g}{n} draws a pair of north-north-west distributors
% with names f,g and length n units
\newcommand{\NNWBIDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(\Y,-#3){\begin{picture}(0,0)%
\put(-\value{x},-\value{y}){\line(-1,2){#3}}%
\put(\value{x},\value{y}){\line(-1,2){#3}}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\monolength,\secondepilength){\nnwhead}%
\put(-\epilength,\secondmonolength){\nnwhead}%
\end{picture}}
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\put(\value{x},\value{y}){\circle{\value{z}}}%
\truex{500}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWADJAR{f}{g}{n} draws a north-north-west pair of adjoint arrows
% with names f,g and length n units
\newcommand{\NNWADJAR}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\put(\Y,-#3){\begin{picture}(0,0)%
\truex{313}\truey{156}%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(-1,2){#3}}%
\put(-\epilength,\secondmonolength){\nnwhead}%
\put(-\monolength,\secondepilength){\line(1,-2){#3}}%
\put(\value{x},\value{y}){\ssehead}%
\end{picture}}
\truex{400}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% \NNWADJDIST{f}{g}{n} draws a north-north-west pair of adjoint distributors
% with names f,g and length n units
\newcommand{\NNWADJDIST}[3]{\testdiagrammode%
\Y=#3%
\divide\Y by 2%
\Z=#3%
\multiply \Z by 2%
\begin{picture}(0,0)%
\truex{313}\truey{156}\truez{400}%
\put(\Y,-#3){\begin{picture}(0,0)%
\monolength=#3%
\advance\monolength by -\value{x}%
\epilength=#3%
\advance\epilength by \value{x}%
\secondmonolength=\Z%
\advance\secondmonolength by -\value{y}%
\secondepilength=\Z%
\advance\secondepilength by \value{y}%
\put(-\value{x},-\value{y}){\line(-1,2){#3}}%
\put(-\epilength,\secondmonolength){\nnwhead}%
\put(-\monolength,\secondepilength){\line(1,-2){#3}}%
\put(\value{x},\value{y}){\ssehead}%
\end{picture}}
\put(\value{x},\value{y}){\circle{\value{z}}}%
\put(-\value{x},-\value{y}){\circle{\value{z}}}%
\truex{500}\truey{1000}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% The following commands produce north-north-west arrows;
% the default length is 6700 units

% basic north-north-west arrow
\def\basicnnwar[#1]{\NNWAR{}{}{#100}}%

% north-north-west arrow
\newcommand{\nnwar}{\@ifnextchar[{\basicnnwar}{\basicnnwar[67]}}%

% basic north-north-west arrow with upper name
\def\basicNnwar[#1]#2{\NNWAR{#2}{}{#100}}%

% north-north-west arrow with upper name
\newcommand{\Nnwar}{\@ifnextchar[{\basicNnwar}{\basicNnwar[67]}}%

% basic north-north-west arrow with lower name
\def\basicnnwaR[#1]#2{\NNWAR{}{#2}{#100}}%

% north-north-west arrow with lower name
\newcommand{\nnwaR}{\@ifnextchar[{\basicnnwaR}{\basicnnwaR[67]}}%

% basic north-north-west distributor
\def\basicnnwdist[#1]{\NNWDIST{}{}{#100}}%

% north-north-west distributor
\newcommand{\nnwdist}{\@ifnextchar[{\basicnnwdist}{\basicnnwdist[67]}}%

% basic north-north-west distributor with upper name
\def\basicNnwdist[#1]#2{\NNWDIST{#2}{}{#100}}%

% north-north-west distributor with upper name
\newcommand{\Nnwdist}{\@ifnextchar[{\basicNnwdist}{\basicNnwdist[67]}}%

% basic north-north-west distributor with lower name
\def\basicnnwdisT[#1]#2{\NNWDIST{}{#2}{#100}}%

% north-north-west distributor with lower name
\newcommand{\nnwdisT}{\@ifnextchar[{\basicnnwdisT}{\basicnnwdisT[67]}}%

% basic north-north-west dotted arrow
\def\basicnnwdotar[#1]{\NNWDOTAR{}{}{#100}}%

% north-north-west dotted arrow
\newcommand{\nnwdotar}{\@ifnextchar[{\basicnnwdotar}{\basicnnwdotar[67]}}%

% basic north-north-west dotted arrow with upper name
\def\basicNnwdotar[#1]#2{\NNWDOTAR{#2}{}{#100}}%

% north-north-west dotted arrow with upper name
\newcommand{\Nnwdotar}{\@ifnextchar[{\basicNnwdotar}{\basicNnwdotar[67]}}%

% basic north-north-west dotted arrow with lower name
\def\basicnnwdotaR[#1]#2{\NNWDOTAR{}{#2}{#100}}%

% north-north-west dotted arrow with lower name
\newcommand{\nnwdotaR}{\@ifnextchar[{\basicnnwdotaR}{\basicnnwdotaR[67]}}%

% basic north-north-west monomorphism
\def\basicnnwmono[#1]{\NNWMONO{}{}{#100}}%

% north-north-west monomorphism
\newcommand{\nnwmono}{\@ifnextchar[{\basicnnwmono}{\basicnnwmono[67]}}%

% basic north-north-west monomorphism with upper name
\def\basicNnwmono[#1]#2{\NNWMONO{#2}{}{#100}}%

% north-north-west monomorphism with upper name
\newcommand{\Nnwmono}{\@ifnextchar[{\basicNnwmono}{\basicNnwmono[67]}}%

% basic north-north-west monomorphism with lower name
\def\basicnnwmonO[#1]#2{\NNWMONO{}{#2}{#100}}%

% north-north-west monomorphism with lower name
\newcommand{\nnwmonO}{\@ifnextchar[{\basicnnwmonO}{\basicnnwmonO[67]}}%

% basic north-north-west epimorphism
\def\basicnnwepi[#1]{\NNWEPI{}{}{#100}}%

% north-north-west epimorphism
\newcommand{\nnwepi}{\@ifnextchar[{\basicnnwepi}{\basicnnwepi[67]}}%

% basic north-north-west epimorphism with upper name
\def\basicNnwepi[#1]#2{\NNWEPI{#2}{}{#100}}%

% north-north-west epimorphism with upper name
\newcommand{\Nnwepi}{\@ifnextchar[{\basicNnwepi}{\basicNnwepi[67]}}%

% basic north-north-west epimorphism with lower name
\def\basicnnwepI[#1]#2{\NNWEPI{}{#2}{#100}}%

% north-north-west epimorphism with lower name
\newcommand{\nnwepI}{\@ifnextchar[{\basicnnwepI}{\basicnnwepI[67]}}%

% basic north-north-west bimorphism
\def\basicnnwbimo[#1]{\NNWBIMO{}{}{#100}}%

% north-north-west bimorphism
\newcommand{\nnwbimo}{\@ifnextchar[{\basicnnwbimo}{\basicnnwbimo[67]}}%

% basic north-north-west bimorphism with upper name
\def\basicNnwbimo[#1]#2{\NNWBIMO{#2}{}{#100}}%

% north-north-west bimorphism with upper name
\newcommand{\Nnwbimo}{\@ifnextchar[{\basicNnwbimo}{\basicNnwbimo[67]}}%

% basic north-north-west bimorphism with lower name
\def\basicnnwbimO[#1]#2{\NNWBIMO{}{#2}{#100}}%

% north-north-west bimorphism with lower name
\newcommand{\nnwbimO}{\@ifnextchar[{\basicnnwbimO}{\basicnnwbimO[67]}}%

% basic north-north-west isomorphism
\def\basicnnwiso[#1]{\NNWAR{\cong}{}{#100}}%

% north-north-west isomorphism
\newcommand{\nnwiso}{\@ifnextchar[{\basicnnwiso}{\basicnnwiso[67]}}%

% basic north-north-west isomorphism with upper name
\def\basicNnwiso[#1]#2{\NNWAR{#2}{\cong}{#100}}%

% north-north-west isomorphism with upper name
\newcommand{\Nnwiso}{\@ifnextchar[{\basicNnwiso}{\basicNnwiso[67]}}%

% basic north-north-west isomorphism with lower name
\def\basicnnwisO[#1]#2{\NNWAR{\cong}{#2}{#100}}%

% north-north-west isomorphism with lower name
\newcommand{\nnwisO}{\@ifnextchar[{\basicnnwisO}{\basicnnwisO[67]}}%

% north-north-west equality
\let\nnweql=\sseeql%

% north-north-west equality with upper name
\let\Nnweql=\Sseeql%

% north-north-west equality with lower name
\let\nnweqL=\sseeqL%

% basic north-north-east pair of arrows
\def\basicnnwbiar[#1]{\NNWBIAR{}{}{#100}}%

% north-north-east pair of arrows
\newcommand{\nnwbiar}{\@ifnextchar[{\basicnnwbiar}{\basicnnwbiar[67]}}%

% basic north-north-east pair of arrows with names
\def\basicNnwbiar[#1]#2#3{\NNWBIAR{#2}{#3}{#100}}%

% north-north-east pair of arrows with names
\newcommand{\Nnwbiar}{\@ifnextchar[{\basicNnwbiar}{\basicNnwbiar[67]}}%
\let\nnwbiaR=\Nnwbiar

% basic north-north-east pair of distributors
\def\basicnnwbidist[#1]{\NNWBIDIST{}{}{#100}}%

% north-north-east pair of distributors
\newcommand{\nnwbidist}{\@ifnextchar[{\basicnnwbidist}{\basicnnwbidist[67]}}%

% basic north-north-east pair of distributors with names
\def\basicNnwbidist[#1]#2#3{\NNWBIDIST{#2}{#3}{#100}}%

% north-north-east pair of distributors with names
\newcommand{\Nnwbidist}{\@ifnextchar[{\basicNnwbidist}{\basicNnwbidist[67]}}%
\let\nnwbidisT=\Nnwbidist

% basic north-north-east pair of adjoint arrows
\def\basicnnwadjar[#1]{\NNWADJAR{}{}{#100}}%

% north-north-east pair of adjoint arrows
\newcommand{\nnwadjar}{\@ifnextchar[{\basicnnwadjar}{\basicnnwadjar[67]}}%

% basic north-north-east pair of adjoint  arrows with names
\def\basicNnwadjar[#1]#2#3{\NNWADJAR{#2}{#3}{#100}}%

% north-north-east pair of adjoint arrows with names
\newcommand{\Nnwadjar}{\@ifnextchar[{\basicNnwadjar}{\basicNnwadjar[67]}}%
\let\nnwadjaR=\Nnwadjar

% basic north-north-east pair of adjoint distributors
\def\basicnnwadjdist[#1]{\NNWADJDIST{}{}{#100}}%

% north-north-east pair of adjoint distributors
\newcommand{\nnwadjdist}{\@ifnextchar[{\basicnnwadjdist}{\basicnnwadjdist[67]}}%

% basic north-north-east pair of adjoint distributors with names
\def\basicNnwadjdist[#1]#2#3{\NNWADJDIST{#2}{#3}{#100}}%

% north-north-east pair of adjoint distributors with names
\newcommand{\Nnwadjdist}{\@ifnextchar[{\basicNnwadjdist}{\basicNnwadjdist[67]}}%
\let\nnwadjdisT=\Nnwadjdist


% EAST-EAST-NORTH-EAST ARROWS
% default length: 21100 units

% \EENEAR{f}{g}{n} draws a east-east-north-east arrow with names f, g
% and length n units
\newcommand{\EENEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(3,1){#3}}%
\put(\Y,\Z){\eenehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic east-east-north-east arrow
\def\basiceenear[#1]{\EENEAR{}{}{#100}}%

% east-east-north-east arrow
\newcommand{\eenear}{\@ifnextchar[{\basiceenear}{\basiceenear[211]}}%

% basic east-east-north-east arrow with upper name
\def\basicEenear[#1]#2{\EENEAR{#2}{}{#100}}%

% east-east-north-east arrow with upper name
\newcommand{\Eenear}{\@ifnextchar[{\basicEenear}{\basicEenear[211]}}%

% basic east-east-north-east arrow with lower name
\def\basiceeneaR[#1]#2{\EENEAR{}{#2}{#100}}%

% east-east-north-east arrow with lower name
\newcommand{\eeneaR}{\@ifnextchar[{\basiceeneaR}{\basiceeneaR[211]}}%

% EAST-EAST-SOUTH-EAST ARROWS
% default length: 21100 units

% \EESEAR{f}{g}{n} draws an east-east-south-east arrow with names f, g
% and length n units
\newcommand{\EESEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(3,-1){#3}}%
\put(\Y,-\Z){\eesehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic east-east-south-east arrow
\def\basiceesear[#1]{\EESEAR{}{}{#100}}%

% east-east-south-east arrow
\newcommand{\eesear}{\@ifnextchar[{\basiceesear}{\basiceesear[211]}}%

% basic east-east-south-east arrow with upper name
\def\basicEesear[#1]#2{\EESEAR{#2}{}{#100}}%

% east-east-south-east arrow with upper name
\newcommand{\Eesear}{\@ifnextchar[{\basicEesear}{\basicEesear[211]}}%

% basic east-east-south-east arrow with lower name
\def\basiceeseaR[#1]#2{\EESEAR{}{#2}{#100}}%

% east-east-south-east arrow with lower name
\newcommand{\eeseaR}{\@ifnextchar[{\basiceeseaR}{\basiceeseaR[211]}}%

% WEST-WEST-NORTH-WEST ARROWs
% default length: 21100 units

% \WWNWAR{f}{g}{n} draws a west-west-north-west arrow with names f, g
%       and length n units
\newcommand{\WWNWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-3,1){#3}}%
\put(-\Y,\Z){\wwnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic west-west-north-west arrow
\def\basicwwnwar[#1]{\WWNWAR{}{}{#100}}%

% west-west-north-west arrow
\newcommand{\wwnwar}{\@ifnextchar[{\basicwwnwar}{\basicwwnwar[211]}}%

% basic west-west-north-west arrow with upper name
\def\basicWwnwar[#1]#2{\WWNWAR{#2}{}{#100}}%

% west-west-north-west arrow with upper name
\newcommand{\Wwnwar}{\@ifnextchar[{\basicWwnwar}{\basicWwnwar[211]}}%

% basic west-west-north-west arrow with lower name
\def\basicwwnwaR[#1]#2{\WWNWAR{}{#2}{#100}}%

% west-west-north-west arrow with lower name
\newcommand{\wwnwaR}{\@ifnextchar[{\basicwwnwaR}{\basicwwnwaR[211]}}%

% WEST-WEST-SOUTH-WEST ARROWS
% default length: 21100 units

% \WWSWAR{f}{g} draws a west-west-south-west arrow with names f, g
\newcommand{\WWSWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-3,-1){#3}}%
\put(-\Y,-\Z){\wwswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic west-west-south-west arrow
\def\basicwwswar[#1]{\WWSWAR{}{}{#100}}%

% west-west-south-west arrow
\newcommand{\wwswar}{\@ifnextchar[{\basicwwswar}{\basicwwswar[211]}}%

% basic west-west-south-west arrow with upper name
\def\basicWwswar[#1]#2{\WWSWAR{#2}{}{#100}}%

% west-west-south-west arrow with upper name
\newcommand{\Wwswar}{\@ifnextchar[{\basicWwswar}{\basicWwswar[211]}}%

% basic west-west-south-west arrow with lower name
\def\basicwwswaR[#1]#2{\WWSWAR{}{#2}{#100}}%

% west-west-south-west arrow with lower name
\newcommand{\wwswaR}{\@ifnextchar[{\basicwwswaR}{\basicwwswaR[211]}}%


% NORTH-NORTH-NORTH-EAST ARROWS
% default length: 7100 units

% \NNNEAR{f}{g}{n} draws a north-north-north-east arrow with names f, g
% and length n units
\newcommand{\NNNEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\multiply \Z by 3%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(1,3){#3}}%
\put(\Y,\Z){\nnnehead}%
\truex{100}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{z}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic north-north-north-east arrow
\def\basicnnnear[#1]{\NNNEAR{}{}{#100}}%

% north-north-north-east arrow
\newcommand{\nnnear}{\@ifnextchar[{\basicnnnear}{\basicnnnear[71]}}%

% basic north-north-north-east arrow with upper name
\def\basicNnnear[#1]#2{\NNNEAR{#2}{}{#100}}%

% north-north-north-east arrow with upper name
\newcommand{\Nnnear}{\@ifnextchar[{\basicNnnear}{\basicNnnear[71]}}%

% basic north-north-north-east arrow with lower name
\def\basicnnneaR[#1]#2{\NNNEAR{}{#2}{#100}}%

% north-north-north-east arrow with lower name
\newcommand{\nnneaR}{\@ifnextchar[{\basicnnneaR}{\basicnnneaR[71]}}%

% SOUTH-SOUTH-SOUTH-WEST ARROWS
% default length: 7100 units

% \SSSWAR{f}{g}{n} draws a south-south-south-west arrow with names f, g
% and length n units
\newcommand{\SSSWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\multiply \Z by 3%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-1,-3){#3}}%
\put(-\Y,-\Z){\ssswhead}%
\truex{100}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{z}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic south-south-south-west arrow
\def\basicssswar[#1]{\SSSWAR{}{}{#100}}%

% south-south-south-west arrow
\newcommand{\ssswar}{\@ifnextchar[{\basicssswar}{\basicssswar[71]}}%

% basic south-south-south-west arrow with upper name
\def\basicSsswar[#1]#2{\SSSWAR{#2}{}{#100}}%

% south-south-south-west arrow with upper name
\newcommand{\Ssswar}{\@ifnextchar[{\basicSsswar}{\basicSsswar[71]}}%

% basic south-south-south-west arrow with lower name
\def\basicssswaR[#1]#2{\SSSWAR{}{#2}{#100}}%

% south-south-south-west arrow with lower name
\newcommand{\ssswaR}{\@ifnextchar[{\basicssswaR}{\basicssswaR[71]}}%

% SOUTH-SOUTH-SOUTH-EAST ARROWS
% default length: 7100 units

% \SSSEAR{f}{g}{n} draws a south-south-south-east arrow with names f, g
% and length n units
\newcommand{\SSSEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\multiply \Z by 3%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(1,-3){#3}}%
\put(\Y,-\Z){\sssehead}%
\truex{200}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{z}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic south-south-south-east arrow
\def\basicsssear[#1]{\SSSEAR{}{}{#100}}%

% south-south-south-east arrow
\newcommand{\sssear}{\@ifnextchar[{\basicsssear}{\basicsssear[71]}}%

% basic south-south-south-east arrow with upper name
\def\basicSssear[#1]#2{\SSSEAR{#2}{}{#100}}%

% south-south-south-east arrow with upper name
\newcommand{\Sssear}{\@ifnextchar[{\basicSssear}{\basicSssear[71]}}%

% basic south-south-south-east arrow with lower name
\def\basicssseaR[#1]#2{\SSSEAR{}{#2}{#100}}%

% south-south-south-east arrow with lower name
\newcommand{\ssseaR}{\@ifnextchar[{\basicssseaR}{\basicssseaR[71]}}%

% NORTH-NORTH-NORTH-WEST ARROWS
% default length: 7100 units

% \NNNWAR{f}{g}{n} draws a north-north-north-west arrow with names f, g
% and length n units
\newcommand{\NNNWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=\Y%
\multiply \Z by 3%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-1,3){#3}}%
\put(-\Y,\Z){\nnnwhead}%
\truex{200}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{z}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic north-north-north-west arrow
\def\basicnnnwar[#1]{\NNNWAR{}{}{#100}}%

% north-north-north-west arrow
\newcommand{\nnnwar}{\@ifnextchar[{\basicnnnwar}{\basicnnnwar[71]}}%

% basic north-north-north-west arrow with upper name
\def\basicNnnwar[#1]#2{\NNNWAR{#2}{}{#100}}%

% north-north-north-west arrow with upper name
\newcommand{\Nnnwar}{\@ifnextchar[{\basicNnnwar}{\basicNnnwar[71]}}%

% basic north-north-north-west arrow with lower name
\def\basicnnnwaR[#1]#2{\NNNWAR{}{#2}{#100}}%

% north-north-north-west arrow with lower name
\newcommand{\nnnwaR}{\@ifnextchar[{\basicnnnwaR}{\basicnnnwaR[71]}}%

% NORTH-EAST-EAST-NORTH-EAST ARROWS
% default length: 21500 units

% \NEENEAR{f}{g}{n} draws a north-east-east-north-east arrow with names f, g
% and length n units
\newcommand{\NEENEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(3,2){#3}}%
\put(\Y,\Z){\neenehead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic north-east-east-north-east arrow
\def\basicneenear[#1]{\NEENEAR{}{}{#100}}%

% north-east-east-north-east arrow
\newcommand{\neenear}{\@ifnextchar[{\basicneenear}{\basicneenear[215]}}%

% basic north-east-east-north-east arrow with upper name
\def\basicNeenear[#1]#2{\NEENEAR{#2}{}{#100}}%

% north-east-east-north-east arrow with upper name
\newcommand{\Neenear}{\@ifnextchar[{\basicNeenear}{\basicNeenear[215]}}%

% basic north-east-east-north-east arrow with lower name
\def\basicneeneaR[#1]#2{\NEENEAR{}{#2}{#100}}%

% north-east-east-north-east arrow with lower name
\newcommand{\neeneaR}{\@ifnextchar[{\basicneeneaR}{\basicneeneaR[215]}}%

% SOUTH-EAST-EAST-SOUTH-EAST ARROWS
% DEFAULT LENGTH: 21500 UNITS

% \SEESEAR{f}{g} draws an sout-east-east-south-east arrow with names f, g
% and length n units
\newcommand{\SEESEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(3,-2){#3}}%
\put(\Y,-\Z){\seesehead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic south-east-east-south-east arrow
\def\basicseesear[#1]{\SEESEAR{}{}{#100}}%

% south-east-east-south-east arrow
\newcommand{\seesear}{\@ifnextchar[{\basicseesear}{\basicseesear[215]}}%

% basic south-east-east-south-east arrow with upper name
\def\basicSeesear[#1]#2{\SEESEAR{#2}{}{#100}}%

% south-east-east-south-east arrow with upper name
\newcommand{\Seesear}{\@ifnextchar[{\basicSeesear}{\basicSeesear[215]}}%

% basic south-east-east-south-east arrow with lower name
\def\basicseeseaR[#1]#2{\SEESEAR{}{#2}{#100}}%

% south-east-east-south-east arrow with lower name
\newcommand{\seeseaR}{\@ifnextchar[{\basicseeseaR}{\basicseeseaR[215]}}%

% NORTH-WEST-WEST-NORTH-WEST ARROWS
% default length: 21500 units

% \NWWNWAR{f}{g}{n} draws a north-west-west-north-west arrow with names f, g
% and length n units
\newcommand{\NWWNWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-3,2){#3}}%
\put(-\Y,\Z){\nwwnwhead}%
\truex{200}\truey{800}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{y}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic north-west-west-north-west arrow
\def\basicnwwnwar[#1]{\NWWNWAR{}{}{#100}}%

% north-west-west-north-west arrow
\newcommand{\nwwnwar}{\@ifnextchar[{\basicnwwnwar}{\basicnwwnwar[215]}}%

% basic north-west-west-north-west arrow with upper name
\def\basicNwwnwar[#1]#2{\NWWNWAR{#2}{}{#100}}%

% north-west-west-north-west arrow with upper name
\newcommand{\Nwwnwar}{\@ifnextchar[{\basicNwwnwar}{\basicNwwnwar[215]}}%

% basic north-west-west-north-west arrow with lower name
\def\basicnwwnwaR[#1]#2{\NWWNWAR{}{#2}{#100}}%

% north-west-west-north-west arrow with lower name
\newcommand{\nwwnwaR}{\@ifnextchar[{\basicnwwnwaR}{\basicnwwnwaR[215]}}%

% SOUTH-WEST-WEST-SOUTH-WEST ARROWS
% default length: 21500 units

% \SWWSWAR{f}{g}{n} draws a south-west-west-south-west arrow with names f, g
% and length n units
\newcommand{\SWWSWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\divide \Z by 3%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-3,-2){#3}}%
\put(-\Y,-\Z){\swwswhead}%
\truex{200}\truey{800}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{y}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic south-west-west-south-west arrow
\def\basicswwswar[#1]{\SWWSWAR{}{}{#100}}%

% south-west-west-south-west arrow
\newcommand{\swwswar}{\@ifnextchar[{\basicswwswar}{\basicswwswar[215]}}%

% basic south-west-west-south-west arrow with upper name
\def\basicSwwswar[#1]#2{\SWWSWAR{#2}{}{#100}}%

% south-west-west-south-west arrow with upper name
\newcommand{\Swwswar}{\@ifnextchar[{\basicSwwswar}{\basicSwwswar[215]}}%

% basic south-west-west-south-west arrow with lower name
\def\basicswwswaR[#1]#2{\SWWSWAR{}{#2}{#100}}%

% south-west-west-south-west arrow with lower name
\newcommand{\swwswaR}{\@ifnextchar[{\basicswwswaR}{\basicswwswaR[215]}}%


% NORTH-EAST-NORTH-NORTH-EAST ARROWS
% default length 14300 units

% \NENNEAR{f}{g}{n} draws a north-east-north-north-east arrow with names f, g
% and length n units
\newcommand{\NENNEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\multiply \Z by 3%
\divide \Z by 4%
\begin{picture}(0,0)%
\put(-\Y,-\Z){\line(2,3){#3}}%
\put(\Y,\Z){\nennehead}%
\truex{100}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{z}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic north-east-north-north-east arrow
\def\basicnennear[#1]{\NENNEAR{}{}{#100}}%

% north-east-north-north-east arrow
\newcommand{\nennear}{\@ifnextchar[{\basicnennear}{\basicnennear[143]}}%

% basic north-east-north-north-east arrow with upper name
\def\basicNennear[#1]#2{\NENNEAR{#2}{}{#100}}%

% north-east-north-north-east arrow with upper name
\newcommand{\Nennear}{\@ifnextchar[{\basicNennear}{\basicNennear[143]}}%

% basic north-east-north-north-east arrow with lower name
\def\basicnenneaR[#1]#2{\NENNEAR{}{#2}{#100}}%

% north-east-north-north-east arrow with lower name
\newcommand{\nenneaR}{\@ifnextchar[{\basicnenneaR}{\basicnenneaR[143]}}%

% SOUTH-WEST-SOUTH-SOUTH-WEST ARROWS
% default length: 14300 units

% \SWSSWAR{f}{g}{n} draws a south-west-south-south-west arrow with names f, g
% and length n units
\newcommand{\SWSSWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\multiply \Z by 3%
\divide \Z by 4%
\begin{picture}(0,0)%
\put(\Y,\Z){\line(-2,-3){#3}}%
\put(-\Y,-\Z){\swsswhead}%
\truex{100}\truez{600}%
\put(-\value{x},\value{x}){\makebox(0,\value{z})[r]{${#1}$}}%
\put(\value{x},-\value{z}){\makebox(0,\value{z})[l]{${#2}$}}%
\end{picture}}%

% basic south-west-south-south-west arrow
\def\basicswsswar[#1]{\SWSSWAR{}{}{#100}}%

% south-west-south-south-west arrow
\newcommand{\swsswar}{\@ifnextchar[{\basicswsswar}{\basicswsswar[143]}}%

% basic south-west-south-south-west arrow with upper name
\def\basicSwsswar[#1]#2{\SWSSWAR{#2}{}{#100}}%

% south-west-south-south-west arrow with upper name
\newcommand{\Swsswar}{\@ifnextchar[{\basicSwsswar}{\basicSwsswar[143]}}%

% basic south-west-south-south-west arrow with lower name
\def\basicswsswaR[#1]#2{\SWSSWAR{}{#2}{#100}}%

% south-west-south-south-west arrow with lower name
\newcommand{\swsswaR}{\@ifnextchar[{\basicswsswaR}{\basicswsswaR[143]}}%

% SOUT-EAST-SOUTH-SOUTH-EAST ARROWS
% default length: 14300 units

% \SESSEAR{f}{g}{n} draws a south-east-south-south-east arrow with names f, g
% and length n units
\newcommand{\SESSEAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\multiply \Z by 3%
\divide \Z by 4%
\begin{picture}(0,0)%
\put(-\Y,\Z){\line(2,-3){#3}}%
\put(\Y,-\Z){\sessehead}%
\truex{200}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{z}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic south-east-south-south-east arrow
\def\basicsessear[#1]{\SESSEAR{}{}{#100}}%

% south-east-south-south-east arrow
\newcommand{\sessear}{\@ifnextchar[{\basicsessear}{\basicsessear[143]}}%

% basic south-east-south-south-east arrow with upper name
\def\basicSessear[#1]#2{\SESSEAR{#2}{}{#100}}%

% south-east-south-south-east arrow with upper name
\newcommand{\Sessear}{\@ifnextchar[{\basicSessear}{\basicSessear[143]}}%

% basic south-east-south-south-east arrow with lower name
\def\basicsesseaR[#1]#2{\SESSEAR{}{#2}{#100}}%

% south-east-south-south-east arrow with lower name
\newcommand{\sesseaR}{\@ifnextchar[{\basicsesseaR}{\basicsesseaR[143]}}%

% NORTH-WEST-NORTH-NORTH-WEST ARROWS
% default length: 14300 units

% \NWNNWAR{f}{g}{n} draws a north-west-north-north-west arrow with names f, g
% and length n units
\newcommand{\NWNNWAR}[3]{\testdiagrammode%
\Y=#3%
\divide \Y by 2%
\Z=#3%
\multiply \Z by 3%
\divide \Z by 4%
\begin{picture}(0,0)%
\put(\Y,-\Z){\line(-2,3){#3}}%
\put(-\Y,\Z){\nwnnwhead}%
\truex{200}\truez{600}%
\put(\value{x},\value{x}){\makebox(0,\value{z})[l]{${#1}$}}%
\put(-\value{x},-\value{z}){\makebox(0,\value{z})[r]{${#2}$}}%
\end{picture}}%

% basic north-west-north-north-west arrow
\def\basicnwnnwar[#1]{\NWNNWAR{}{}{#100}}%

% north-west-north-north-west arrow
\newcommand{\nwnnwar}{\@ifnextchar[{\basicnwnnwar}{\basicnwnnwar[143]}}%

% basic north-west-north-north-west arrow with upper name
\def\basicNwnnwar[#1]#2{\NWNNWAR{#2}{}{#100}}%

% north-west-north-north-west arrow with upper name
\newcommand{\Nwnnwar}{\@ifnextchar[{\basicNwnnwar}{\basicNwnnwar[143]}}%

% basic north-west-north-north-west arrow with lower name
\def\basicnwnnwaR[#1]#2{\NWNNWAR{}{#2}{#100}}%

% north-west-north-north-west arrow with lower name
\newcommand{\nwnnwaR}{\@ifnextchar[{\basicnwnnwaR}{\basicnwnnwaR[143]}}%

% HORIZONTAL CURVED ARROWS

% The following commands produce horizontal curved arrows
% default length: 160 units

% North\East curved arrow with name [1] and length [2]x100 units
\newcommand{\Necurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1300}\truey{2000}\truez{200}%
\put(0,\value{x}){\oval(#200,\value{y})[t]}%
\put(0,\value{x}){\makebox(0,0){\begin{picture}(#200,0)%
\put(#200,0){\line(0,-1){\value{z}}}%
\put(#200,-\value{z}){\shead}%
\put(0,0){\line(0,-1){\value{z}}}\end{picture}}}%
\truex{2500}%
\put(0,\value{x}){\makebox(0,0)[b]{${#1}$}}%
\end{picture}}%

% basic north\east curved arrow
\def\basicnecurvar[#1]{\Necurve{}{#1}}

% north\east curved arrow
\newcommand{\necurvar}{\@ifnextchar[{\basicnecurvar}{\basicnecurvar[160]}}%

% basic north\east curved arrow with name
\def\basicNecurvar[#1]#2{\Necurve{#2}{#1}}%

% north\east curved arrow with name
\newcommand{\Necurvar}{\@ifnextchar[{\basicNecurvar}{\basicNecurvar[160]}}%
\let\necurvaR=\Necurvar

% North\West curved arrow with name [1] and length [2]x100 units
\newcommand{\Nwcurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1300}\truey{2000}\truez{200}%
\put(0,\value{x}){\oval(#200,\value{y})[t]}%
\put(0,\value{x}){\makebox(0,0){\begin{picture}(#200,0)%
\put(#200,0){\line(0,-1){\value{z}}}%
\put(0,0){\line(0,-1){\value{z}}}%
\put(0,-\value{z}){\shead}%
\end{picture}}}%
\truex{2500}%
\put(0,\value{x}){\makebox(0,0)[b]{${#1}$}}%
\end{picture}}%

% basic north\west curved arrow
\def\basicnwcurvar[#1]{\Nwcurve{}{#1}}

% north\west curved arrow
\newcommand{\nwcurvar}{\@ifnextchar[{\basicnwcurvar}{\basicnwcurvar[160]}}%

% basic north\west curved arrow with name
\def\basicNwcurvar[#1]#2{\Nwcurve{#2}{#1}}%

% north\west curved arrow with name
\newcommand{\Nwcurvar}{\@ifnextchar[{\basicNwcurvar}{\basicNwcurvar[160]}}%
\let\nwcurvaR=\Nwcurvar

% South\East curved arrow with name [1] and length [2]x100 units
\newcommand{\Securve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1300}\truey{2000}\truez{200}%
\put(0,-\value{x}){\oval(#200,\value{y})[b]}%
\put(0,-\value{x}){\makebox(0,0){\begin{picture}(#200,0)%
\put(#200,0){\line(0,1){\value{z}}}%
\put(0,0){\line(0,1){\value{z}}}%
\put(#200,\value{z}){\nhead}%
\end{picture}}}%
\truex{2500}%
\put(0,-\value{x}){\makebox(0,0)[t]{${#1}$}}%
\end{picture}}%

% basic south\east curved arrow
\def\basicsecurvar[#1]{\Securve{}{#1}}

% south\east curved arrow
\newcommand{\securvar}{\@ifnextchar[{\basicsecurvar}{\basicsecurvar[160]}}%

% basic south\east curved arrow with name
\def\basicSecurvar[#1]#2{\Securve{#2}{#1}}%

% south\east curved arrow with name
\newcommand{\Securvar}{\@ifnextchar[{\basicSecurvar}{\basicSecurvar[160]}}%
\let\securvaR=\Securvar

% South\West curved arrow with name [1] and length [2]x100 units
\newcommand{\Swcurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1300}\truey{2000}\truez{200}%
\put(0,-\value{x}){\oval(#200,\value{y})[b]}%
\put(0,-\value{x}){\makebox(0,0){\begin{picture}(#200,0)%
\put(#200,0){\line(0,1){\value{z}}}%
\put(0,0){\line(0,1){\value{z}}}%
\put(0,\value{z}){\nhead}%
\end{picture}}}%
\truex{2500}%
\put(0,-\value{x}){\makebox(0,0)[t]{${#1}$}}%
\end{picture}}%

% basic south\west curved arrow
\def\basicswcurvar[#1]{\Swcurve{}{#1}}

% south\west curved arrow
\newcommand{\swcurvar}{\@ifnextchar[{\basicswcurvar}{\basicswcurvar[160]}}%

% basic south\west curved arrow with name
\def\basicSwcurvar[#1]#2{\Swcurve{#2}{#1}}%

% south\west curved arrow with name
\newcommand{\Swcurvar}{\@ifnextchar[{\basicSwcurvar}{\basicSwcurvar[160]}}%
\let\swcurvaR=\Swcurvar

% VERTICAL CURVED ARROWS

% The following commands produce vertical curved arrows
% default length: 160pt

% East\South curved arrow with name [1] and length [2]x100 units
\newcommand{\Escurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1400}\truey{2000}\truez{200}%
\put(\value{x},0){\oval(\value{y},#200)[r]}%
\put(\value{x},0){\makebox(0,0){\begin{picture}(0,#200)%
\put(0,0){\line(-1,0){\value{z}}}%
\put(0,#200){\line(-1,0){\value{z}}}%
\put(-\value{z},0){\whead}%
\end{picture}}}%
\truex{2500}%
\put(\value{x},0){\makebox(0,0)[l]{${#1}$}}%
\end{picture}}%

% basic east\south curved arrow
\def\basicescurvar[#1]{\Escurve{}{#1}}

% east\south curved arrow
\newcommand{\escurvar}{\@ifnextchar[{\basicescurvar}{\basicescurvar[160]}}%

% basic east\south curved arrow with name
\def\basicEscurvar[#1]#2{\Escurve{#2}{#1}}%

% east\south curved arrow with name
\newcommand{\Escurvar}{\@ifnextchar[{\basicEscurvar}{\basicEscurvar[160]}}%
\let\escurvaR=\Escurvar

% East\North curved arrow with name [1] and length [2]x100 units
\newcommand{\Encurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1400}\truey{2000}\truez{200}%
\put(\value{x},0){\oval(\value{y},#200)[r]}%
\put(\value{x},0){\makebox(0,0){\begin{picture}(0,#200)%
\put(0,0){\line(-1,0){\value{z}}}%
\put(0,#200){\line(-1,0){\value{z}}}%
\put(-\value{z},#200){\whead}%
\end{picture}}}%
\truex{2500}%
\put(\value{x},0){\makebox(0,0)[l]{${#1}$}}%
\end{picture}}%

% basic east\north curved arrow
\def\basicencurvar[#1]{\Encurve{}{#1}}

% east\north curved arrow
\newcommand{\encurvar}{\@ifnextchar[{\basicencurvar}{\basicencurvar[160]}}%

% basic east\north curved arrow with name
\def\basicEncurvar[#1]#2{\Encurve{#2}{#1}}%

% east\north curved arrow with name
\newcommand{\Encurvar}{\@ifnextchar[{\basicEncurvar}{\basicEncurvar[160]}}%
\let\encurvaR=\Encurvar

% West\South curved arrow with name [1] and length [2]x100 units
\newcommand{\Wscurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1300}\truey{2000}\truez{200}%
\put(-\value{x},0){\oval(\value{y},#200)[l]}%
\put(-\value{x},0){\makebox(0,0){\begin{picture}(0,#200)%
\put(0,0){\line(1,0){\value{z}}}%
\put(0,#200){\line(1,0){\value{z}}}%
\put(\value{z},0){\ehead}%
\end{picture}}}%
\truex{2400}%
\put(-\value{x},0){\makebox(0,0)[r]{${#1}$}}%
\end{picture}}%

% basic west\south curved arrow
\def\basicwscurvar[#1]{\Wscurve{}{#1}}

% west\south curved arrow
\newcommand{\wscurvar}{\@ifnextchar[{\basicwscurvar}{\basicwscurvar[160]}}%

% basic west\south curved arrow with name
\def\basicWscurvar[#1]#2{\Wscurve{#2}{#1}}%

% west\south curved arrow with name
\newcommand{\Wscurvar}{\@ifnextchar[{\basicWscurvar}{\basicWscurvar[160]}}%
\let\wscurvaR=\Wscurvar

% West\North curved arrow with name [1] and length [2]x100 units
\newcommand{\Wncurve}[2]%
{\testdiagrammode\begin{picture}(0,0)%
\truex{1300}\truey{2000}\truez{200}%
\put(-\value{x},0){\oval(\value{y},#200)[l]}%
\put(-\value{x},0){\makebox(0,0){\begin{picture}(0,#200)%
\put(0,0){\line(1,0){\value{z}}}%
\put(\value{z},#200){\ehead}%
\put(0,#200){\line(1,0){\value{z}}}%
\end{picture}}}%
\truex{2400}%
\put(-\value{x},0){\makebox(0,0)[r]{${#1}$}}%
\end{picture}}%

% basic west\north curved arrow
\def\basicwncurvar[#1]{\Wncurve{}{#1}}

% west\north curved arrow
\newcommand{\wncurvar}{\@ifnextchar[{\basicwncurvar}{\basicwncurvar[160]}}%

% basic west\north curved arrow with name
\def\basicWncurvar[#1]#2{\Wncurve{#2}{#1}}%

% west\north curved arrow with name
\newcommand{\Wncurvar}{\@ifnextchar[{\basicWncurvar}{\basicWncurvar[160]}}%
\let\wncurvaR=\Wncurvar

\catcode`\@=12

